The information content of galaxy surveys

A large fraction of this thesis is dedicated to the study of the information content of random fields with heavy tails, in particular the lognormal field, a model for the matter density fluctuation field. It is well known that in the nonlinear regime of structure formation, the matter fluctuation field develops such large tails. It has also been suggested that fields with large tails are not necessarily well described by the hierarchy of $N$-point functions. In this thesis, we are able to make this last statement precise and with the help of the lognormal model to quantify precisely its implications for inference on cosmological parameters : we find as our main result that only a tiny fraction of the total Fisher information of the field is still contained in the hierarchy of $N$-point moments in the nonlinear regime, rendering parameter inference from such moments very inefficient. We show that the hierarchy fails to capture the information that is contained in the underdense regions, which at the same time are found to be the most rich in information. We find further our results to be very consistent with numerical analysis using $N$-body simulations. We also discuss these issues with the help of explicit families of fields with the same hierarchy of $N$-point moments defined in this work. A similar analysis is then applied to the convergence field, the weighted projection of the matter density fluctuation field along the line of sight, with similar conclusions. We also show how simple mappings can correct for this inadequacy, consistently with previous findings in the literature (Abridged) .

==> chapter1.tex <==
%\setprelude{\uppercase{A\scriptsize{n inconceivably numerous host of stars must be here arranged\\ together }\normalsize{[...],}\scriptsize{ because their free positions towards each other\\ would otherwise have presented irregular forms and not exact\\ figures}}\normalsize{.}
%\vspace{5truemm}\\
%\normalsize{Immanuel Kant, {\it Universal History and Theory of the Heavens} \cite{kant1755}}}

\chapter{Entropy, Information and weak lensing}
\label{ch1}

\newcommand{\btheta}{\boldsymbol {\theta}}
\newcommand{\bmu}{\boldsymbol {\mu}}
\newcommand{\bphi}{\boldsymbol {\phi}}
\newcommand{\vecl}{\boldsymbol {l}}



\begin{center}
This paper is aimed at developing a better understanding of the structure of the information that in contained in galaxy surveys, so as  to find optimal ways to combine observables from such surveys. We first show how Jaynes' Maximal Entropy Principle allows us, in the general case, to express the Fisher information content of data sets in terms of the curvature of the Shannon entropy surface with respect to the relevant observables. This allows us to understand the Fisher information content of a data set, once a physical model is specified, independently of the specific way that the data will be processed, and without any assumptions of Gaussianity. This includes as a special case the standard Fisher matrix prescriptions for Gaussian variables widely used in the cosmological community, for instance for power spectra extraction.
\textbf{As an application of this approach, we evaluate the prospects of a joint analysis of weak lensing tracers up to second order in the shapes distortions}, in the case that the noise in each probe can be effectively treated as model independent. These include the magnification, the two ellipticity and the four flexion fields. At the two point level, we show that the only effect of treating these observables in combination is a simple scale dependent decrease of the noise contaminating the accessible spectrum of the lensing E-mode. We provide simple bounds to its extraction by a combination of such probes, as well as its quantitative evaluation when the correlations between the noise variables for any two such probes can be neglected.
\end{center}

\begin{center}
Parts of Section \ref{sec:gim2dprofiles} are based on \citet{sargent07} (\url{http://adsabs.harvard.edu/abs/2007ApJS..172..434S}).\\ Section \ref{sec:ZEST} is extracted from Scarlata, Carollo, Lilly, Sargent et al. \cite{scarlata07a} (\url{http://adsabs.harvard.edu/abs/2007ApJS..172..406S}).
\end{center}


\section{Introduction} 

With cosmological data sets currently going through a rapid period of growth, it is increasingly important to quantitatively understand the potential and limits of particular data sets to test a physical model or hypothesis. For this, the Fisher information matrix has become a widely used tool in cosmology.

The concept of Fisher information has a long history. It was first coined by the statistician and geneticist R.A. Fisher \citep{fisher25} under the name of intrinsic accuracy of frequency curves. It has found its way into the cosmological community over the last decade, where it is often used to optimise survey configurations \citep{2007MNRAS.381.1018A,2007MNRAS.377..185P,2006astro.ph..9591A,2009ApJ...695..652B} of planned cosmology experiments or to evaluate the expected errors on certain cosmological parameters with some observables \citep{1997ApJ...480...22T,Tegmark97,1999ApJ...514L..65H,2004PhRvD..70d3009H}. 

Much of the work to date has been limited to particular sets of observables and estimators. Usually, it is assumed that observational errors as well as the parameters probability distribution have Gaussian shape. The first aim of this work is to propose a framework to express the global Fisher information content of large data sets in a way that is independent of the specific ways that the data will be processed, and in realistic situations, where the exact statistical properties of the data are not known precisely. This should then provide a well motivated basis point in order to perform systematic and robust trade-off studies. For this purpose a number of useful concepts already exist in  the fields of information theory and probability theory, such as Shannon entropy or relative entropy \citep{Kullback}, which we can use to gain a better understanding of what we can achieve with planned experiments. Specifically, we will show that we can achieve our aim by combining Fisher's information measure with Jaynes' Principle of Maximal Entropy.  \citep{jaynes83,jaynes2003}.
\newline\indent 
In a second step, as a concrete application of this approach, we investigate the joint entropy and information content of multiple observables of the same underlying, cosmologically interesting field. This is a very relevant situation in weak lensing \citep{1992grle.book.....S,2001PhR...340..291B,2003ARA&A..41..645R,2006astro.ph.12667M,2006glsw.book.....S}, where the distortions of galaxy images to any order are sourced by the lensing potential field. \newline\newline\indent
This paper is divided into the following sections. In section \ref{Setting the scene},  we present in details our approach.  We first review and develop some key properties of Fisher information, and its link to the Cramer Rao inequality. We put a strong emphasis on its interpretation as a measure of information on model parameters in a data set, that is obtained from the probability distribution of different observational outcomes as function of these same model parameters. Readers familiar with these aspects may jump to section {\ref{The structure of the information in a physical model}}, where we introduce Jaynes' Maximum Entropy Principle, and show how it ideally completes Fisher's information measure, allowing us to understand the information content of a data set on a physical model in the case of incomplete knowledge.
In section \ref{application}, we show how the study of the Shannon entropy of a set of homogeneous fields provide a simple and model parameter independent answer to the question of the combination of the weak lensing observables shear, magnification and flexion.
We provide in section \ref{results}  quantitative evaluation of the prospects of such a combination at the two-point level for typical dark energy surveys parameters, and conclude in section \ref{discussion} with a summary of the results and a discussion. A set of appendices collects some technical details.
%-------------------------------------------------------------------------
\section{Fisher Information and Jaynes MaxEnt principle}
\label{Setting the scene}
The concept of Fisher information is rich and not limited to parameter error estimation. We review here a few simple points of interest that justify the interpretation of the Fisher matrix as a measure of the information content of an experiment. Let us begin by considering the case of a single measurement $X$, with different possible outcomes, or realisations, $x$, and our model has a single parameter $\alpha$. We also assume that we have knowledge, prior to the given experiment, of the probability density function $p_X(x,\alpha)$, which depends on our parameter $\alpha$, that gives the probability of observing particular realisations for each value of the model parameter.
The Fisher information, $F$, in $X$ on $\alpha$, is a non-negative scalar in this one parameter case. It is defined  in a fully general way as a sum over all realisations of the data \citep{fisher25}:
\beq \label{FisherI}
F^X(\alpha) = \av{\left( \frac{\partial \ln p_X(x,\alpha)}{\partial\alpha} \right)^2}.
\enq
Angle brackets will always stand for mean value with respect to the probability density function, i.e. for any function $f$,
\beq
\av{f} \equiv \int dx\: p_X(x,\alpha) f(x).
\enq
Three simple but important properties of Fisher information are worth highlighting at this point. \newline

\indent The first is that $F^X(\alpha)$ is positive definite, and it vanishes if and only if the parameter $\alpha$ does not impact the data, i.e. if the derivative of $p_X(x,\alpha)$ with respect to $\alpha$ is zero for every realisation $x$.
\newline

\indent The second point is that it is invariant to invertible manipulations of the observed data. This can be seen by considering an invertible change of variable $y = f(x)$, which, due to the rules of probability theory can be expressed as 
\beq
p_Y(y,\alpha) = p_X(x,\alpha)\left |\frac {dx}{dy}\right|.
\enq
Thus
\beq
\frac{\partial \ln p_Y(y,\alpha)}{\partial \alpha} = \frac{\partial \ln p_X(x,\alpha)}{\partial \alpha},
\enq 
leading to the simple equivalence that $F^X(\alpha) = F^Y(\alpha)$. On the other hand, information may be lost when the transformation is not unique in both directions. \citep[e.g., see][for a proof]{Rao}. For instance, if the data is combined to produce a new variable that could arise from different sets of data points.
This is only the statement that manipulations of the data leads, at best, only to conservation of the information.\newline

\indent The third point is that information from independent experiments add together. Indeed, if two experiments with data $X$ and $Y$ are independent, then the joint probability density factorises,
\beq
p_{XY}(x,y) = p_X(x)p_Y(y),
\enq
and it is easy to show that the joint information in the observations decouples,
\beq
F^{XY}(\alpha) = F^X(\alpha) + F^Y(\alpha).
\enq\newline
\indent 
%These three properties satisfy what we might intuitively expect from a mathematical implementation of an abstract concept such as information. However, we can ask the reverse question and try to find an alternative measure of information that may be better suited, for a particular purpose, than the Fisher information. The integrand in equation (\ref{FisherI}), Fisher's information 'density',  associates some information content to observations of realisations of $x$ within the range $[x,x + dx]$. In appendix \ref{appendix_unique}, we show that it  is in fact the only such density that, up to a constant factor, : (i) depends on $p_X(x,\alpha)$ and $\partial_\alpha p_X(x,\alpha)$ only; and (ii) meets the three requirements above.
These properties are making the Fisher information a meaningful measure of information. This is independent of its interpretation as providing error bars on parameters. It further implies that once a physical model is specified with a given set of parameters, a given experiment has a definite information content that can only decrease with data processing.
\subsection{The case of a single observable}\label{single observable}
To quantify the last point above, and in order to get an understanding of the structure of the information in a data set, we first review a simple situation, common in cosmology, where the extraction of the model parameter $\alpha$ from the data goes through the intermediate step of estimating a particular observable, $D$, from the data, $x$, with the help of which $\alpha$  will be inferred. A typical example could be, from the temperature map of the  CMB ($x$), the measurement of the power spectra of the fluctuations ($D$), from which a cosmological parameter ($\alpha$) is extracted.
The observable $D$ is measured from $x$ with the help of an estimator, that we call $\hat D$, and that we will take as unbiased. This means that its mean value, as would be obtained for instance if many realizations of the data were available, converges to the actual value that we want to compare with the model prediction,
\beq
\lat \hat D\rat = D(\alpha).
\enq
A measure for its deviations from sample to sample, or the uncertainty in the actual measurement, is then given by the variance of $\hat D$, defined as
\beq \label{variance}
\Var{\hat D} = \av{\hat D^2} - \av{\hat D}^2.
\enq
In such a situation, a major role is played by the so-called Cram\'{e}r-Rao 
 inequality (\cite{Rao}),  that links the Fisher information content of the data to the variance of the estimator, stating that
\beq \label{CR}
\textrm{Var}(\hat D) F^X(\alpha) \ge \left(\frac{\partial D(\alpha)}{\partial \alpha}\right)^2.
\enq
This equation holds for any such estimator $\hat D$ and any model parameter $\alpha$. Two different interpretations of this equation are possible: \newline

\indent The first bounds the variance of $\hat D$ by the inverse of the Fisher information. To see this, we consider the special case of the model parameter $\alpha$ being $D$ itself. Although we are making in general a conceptual distinction between the observable $D$ and the model parameter $\alpha$, nothing requires us from doing so. Since $\alpha$ is now equal to $D$, the derivative on the right hand side becomes unity, and one obtains
\beq \label{CRB}
\textrm{Var}(\hat D) \ge \frac 1 {F^X(D)}.
\enq
The variance of any unbiased estimator $\hat D$ of  $D$ is therefore bounded by the inverse of the amount of information $F^X(D)$ the data possess on $D$. If $F^X(D)$ is known it gives a useful lower limit on the error bars that the analysis of the data can put on this observable.
\newline
\newline
We emphasise at this point that this bound only holds in the case of unbiased estimators. There are cosmologically relevant situations where biased estimators can go beyond this level, as in the zero mean Gaussian variable case discussed in Appendix \ref{appendix_biased}.
\indent The second reading of the Cram\'{e}r-Rao 
 inequality, closer in spirit to the present work, is to look at how information is lost by constructing the observable $D$, and discarding the rest of the data set. For this, we rewrite trivially equation (\ref{CR}) as
\beq \label{CramerRao}
F^X(\alpha) \ge  \left(\frac{\partial D}{\partial \alpha}\right)^{2} \frac 1 {\textrm{Var}(\hat D)}.
\enq
The expression on the right hand side is the ratio of the sensitivity of the observable to the model parameter $\lp \frac{ \partial D}{\partial \alpha}\rp^2 $, to the accuracy with which the observable can be extracted from the data, $\textrm{Var}(\hat D)$. One of the conceivable approaches in order to estimate the true value of the parameter $\alpha$, is to perform a $\chi^2$ fit to the measured value of $D$ . It is simple to show that this ratio, evaluated at the best fit value, is in fact proportional to the expected value of the curvature of $\chi^2(\alpha)$ at this value. Since the curvature of the $\chi^2$ surface describes how fast the value of the $\chi^2$ is increasing when moving away from the best fit value, its inverse can be interpreted as an approximation to the error bar that the analysis with the help of  $\hat D$ will put on $\alpha$. 
\newline
\newline
Thus, equation (\ref{CramerRao}) shows that by only considering $D$ and not the full data set, we may have lost information on $\alpha$, a loss given by the difference between the left and right hand side of that equation. While the latter may be interpreted as the information on $\alpha$ contained in the part of the data represented by $D$, we may have lost trace of any other source of information. 
%-------------------------------------------------------------------------
\subsection{The general case} \label{CramerRaoMulti}
These considerations on the Cram\'{e}r-Rao 
 bound can be easily generalised to the case of many parameters and many estimators of as many observables. Still dealing with a measurement $X$ with outcomes $x$, we want to estimate a set of parameters
\beq
\boldsymbol \theta = (\alpha, \beta,\cdots)
\enq
 with the help of some vector of observables,
\beq
\mathbf D = (D_1,\cdots,D_n)
\enq
that are extracted from $x$ with the help of an array of unbiased estimators,
\beq
\mathbf {\hat D} = \bem \hat D_1,\cdots, \hat D_n \enm,\quad \av{\mathbf{\hat D}} = \mathbf D
\enq
In this multidimensional setting, all the three scalar quantities that played a role in our discussion in section \ref{single observable}, i.e. the variance of the estimator, the derivative of the observable with respect to the parameter, and the Fisher information, are now matrices.
\newline
\newline
The Fisher information $F$ in $X$ on the parameters $\boldsymbol \theta$ is defined as the square matrix
\beq \label{FisherII}
\lb F^X\lp \boldsymbol \theta \rp \rb_{\alpha\beta} = \av{ \ \frac {\partial \ln p_X}{\partial \alpha}\frac{\partial\ln p_X}{\partial \beta}}.
\enq
While the diagonal elements are identical to the information scalars in equation (\ref{FisherI}), the off diagonal ones describe correlated information.
The Fisher information matrix still carries the three properties we discussed in section \ref{Setting the scene}.
\newline
%\indent
The variance of the estimator in equation (\ref{variance}) now becomes the covariance matrix $\textrm{cov}(\mathbf {\hat D})$ of the estimators $\mathbf {\hat D}$, defined as
\beq
\textrm{cov} \lp \mathbf {\hat D} \rp _{ij} = \av{\hat D_i \hat D_j} - D_iD_j.
\enq
%\indent
Finally, the derivative of the observable with respect to the parameter, in the right hand side of (\ref{CR}), becomes a matrix $\Delta$, in general rectangular, defined as
\beq
\Delta_{\alpha \:i} = \frac{\partial D_i}{\partial \alpha},
\enq
where $\alpha$ runs over all elements of the set $\btheta$ of model parameters.
Again, the Cram\'{e}r-Rao 
 inequality provides a useful link between these three matrices, and again there are two approaches to that equation : first, as usually presented in the literature \citep{Rao}, in the form of a lower bound to the covariance matrix of the estimators,
\beq \label{CRmulti}
\textrm{cov} \left( \mathbf {\hat D} \right) \ge \Delta^T \lb  F^X\lp \boldsymbol \theta \rp \rb ^{-1}  \Delta.
\enq
The inequality between two symmetric matrices $A \ge B$ having the meaning that the matrix $A - B$ is positive definite \footnote{A matrix $A$ is called positive definite when for any vector $x$ holds that $x^TAx \ge 0$.  A concrete implication for our purposes is e.g. that the diagonal entries of the left hand side of (\ref{CRmulti}) or (\ref{covF}), which are the individual variances of each estimator $\hat D_i$, are greater than those of the right hand side.   For many more properties of positive definite matrices, see for instance \citep{Bhatia}}. If, as above, we consider the special case of identifying the parameters with the observables themselves, the matrix $\Delta$ is the identity matrix, and so we obtain that the covariance of the vector of the estimators is bounded by the inverse of the amount of Fisher information that there is on the observables in the data,
\beq \label{covF}
\textrm{cov}(\mathbf {\hat D}) \ge \lb F^X(\mathbf D)\rb^{-1}.
\enq
\newline
 Second, we can turn this lower bound on the covariance to a lower bound on the amount of information in the data set as well. By rearranging equation (\ref{CRmulti}), we obtain the multidimensional analogue of equation (\ref{CramerRao}), which describes the loss of information that occurs when the data is reduced to a set of estimators,
\beq \label{MultiCramer}
 F^X\lp \boldsymbol \theta \rp \ge \Delta \lb \textrm {cov} \lp \mathbf {\hat D }\rp\rb^{-1} \Delta^{T}.
\enq
For the sake of completeness, a proof of these two inequalities can be found in Appendix \ref{CramerRao bound}.
\newline
\newline
Instead of giving a useful lower bound to the covariance of the estimator as in equation (\ref{CRmulti}), in this form the Cram\'{e}r-Rao 
 inequality makes clear how information is in general lost when reducing the data to any particular set of estimators. The right hand side may be seen, as before, as the expected curvature of a $\chi^2$ fit to the estimates produced by the estimators $\mathbf {\hat D}$, when evaluated at the best fit value, with all correlations fully and consistently taken into account.\newline 

\noindent In the next two sections, we show how Jaynes' Maximal Entropy Principle allow us to understand the total information content of a data set, once a model is specified, in very similar terms.
%-------------------------------------------------------------------------
\subsection{Jaynes Maximal Entropy Principle}
\label{The structure of the information in a physical model}
In cosmology,  the knowledge of the probability distribution  of the data as function of the parameters, $p_X(x,\btheta)$,  which is compulsory in order to evaluate its Fisher information content, is usually very limited. In a galaxy survey, a data outcome $x$ would be typically the full set of angular positions of the galaxies, together with some redshift estimation if available, to which we may add any other kind of information, such as luminosities, shapes, etc.  Our ignorance of both initial conditions and of many relevant physical processes does not allow us to predict either galaxy positions in the sky, or all interconnections with all this additional information.  Our predictions of the shape of $p_X$ is thus limited to some statistical properties, that are sensitive to the model parameters $\btheta$, such as the mean density over some large volume, or certain types of correlation functions.\newline\newline
In fact, even if it were possible to devise some procedure in order to get the exact form of $p_X$, it may eventually turn out to be useless, or even undesirable, to do so. The incredibly large number of degrees of freedom of such a function is very likely to overwhelm the analyst with a mass of irrelevant details,  which may have no relevant significance on their own, or improve the analysis in any meaningful way.
\newline 
\newline
These arguments call for a kind a thermodynamical approach, which would try and capture those aspects of the data which are relevant to our purposes, reducing the number of degrees of freedom in a drastic way. Such an approach already exists in the field of probability theory \citep{jaynes57}. It is based on Shannon's concept of entropy of a probability distribution \citep{shannon48} and shed new light on the connection between probability theory and statistical mechanics.
\newline
\newline
As we have just argued, our predictive knowledge of $p_X(x,\btheta)$ is limited to some statistical properties. Let us formalise this mathematically, in a similar way as in section \ref{CramerRaoMulti}.  Astrophysical theory gives us a set of constraints on the shape of $p_X$, in the form of averages of some functions $o_i$,
\beq \label{constraints} 
O_i(\btheta) = \lat o_i(x) \rat (\btheta), \quad i = 1,\cdots,n.
\enq
where $p_X$ enters through the angle brackets. As an example, suppose the data outcome $x$ is a map of the matter density field as a function of position. \textbf{In this case, one of these constraints  $O_i$  could be the mean of the field or its power spectrum, as given by some cosmological model.}
\newline\newline
The role of this array $\mathbf O = (O_1,\cdots,O_n)$ is to represent faithfully the physical understanding we have of $p_X$, according to the model, as a function of the model parameters $\btheta$.  In the ideal case, some way can be devised to extract each one of these quantities $O_i$ from the data and to confront them to theory. 
\newline\newline
The set of observables $\mathbf D$, that we used in section \ref{CramerRaoMulti},  would be a subset of these predictions $\mathbf O$, and we henceforth refer to $\mathbf O $ as the 'constraints'.
%-------------------------------------------------------------------------
\subsection{Maximal entropy distributions} 
Although $p_X$ must satisfy the constraints (\ref{constraints}), there may still be a very large number of different distributions compatible with these. However, a very special status among these distributions has the one which maximises the value of Shannon's entropy\footnote{Formally, for continuous distributions the reference to another distribution is needed to render S invariant with respect to invertible transformations, leading to the concept of the entropy of $p_X$ relative to another distribution $q_X$, $S = \int dx \:p_X(x)\ln \frac {p_X(x)}{q_X(x)}$, also called Kullback-Leibler divergence. The quantity defined in the text is more precisely the entropy of $p_X(x)$ relative to a uniform probability density function. For an recent account on this, close in spirit to this work, see \cite{caticha08}.}, defined as
\beq\label{Entropy}
S = - \int dx \:p_X(x,\btheta)\ln p_X(x,\btheta).
\enq
First introduced by Shannon \citep{shannon48} as a  measure of the uncertainty in a distribution on the actual outcome, Shannon's entropy is now the cornerstone of information theory. Jaynes' Maximal Entropy Principle states that the $p_X$  for which this measure $S$ is maximal is the one that best deals with our insufficient knowledge of the distribution, and should be therefore preferred. We refer the reader to Jaynes' work \citep{jaynes83,jaynes2003} and to \cite{caticha08} for detailed discussions of the role of entropy in probability theory and for the conceptual basis of maximal entropy methods. Astronomical applications related to some extent to Jaynes's ideas include image reconstruction from noisy data, (see e.g. \citep{1984MNRAS.211..111S,1996VA.....40..563S,2004MNRAS.347..339M} and references therein) , mass profiles reconstruction from shear estimates \citep{1998MNRAS.299..895B,2002MNRAS.335.1037M}, as well as model comparison when very few data is available \citep{2007MNRAS.380..865Z}. We will see that for our purposes as well it provides us a powerful tool, and that the Maximal Entropy Principle is the ideal complement to Fisher information, fitting very well within our discussions in section \ref{Setting the scene} on the Cram\'{e}r-Rao 
 inequality.\newline
\newline
Intuitively, the entropy $S$ of $p_X$ tells us how sharply constrained the possible outcomes $x$ are, and Jaynes' Maximal Entropy Principle selects the $p_X$ which is as wide as possible, but at the same time consistent with the constraints (\ref{constraints}) that we put on it. 
The actual maximal value attained by the entropy $S$, among all the possible distributions which satisfy (\ref{constraints}), is a function of the constraints $\mathbf O$, which we denote by
\beq \label{EntropyII}
S(O_1,\cdots,O_n).
\enq
Of course it is a function of the model parameters $\btheta$ as well, since they enter the constraints.  As we will see, the shape of that surface as a function of $\mathbf O$, and thus implicitly as a function of $\btheta$, is the key point in understanding the Fisher information content of the data. In the following, in order to keep the notation simple, we will omit the dependency on $\btheta$ of most of our expressions, though it will always be implicit.
\newline
\newline
The problem of finding the distribution $p_X$ that maximises the entropy (\ref{Entropy}), while satisfying the set of constraints (\ref{constraints}), is an optimization exercise. We can quote the end result \textbf{\cite[chap. 11]{jaynes83},\cite[chap. 4]{caticha08}}: \newline
The probability density function $p_X$, when it exists, has the following exponential form,
\beq \label{MaxEnt}
p_X(x) = \frac 1 {Z} \exp\left(-\sum_{i = 1}^{n}\lambda_i o_i(x)\right),
\enq
in which to each constraint $O_i$ is associated a conjugate quantity $\lambda_i$, that arises formally as a Lagrange multiplier in this optimization problem with constraints. The conjugate variables $\lambda$'s are also called  'potentials', terminology that we will adopt in the following. We will see below in equation (\ref{potentials}) that the potentials have a clear interpretation, in the sense that the each potential $\lambda_i$ quantifies how sensitive is the entropy function $S$ in (\ref{EntropyII}) to its associated constraint $O_i$. The quantity $Z$, that plays the role of the normalisation factor, is called the partition function. Since equation (\ref{MaxEnt}) must integrate to unity, the explicit form of the partition function is 
\beq \label{partitionfunction}
Z(\lambda_1,\cdots,\lambda_n) = \int dx \: \exp\left(-\sum_{i=1}^{n}\lambda_i o_i(x)\right).
\enq
The actual values of the potentials are set by the constraints (\ref{constraints}). They reduce namely, in terms of the partition function, to a system of equations to solve for the potentials,
\beq \label{lambda}
 O_i = -\frac{\partial}{\partial \lambda_i}\ln Z,\quad i = 1,\cdots,n.
\enq
The partition function $Z$ is closely related to the entropy $S$ of $p_X$. It is simple to show that the following relation holds,
\beq \label{legendre}
S = \ln Z + \sum_{i = 1}^n \lambda_iO_i,
\enq
and the values of the potentials can be explicitly written as function of the entropy, in a relation mirroring equation (\ref{lambda}),
\beq \label{potentials}
 \lambda_i =  \frac{\partial S}{\partial O_i}, \quad i = 1,\cdots,n
\enq
Given the nomenclature, it is of no surprise that a deep analogy between this formalism and statistical physics does exist. Just as the entropy, or partition function, of a physical system determines the physics of the system, the statistical properties of these maximal entropy distributions follow from the functional form of the Shannon entropy or its partition function as a function of the constraints. For instance, the covariance matrix of the constraints is given by
\beq \label{fluctuations}
\lat \left(o_i(x) - O_i\right)\left(o_j(x) - O_j\right)\rat = \frac{\partial^2\ln Z}{\partial \lambda_i\partial\lambda_j} 
\enq
In statistical physics the constraints can be the mean energy, the volume or the mean particle number, with potentials being the temperature, the pressure and the chemical potential. We refer to \cite{jaynes57} for the connection to the physical concept of entropy in thermodynamics and statistical physics.
%-------------------------------------------------------------------------
\subsection{The structure of the information in large data sets} \label{combinations}
With our choice of probabilities $p_X$ given by equation (\ref{MaxEnt}), the amount of Fisher information on the parameters $\btheta = (\alpha,\beta,\cdots)$ of the model can be evaluated in a straightforward way. The dependence on the model goes through the constraints, or, equivalently, through their associated potentials. It holds therefore that
\beq \begin{split}
\frac{ \partial \ln p_X(x)}{\partial \alpha}& =-\frac {\partial \ln Z}{\partial \alpha} -\sum_{i= 1}^n\frac{\partial\lambda_i}{\partial \alpha} o_i(x)
\\ &= \sum_{i= 1}^n \frac{\partial\lambda_i}{\partial \alpha}\left[O_i - o_i(x)\right],
\end{split}
\enq
where the second line follows from the first after application of the chain rule and equation (\ref{lambda}).
Using the covariance matrix of the constraints given in (\ref{fluctuations}), the Fisher information matrix, defined in (\ref{FisherII}), can then be written as a double sum over the potentials,
\beq
\begin{split}\label{Zform}
F^X_{\alpha\beta} &= \sum_{i,j = 1}^n\frac{\partial\lambda_i}{\partial \alpha}\frac{\partial^2\ln Z}{\partial \lambda_i\partial\lambda_j} \frac{\partial\lambda_j}{\partial \beta}.
\end{split}
\enq
There are several ways to rewrite this expression as a function of the constraints and/or their potentials. First, it can be written as a single sum by using equation (\ref{lambda}) as
\beq \label{sumform}
F^X_{\alpha\beta} = -\sum_{i = 1}^n\frac{\partial\lambda_i}{\partial\alpha}\frac{\partial O_i}{\partial \beta}.
\enq
Alternatively, since we will be more interested in using the constraints as the main variables, and not the potentials,  we can show, using equation (\ref{potentials}), that it also takes the form \footnote{We note that this result is valid only for maximal entropy distributions and is not equivalent to the second derivative of the entropy with respect to the parameters themselves. However it is formally identical to the corresponding expression for the information content of distributions within the exponential family \citep{Jennrich75}, or \citep[chapter 4]{vandenbos07}, once the curvature of the entropy surface is identified with the generalized inverse of the covariance matrix.}
\beq \label{fishermaxent}
F^X_{\alpha\beta} = -\sum_{i,j = 1}^n\frac{\partial O_i}{\partial \alpha} \frac{\partial^2 S}{\partial O_i O_j}\frac{\partial O_j}{\partial \beta}.
\enq
We will use both of these last expressions in the following parts of this work.\newline
Equation (\ref{fishermaxent}) presents the total amount of information on the model parameters $\btheta$ in the data $X$, when the model predicts the set of constraints $O_i$. The amount of information is in the form of a sum of the information contained in each constraint, with correlations taken into account, as in the right hand side in equation (\ref{MultiCramer}). In particular, it is a property of the maximal entropy distributions, that if the constraints $O_i$ are not redundant, then it follows that the curvature matrix of the entropy surface $- \partial^2S$ is invertible and is the inverse of the covariance matrix $\partial^2 \ln Z $  between the observables. To see this explicitly,  consider the derivative of equation (\ref{lambda}) with respect to the potentials,
\beq
-\frac{\partial O_i }{\partial \lambda_j}  = \frac{\partial^2\ln Z}{\partial \lambda_i\partial\lambda_j}.
\enq
The inverse of the matrix on the left hand side, if it can be inverted, is $-\frac{\partial \lambda_i }{\partial O_j}$, which can be obtained taking the derivative of equation (\ref{potentials}), with the result
\beq
-\frac{\partial \lambda_i }{\partial O_j} =- \frac{\partial^2 S}{\partial O_i\partial O_j}.
\enq
We have thus obtained in equation (\ref{fishermaxent}), combining Jaynes' Maximal Entropy Principle together with Fisher's information, the exact expression of the Cram\'{e}r-Rao 
 inequality (\ref{MultiCramer}) for our full set of constraints,  but with an equality sign. \newline\newline
We see that the choice of maximal entropy probabilities is fair, in the sense that all the Fisher information comes from what was forced upon the probability density function, i.e. the constraints. No additional Fisher information is added when these probabilities are chosen. In fact, this requirement alone is enough to single out the maximal entropy distributions, as being precisely those for which the Cram\'{e}r-Rao 
 inequality is an equality. This can be understood in terms of sufficient statistics and goes back to \citep{1936PCPS...32..567P} and \cite{koopman36}. This was shown in \citep{RePEc:spr:metrik:v:41:y:1994:i:1:p:109-119}. We provide in appendix \ref{CramerRao bound} for completeness a similar argument that if the equality sign holds in equation (\ref{MultiCramer}) for some distribution, then it is the one that maximises the entropy relative to some other distribution. \newline\newline
In the special case that the model parameters are the constraints themselves, we have
\beq \label{entropysurface}
F^X_{O_iO_j}= - \frac{\partial^2 S}{\partial O_i O_j} = -\frac{\partial \lambda_i }{\partial O_j},
\enq
which means that the Fisher information on the model predictions contained in the expected future data is directly given by the sensitivity of their corresponding potential. Also, the application of the Cram\'{e}r-Rao 
 inequality, in the form given in equation (\ref{covF}), to any set of unbiased estimators of $\mathbf O$, shows that the best joint, unbiased, reconstruction of $\mathbf O$ is given by the inverse curvature of the entropy surface $-\partial^2S$, which is, as we have shown, $\partial^2 \ln Z$.\newline\newline
We emphasise at this point that although the amount of information is seen to be identical to the Fisher information in a Gaussian distribution of the observables with the above correlations, nowhere in our approach do we assume Gaussian properties. The distribution of the constraints $o_i(x)$ themselves is set by the  maximal entropy distribution of the data.\newline
\subsection{Redundant observables}\label{redundant}
We have just seen that in the case of independent constraints, the entropy of $p_X$ provides through equation (\ref{fishermaxent}) both the joint information content of the data, as well as the inverse correlation matrix between the observables. \textbf{However, if the constraints put on the distribution are redundant, the correlation matrix is not invertible, and the curvature of the entropy surface cannot be inverted either}. We show however that in these cases, our equations for the Fisher information content (\ref{Zform}, \ref{sumform}, \ref{fishermaxent}) are still fully consistent, dealing automatically with redundant information to provide the correct answer.\newline

\indent An example of redundant information occurs trivially if one of the functions $o_i(x)$ can be written in terms of the others. For instance, for galaxy survey data, the specification of the galaxy power spectrum as an constraint, together with the mean number of galaxy pairs as function of distance, and/or the two-points correlation function, which are three equivalent descriptions of the same statistical property of the data. Although the number of observables $\mathbf O$, and thus the number of potentials, describing the maximal entropy distribution greatly increases by doing so, it is clear that we should expect the Fisher matrix to be unchanged, by adding such superfluous pieces of information. A small calculation shows that the potentials adjust themselves so that it is actually the case, meaning that this type of redundant information is automatically discarded within this approach.  Therefore, we need not worry about the independency of the constraints when evaluating the information content of the data, which will prove convenient in some cases.\newline

\indent There is another, more relevant type of redundant information, that allow us to understand better the role of the potentials. Consider that we have some set of constraints $\{O_i\}_{i =1}^n$, and that we obtain the corresponding $p_X$ that maximises the entropy. This $p_X$ could then be used to predict the value $O_{n+1}$ of the average some other function $o_{n+1}(x)$, that is not contained in our set of predictions, 
\beq
\av{o_{n +1}(x)}  = : O_{n +1}.
\enq
For instance, the maximal entropy distribution built with constraints on the first $n$ moments of $p_X$, will predict some particular value for the $n+1$-th moment, $O_{n+1}$, that the model was unable to predict by itself.\newline
Suppose now some new theoretical work provides the shape of $O_{n+1}$ as a function of the model parameters. This new constraint can thus now be added to the previous set, and a new, updated $p_X$ is obtained by maximising the entropy. There are two possibilities at this point :
\newline
\newline \indent
It may occur that the value of $O_{n+1}$ as provided by the model is identical to the prediction by the maximal entropy distribution that was built without that constraint. Since the new constraint was automatically satisfied, the maximal entropy distribution satisfying the full set of $n +1$ constraints must be equal to the one satisfying the original set. From the equality of the two distributions, which are both of the form (\ref{MaxEnt}), it follows that the additional constraint must have vanishing associated potential,
\beq
\lambda_{n+1} = 0,
\enq
while the other potentials are pairwise identical. It follows immediately that the total information, as seen from equation (\ref{sumform}) is unaffected, and no information on the model parameters was gained by this additional prediction.
A cosmological example would be to enforce on the distribution of some field, together with the two-points correlation function, fully disconnected higher order correlation functions. It is well known that the maximal entropy distribution with constrained two-points correlation function has a Gaussian shape, and that Gaussian distributions have disconnected points function at any order. No information is thus provided by these field moments of higher order in this case.\newline
This argument shows that, for a given set of original constraints and associated maximal entropy distribution, any function $f(x)$, which was not contained in this set, with average $F$, can be seen as being set to zero potential. Such $F$'s therefore do not contribute to the information.
\newline\newline\indent
More interesting is, of course, the case where this additional constraint differs from the predictions obtained from the original set $\left\{O_i\right\}_{i = 1}^n$. Suppose that there is a mismatch $\delta O_{n+1}$ between the predictions of the maximal entropy distribution and the model. In this case, when updating $p_X$ to include this constraint, the potentials are changed by this new information, a change given to first order by
\beq
\delta\lambda_i = \frac{\partial^2S}{\partial O_i \partial O_{n+1}}\delta O_{n+1}, \quad  i = 1,\cdots, n+1,
\enq
and the amount of Fisher information changes accordingly.
%It is interesting to note that the entropy itself is invariant at this order. From equation (\ref{potentials}) we have namely
%\beq
%\delta S = \sum_{i = 1}^{n+1} \lambda_{i}\:\delta O_i =  \lambda_{n + 1}\delta O_{n+1} = 0,
%\enq
%since the new constraint was originally at zero potential.
%The entropy is, therefore, stationary not only with respect to changes in the probability distribution function, but also with respect to the predictions its associated maximal entropy distribution makes on any other quantities.
\newline\newline
Of course, although the formulae of this section are valid for any model, it requires numerical work in order to get the partition function and/or the entropy surface in a general situation.
%-------------------------------------------------------------------------
\subsection{The entropy and Fisher information content of Gaussian homogeneous fields} \label{Examples}
In order to close this section, we obtain now the Shannon entropy of a family of fields when only the two-point correlation function is the relevant constraint, that we will use extensively in the next section dealing with our cosmological application. It is easily obtained by a straightforward generalisation of the finite dimensional multivariate case, where the means and covariance matrix of the variables are known. It is well known  \citep{shannon48}  that the maximal entropy distribution is in this case the multivariate Gaussian distribution. Denoting the constraints on $p_X$ with the matrix $D$ and vector $\boldsymbol \mu$
\beq \label{cov} \begin{split}
D_{ij} &=  \av{x_{i}x_{j}} \\
\mu_i &= \av{x_i}, \quad i,j = 1,\cdots,N
\end{split}
\enq
the associated potentials are given explicitly by the relations
\beq \begin{split} \label{Dm}
 \lambda &= \frac 12 C^{-1}
\\\eta &= - C^{-1}\bmu,
\end{split}
\enq
where the matrix $C$ is the covariance matrix
\beq
C := D - \bmu \bmu^T.
\enq
The Shannon entropy is given by, up to some irrelevant additive constant,
\beq \label{entropyG}
S(D,\bmu) = \frac 12 \ln \det (D -  \bmu \bmu^T).
\enq
The fact that about half of the constraints are redundant, due to the symmetry of the $D$ and $C$ matrices, is reflected by the fact that the corresponding inverse correlation matrix in equation (\ref{fishermaxent}),
\beq
-\frac{\partial^2 S}{\partial D_{ij}\partial D_{kl}} = - \frac{\partial \lambda_{ij}}{\partial D_{kl}} =  \frac 12  C\inv_{ik}C\inv_{jl},
\enq
is not invertible as such if we considers all entries of the matrix $D$ as constraints. Of course,  this is not the case anymore if only the independent entries of $D$ form the constraints.  
\subsubsection{Fields, means and correlations}
\newcommand{\bbphi}{\bar\bphi}
Using  the handy formalism of functional calculus, we can straightforwardly extend the above relations to systems with infinite degrees of freedom, i.e. fields, where means as well as the two-point correlation functions are constrained. A realisation of the variable $X$ is now a field, or a family of fields $\bphi = (\phi_1,\cdots,\phi_N)$, taking values on some $n$-dimensional space.  The expressions above in the multivariate case all stays valid, with the understanding that operations such as matrix multiplications have to be taken with respect to the discrete indices as well as the continuous ones.\newline\newline
With the two-point correlation function and means
\beq
\begin{split}
\rho_{ij}(\vecx,\vecy) &= \av{\phi_i(\vecx)\phi_j(\vecy)} \\
\bar\phi_i(\vecx) &= \av{\phi_i(\vecx)}
\end{split}
\enq
we still have, up to an unimportant constant,
\beq \label{entropyfield}
S = \frac 12 \ln \det (\rho - \bphi\bphi^T). 
\enq
\newline\newline
In n-dimensional Euclidean space, within a box of volume $V$ for a family of homogeneous fields, it is simplest to work with the spectral matrices. These are defined as
\beq \label{spectralmatrix}
\frac 1 V \lat \tilde\phi_i(\veck) \tilde\phi_j^*(\veck')\rat =  P_{ij}(\veck)\:\delta_{\veck\veck'},
\enq
where the Fourier transforms of the fields are defined through
\beq
\tilde\phi_i(\veck) = \int_V d^nx \: \phi_i(x)\:e^{-i\veck\cdot\vecx}.
\enq
It is well known that these matrices provide an equivalent description of the correlations, since the they form Fourier pairs with the correlation functions
\beq
\rho_{ij}(\vecx,\vecy) = \frac 1 V \sum_{\veck} P_{ij}(\veck) e^{i\veck \cdot (\vecx - \vecy)} = \rho_{ij}(\vecx -\vecy).
\enq
In this case, the entropy in equation (\ref{entropyfield}) reduces, again discarding irrelevant constants, to an uncorrelated sum over the modes,
\beq \label{entropy field}
S = \frac 12 \ln\det\left[ \frac {P(0)}{V} - \bar\phi\bar\phi^T \right]+ \frac 12\sum_{\veck}\ln \det \frac{ P(\veck) }{V},
\enq
which is the straightforward mutlidimensional version of \citep[eq. 39]{2001MNRAS.328.1027T}.
Comparison with equation (\ref{entropyG}) shows the well-known fact that the modes can be seen as Gaussian, uncorrelated and complex variables with correlation matrices proportional to $P(\veck)$.  All modes have zero mean, except for the zero-mode, which, as seen from its definition, is proportional to the mean of the field itself. Accordingly, taking the appropriate derivatives, the potentials $\lambda(\veck)$ associated to $P(\veck) $ read
\beq
\begin{split} 
\lambda(\veck) &= \frac V{2} P(\veck) ^{-1},\quad \veck \ne 0 \\
\lambda(0) &=  \frac 1{2} \lb  \frac{P(0)}{V} - \bphi\bphi^T \rb^{-1} . 
\end{split}
\enq
and those associated to the means $\bphi$,
\beq
\boldsymbol \eta = - \lb  \frac{P(0)}{V} - \bphi\bphi^T \rb^{-1}\bphi
\enq
Note that although the spectral matrices are, in general, complex, they are hermitian, so that the determinants are real. The amount of Fisher information in the family of fields is easily obtained with the help of equation (\ref{sumform}) , with the familiar result
\beq \label{FPk} \begin{split}
\Fab &= \frac 1 2\sum_{\veck } \Tr\left[P_c^{-1}(\veck)\frac{\partial P_c(\veck)}{\partial \alpha}P_c^{-1}(\veck)\frac{\partial P_c(\veck)}{\partial \beta}\right]\\
&\quad+ \frac{\partial \bbphi^T}{\partial \alpha}\lb \frac{P_c(0)}{V}\rb^{-1} \frac{\partial\bbphi}{\partial \beta},
\end{split}
\enq
with $P_c(\veck)$ being the connected part of the spectral matrices,
\beq
\begin{split}
P_c(\veck) &= P(\veck) - \delta_{\veck0}V\bphi\bphi^T.
\end{split}
\enq
These expressions are of course also valid for isotropic fields on the sphere. With a decomposition in spherical harmonics, the sum runs over the multipoles.
%--------------------------------------------------------------------------------
%--------------------------------------------------------------------------------
%\color{red}
\section{Cosmological application to weak lensing observables} \label{application}
Gravitational lensing, which can be used to measure the distribution of mass along the line of sight, has been recognized as powerful probe of the dark components of the Universe \citep{1992grle.book.....S,2001PhR...340..291B,2003ARA&A..41..645R,2006astro.ph.12667M,2006glsw.book.....S} since it is  sensitive to both the geometry of the Universe, and to the growth of structure. Weak lensing data is typically used in two ways. The first, which is deployed for cosmological parameter fitting, relies on measuring the correlated distortions in galaxy images \citep{2006astro.ph..9591A}. The second approach uses each galaxy to make a noisy measurement of the lensing signal at that position. These point estimates are then used to reconstruct the dark matter density distribution \citep[e.g.][]{1993ApJ...404..441K,2001A&A...374..740S}. Most of the measurements of weak lensing to date have focused on the shearing that galaxy images experience. However, gravitational lensing causes a number of other distortions of galaxy images. These include change in size, which is related to the magnification, and higher order image distortions known as the flexion \citep{2006MNRAS.365..414B}. A number of techniques have been developed for measuring these higher order images distortions, such as HOLICS \citep{2007ApJ...660..995O} and shapelets methods \citep{2007MNRAS.380..229M}. Since all of the image distortions originate from the same cause, i.e. the lensing potential field, the information content of any two lensing measurements must be degenerate. At the same time, since each method has different systematics and specific noise properties, combining multiple measurement can may bring substantial benefits. Some recent works have looked at the impact of combining shear and flexion measurements for mass reconstruction \citep{2010arXiv1008.3088E,2010ApJ...723.1507P,2010arXiv1011.3041V}, as well as the benefits for breaking multiplicative bias of including galaxy size measurements  \citep{2010arXiv1009.5590V}.
\black
%\indent In the following we will focus on tracers of galaxy image distortions up to second order in the distortions. These include, to first order, the change in apparent size of the galaxies, due to the magnification source by the convergence field, the two components of the shear, and, to second order, the four components of the two flexion fields. We will limit ourselves to the case where the noise contaminating each probe can be effectively treated as independent of the model parameters. The common point of the probes cited above is that they all trace, in some noisy way, the same central field on a discrete set of points, represented by the  positions of the galaxies on which the tracers are measured. The framework we presented in the last section is ideal to deal with the special structure of the situation. We will first show how we can understand the total information content of such degenerate probes of a central field in a general situation, and then make quantitative evaluations at the two-point level. 
%\color{black}
%--------------------------------------------------------------------------------
%--------------------------------------------------------------------------------
\subsection{Linear probes}
%The situation that we consider here is one where a broad number of observables are linked in some way to a central field. We will limit ourselves to the case where the noise contaminating each probe can be effectively treated as independent of the model parameters.  
%Imagine one plans to perform different measurements, of observables that are all linked in some way or another to the same central field, which is the actually interesting quantity from the point of view of the analyst. 
%The most straightforward example of such a situation, which is the one we will explore in more details later, occurs when the two point correlations of the central field, say the the power spectrum of the convergence in weak lensing, is predicted from theory, while we try to extract it looking at the correlations of the two ellipticity components of galaxies. In this case, predictive power of the power spectrum of the convergence turns into predictive power of (parts of) the three correlation functions there are between the two ellipticity components.
%\newline\newline
The predictive power of some observable  $O_c$ of a central field (for instance its power spectrum at some mode)  translates into an array of constraints $O_i,\:\: i = 1,\cdots,n$ in the noisy probes, that we could try and extract and confront to theory :
\beq
\begin{split}\label{assum}
O_i(\btheta) = f_i(O_c(\btheta)), \quad i = 1,\cdots, n
\end{split}
\enq
for some functions $f_i$.\newline
For the purpose of this work,  the case of functions linear with respect to $O_c$ is generic enough, i.e. we will consider that
\beq
\frac{\partial^2 f_i}{\partial O_c^2} = 0,\quad i = 1,\cdots,n.
\enq
The entropy $S$ of the data is a function of the $n$ constraints $\mathbf O$. It is however fundamentally a function of $O_c$ since it does enter all of these observables. It is therefore very natural to associate a potential $\lambda_c$ to $O_c$, although it is not itself a constraint on the probability density function. In analogy with
\beq
\lambda_i =  \frac{\partial S}{\partial O_i}, \quad i = 1,\cdots,n
\enq
we define
\beq
\lambda_c := \frac{d S}{dO_c}(O_1,\cdots,O_m),
\enq
with the result, given by application of the chain rule, of
\beq  \label{un}
\lambda_c = \boldsymbol \lambda \cdot \frac{\partial \mathbf f}{\partial O_c}.
\enq
On the other hand, the impact of a model parameter on each observables can be similarly written in terms of the central observable $O_c$,
\beq \label{deux}
\frac{\partial \mathbf O}{\partial \alpha} = \frac{\partial O_c}{\partial \alpha} \frac{\partial \mathbf f}{\partial O_c} .
\enq
It follows directly from these relations (\ref{un}) and (\ref{deux}), and the linearity of $f_i$, that the joint information in the full set of constraints $\mathbf O$, given in equation (\ref{sumform}) as a sum over all $n$ constraints, reduces to a formally identical expression with the only difference that only $O_c$ enters :
\beq
\Fab^X = \frac{\partial \mathbf O}{\partial \alpha }\cdot \frac{\partial \boldsymbol \lambda}{ \partial \beta} = \frac{\partial \lambda_c}{\partial \alpha}\frac{\partial O_c}{\partial \beta},
\enq
which can also be written in the form analog to (\ref{fishermaxent}),
\beq  \label{infreduction}
\Fab^X =  -\frac{\partial O_c}{\partial \alpha}\frac{d^2 S}{dO_c^2} \frac{\partial O_c}{\partial \beta}.
\enq
This last equation shows that all the effect of combining this set of constraints have been absorbed into the second total derivative of the entropy. This second total derivative is the total amount of information there is on the central quantity $O_c$ in the data. Indeed, taking as a special case of model parameter to the central quantity itself, i.e. 
\beq
\alpha =  \beta =  O_c, 
\enq
one obtains now that the full amount of information in $X$ on $O_c$ is 
\beq \label{Infcentr}
F^X_{O_cO_c} = -\frac{d^2 S}{d O_c^2}\lp O_1,\cdots,O_n \rp \equiv \frac{1}{\sigma^2_{\eff}}.
\enq
A simple application of the Cramer Rao inequality presented in equation (\ref{CramerRao}) shows that this effective variance $\sigma_{\eff}$ is the lower bound to an unbiased reconstruction of the central observable from the noisy probes. \newline\newline
These considerations on the effect of probe combination in the case of a single central field observable $O_c$ generalize easily to the case where there are many, $(O_c^1,\cdots, O_c^m)$. In this case, each central field quantity leads to an array of constraints in the form of equation (\ref{assum}), it is simple to show that the amount of Fisher information can again be written in terms of the information associated to the central field, with an effective covariance matrix between the $O_c's$. The result is
\beq
\Fab^X = -\sum_{i,j = 1}^{m}\frac{\partial O_c^i}{\partial \alpha}\frac{d^2S}{dO_c^iO_c^j}\frac{\partial O_c^j}{\partial \beta}.
\enq
All the effects of probe combination are thus encompassed in  an effective covariance matrix $\Sigma_\eff$ of the central field observables,
\beq
-\frac{d^2S}{dO_c^iO_c^j} \equiv \lb \Sigma^{-1}_\eff\rb_{ij}.
\enq
Again, an application of the Cramer Rao inequality, in the multi-dimensional case, shows that this effective covariance matrix is the best achievable unbiased joint reconstruction of  $(O_c^1,\cdots, O_c^m)$.
\newline\newline
We now explore further the case of linear probes of homogeneous Gaussian fields, which is cosmologically relevant and can be solved analytically to full extent. We will focus on zero mean fields,  for which according to our previous section the entropy can be written in terms of the spectral matrices, up to a constant,
\beq \label{EntropyField}
S = \frac 12 \sum_{\veck} \ln \det P(\veck).
\enq
\color{black}
%-------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------
\subsection{Linear tracers at the two-point level}
A standard instance of a linear tracer $\phi_i$ of some central field $\kappa$ in weak lensing is provided by a relation in Fourier space of the form
\beq \label{example}
\tilde \phi_i(\veck) = v_i \tilde \kappa(\veck) +\tilde \epsilon_i(\veck),
\enq
for some noise term $\tilde\epsilon_i$, uncorrelated with $\kappa$, and coefficient $v_i$. \textbf{Typically, if one observes a tracer of the derivative of the field $\kappa$, then the vector $\vecv$ would be proportional to $-i\veck$. We are ignoring here any observational effect, such as incomplete sky coverage, that would require corrections to this relation.}  It is clear from this relation that the spectral matrices of this family take a special form of equation (\ref{assum}): defining the spectrum of the $\kappa$ field by $P^\kappa$, we obtain by putting this relation (\ref{example}) into (\ref{spectralmatrix}), that the spectral matrices can be written at each mode in the form
\beq \label{specmatrix}
P =  P^\kappa \vecv\vecv^\dagger + N,
\enq
where $\vecv^\dagger$ is the hermitian conjugate of $\vecv = \lp v_1,\cdots,v_n\rp$. The matrix $N$ is the spectrum of the noise components $\epsilon$,
\beq
N_{ij}(\veck) = \frac 1 V\av{\tilde \epsilon_i(\veck)\tilde \epsilon^*(\veck)}.
\enq 
Our subsequent results hold for any family of tracers that obey this relation. While the special case in (\ref{example}) enter this category, this need not be the only instance. All the weak lensing observables we deal with in this work will satisfy equation (\ref{specmatrix}).
\newline\newline
Both the n-dimensional vector $\vecv$ and the noise matrix $N$ can depend on the wave vector $\veck$, but they are independent from the model parameters. The  matrix $N$ of dimension $n\times n$ is the noise component of the spectra of the fields, typically built from two parts. The first is due to the discrete nature of the fields, since such data consist in quantities measured where galaxies sits, and the second to the intrinsic dispersion of the measured values.
\subsection{Joint entropy and information content}
\indent Information on the model parameters enters through $P^\kappa$ only.
To evaluate the full information content, we need only evaluate eq. (\ref{EntropyField}) with the spectral matrix given in (\ref{specmatrix}), keeping in mind the result from last section, that we need only the total derivative with respect to $P^\kappa$. In other words, any additive terms in the expression of the entropy that are independent of $P^\kappa$ can be discarded.
\newline\newline
This determinant can be evaluated immediately. Defining for each mode the real positive number $N_\eff$ through
\beq \label{noise}
\frac 1 {N_\eff} \equiv \vecv^\dagger N^{-1}\vecv,
\enq
which can be seen as an effective noise term, a simple\footnote{We have namely for any invertible matrix $A$ and vectors $\vecu,\vecv$ the matrix determinant lemma,
\beq
\det \left(A + \vecu \vecv^T\right) = \det\lp A\rp \lp 1 + \vecv^TA^{-1}\vecu \rp. 
\enq}  calculation shows that the joint entropy (\ref{EntropyField}) is equivalent to the following, where the $n$ dimensional determinant has disappeared,
\beq \label{Entropy2}
S = \frac12\sum_{\veck}\ln \left(P^\kappa(\veck)  +  N_\eff(\veck)\right).
\enq
Comparison with equation (\ref{EntropyField}) shows that we have with this equation (\ref{Entropy2}) the entropy of the field $\kappa$ itself, where all the effects of the joint observation of this $n$ fields have been absorbed into the effective noise term $N_\eff$, that contaminates its spectrum. It means that the full combined information in the $n$ probes of the field $\kappa$ is equivalent to the information in $\kappa$, observed with spectral noise $N_\eff$.\newline\newline
Our result (\ref{Infcentr}) applied to (\ref{Entropy2}) puts  bounds on reconstruction of the field $\kappa$ out of the observed samples, which can be at best reconstructed with a contaminating noise term of $N_\eff$ in its spectrum, whose best unbiased reconstruction is given by
\beq
 2\lp P^\kappa(\veck) +N_\eff(\veck)\rp^2.
\enq
\newline
Since the effect of combining these probes at a single mode is only to change the model independent noise term, the parameter correlations and degenaracies as approximated by the Fisher information matrix stay unchanged, whatever the number of such probes is. We have namely from (\ref{Entropy2}) that at a given mode $\veck$, the Fisher information matrix reads
\beq \label{fmatrixpk}
\Fab^X = \frac 12 \frac{\partial \ln \tilde P^\kappa(\veck) }{\partial\alpha}\frac{\partial \ln \tilde P^\kappa(\veck)}{\partial\beta},
\enq
with
\beq
 \tilde P^\kappa(\veck) =  P^\kappa(\veck)  + N_\eff(\veck).
\enq
\textbf{From the point of view of the Fisher information, it makes formally no difference to extract the full set of $n(n-1)/2$ independent elements of each spectral matrices, or reconstruct the field $\kappa$ and extract its spectrum. They carry indeed the same amount of Fisher information.
\newline\newline
These results still hold when other fields are present in the analysis, which are correlated 
with the field $\kappa$. To make this statement rigorous, consider in the analysis on top of our $n$ samples of the form (\ref{example}) of $\kappa$, another homogeneous field $\theta$, with spectrum $P^\theta(\veck)$, and cross spectrum to $\kappa$ given by $P^{\theta\kappa}(\veck)$ The full spectral matrices are in this case
\beq
P(\veck) = \bem P^\kappa(\veck) \vecv\vecv^T + N  & P(\veck)^{\kappa\theta}\vecv 
\\ P^{\theta\kappa}\vecv^T & P^{\theta}(\veck) \enm.
\enq
Again, the determinant of this matrix can be reduced to a determinant of lower 
dimension, leading to the equivalent entropy
\beq \label{multis}
S = \cst + \frac 12 \ln \det \bem P^\psi(\veck) + N_\eff & P^{\kappa\theta}
(\veck) \\ P^{\theta\kappa}(\veck) & P^\theta(\veck) \enm.
\enq
It shows that the the full set of $n + 1$ 
fields can be reduced without loss to two fields, $\kappa$ and 
$\theta$, with the effective noise $N_\eff$ contaminating the spectrum of $\kappa$. }\newline\newline
Note that the derivation of our results do not refer to any hypothetical estimators, but 
came naturally out of the expression of the entropy.
%----------------------------------------------------------------
%----------------------------------------------------------------
\subsection{Weak lensing probes}
We now seek a quantitative evaluation of the full joint information content of the weak lensing probes in galaxy surveys, up to second order in the image distortions of galaxies. The data $X$ consists of a set of fields, which are discrete point fields, which take values where galaxies sits. We work in the two-dimensional flat sky limit, using the more standard notation $\mathbf l$ for the wave vector, and decompose it in modulus and polar coordinate as
\beq
\vecl = l\bem \cos \varphi_l \\ \sin \varphi_l \enm
\enq
For the scope of this paper, we will throughout assume that the intrinsic values of each probe are pairwise uncorrelated, as commonly done. Also, we will assume that the set of points on which the relevant quantities are measured show low enough clustering so that corrections to the spectra due to intrinsic clustering can be neglected. This is however not a limitation of our approach, since corrections to the above assumptions, such as the introduction of some level of intrinsic alignment, can be accommodated for by introducing appropriate terms in the noise matrices $N(\veck)$ in (\ref{noise}). 
As a central field to which all our point fields relates, we take for convenience the isotropic convergence field $\kappa$, with spectrum
\beq
C^\kappa(\vecl) = C^\kappa(l).
\enq
In the case of pairwise uncorrelated intrinsic values that we are following, we see easily from (\ref{noise}) that by combining any number of such probes the effective noise is reduced at a given mode according to
\beq \label{combination}
\frac 1 {N^{\textrm{tot}}_\eff} = \sum_i \frac{1}{N_\eff^i}.
\enq
We therefore only need to evaluate the effective noise for each probe separately, while their combination follows (\ref{combination}). To this aim, the evaluation of the spectral matrices (\ref{specmatrix}), giving us $N_\eff$, is necessary. The calculations for this are presented in appendix \ref{pf} and we use the final results in this section.
\subsubsection{First order, distortion matrix}
To first order, the distortion induced by weak lensing on a galaxy image is described by the distortion matrix that contains the shear, $\gamma$, and convergence, $\kappa$, which come from the second derivatives of the lensing potential field $\psi$, \citep[e.g. ][]{2006glsw.book.....S}
\beq \label{distortion}
\bem \kappa + \gamma_1 & \gamma_2 \\ \gamma_2 & \kappa - \gamma_1 \enm = \psi_{,ij}.
\enq
The shear components read
\beq
\gamma_1 = \frac 12 \left(\psi_{,11} - \psi_{,22}\right), \quad \gamma_2 = \psi_{,12}
\enq
and we assume they are measured from the apparent ellipticities of the galaxies, with identical intrinsic dispersion $\sigma^2_\gamma$. Denoting with $\bar n_\gamma$ the number density of galaxies for which ellipticity measurements are available,
the effective noise is 
\beq \label{neffgamma}
N^\gamma_\eff = \frac{\sigma^2_\gamma}{\bar n_\gamma}.
\enq
The information content of the two observed ellipticity fields is thus exactly the same as the one of the convergence field, with a mode independent noise term as above. 
\newline\newline
\newcommand{\intr}{\textrm{int}}
\textbf{To reach for the $\kappa$ component of the distortion matrix, we imagine we have measurements of their angular size $s_\obs$, with intrinsic dispersion $\sigma^2_s$. The intrinsic sizes of the galaxies $s_\intr$ gets transformed through weak lensing according to}
\beq
s_\obs = s_{\textrm{int}}( 1 +\alpha_s\kappa).
\enq 
The coefficient $\alpha_s$, is equal to unity in pure weak lensing theory, but we allow it to take other values, since in a realistic situation, other effects such as magnification bias effectively enter this coefficient (e.g. \citep{2010arXiv1009.5590V}). Under our assumption that the correlation of the fluctuations in intrinsic sizes can themselves be neglected, the effective noise reduces to
\beq\label{neffsize}
 N^s_\eff =  \frac 1 {\alpha_s^2}\lp \frac{\sigma_s} { \bar s_\textrm{int}} \rp ^2\frac{1}{\bar n_s}.
\enq
This combination of $\alpha_s$ with the dispersion parameters $\bar s$ and $\sigma_s$ becomes the only relevant parameter in our case, and not the value of each of them.
\subsubsection{Second order, flexion}
To second order, the distortions caused by lensing on the galaxies images are given by third order derivatives of the lensing potential. These are conveniently described by the spin 1 and spin 3 flexion components $\mathcal F$ and $\mathcal G$, which in the notation of  \citep{2008A&A...485..363S} read
\beq \begin{split}
\mathcal F &= \frac 12 \bem \psi_{,111} + \psi_{,122} \\ \psi_{,112} + \psi_{,222} \enm 
\\
\mathcal G &= \frac 12 \bem \psi_{,111} - 3\psi_{,122} \\ 3\psi_{,112} - \psi_{,222} \enm,
\end{split}
\enq
and are extracted from measurements with intrinsic dispersion $\sigma^2_\mathcal F$ and $\sigma^2_\mathcal G$.
The effective noise is this time mode-dependent,
\beq \label{neffflex}
\frac 1 { N^{\mathcal F \mathcal G}_\eff} = l^2\left(\frac{\bar n_F}{\sigma_F^2} + \frac{\bar n_G}{\sigma_G^2}\right).
\enq
%------------------------------------------------
\section{Results} \label{results}
Figure \ref{noiseratio} shows the ratio of the effective noise to the noise present considering the shear fields only, assuming the same number densities of galaxies for each probe, and the values for the intrinsic dispersion stated in table \ref{paramtable}. The conversion multipole $l$ (upper x-axis) to angular scale $\theta$ (lower x-axis) follows $\theta = \pi / (l + 1/2)$.  We have adopted for the size dispersion parameters the numbers from \citep{2010arXiv1009.5590V}, who evaluated this number for the DES survey conditions \citep{2005astro.ph.10346T}. 
\textbf{We refer to the discussion in \citep{2010ApJ...723.1507P} for our choice of flexion dispersion parameters.}
The curves on this figure are rations and therefore independent of the galaxy number density. They are redshift independent as well, only to the extent that the dispersion in intrinsic values can be treated as such. We can draw two main conclusions from figure \ref{noiseratio}. First, flexion information beings to play role only at the smallest scales, on the arcsecond scales, where it takes over and becomes the most interesting probe. On the scale of $1$ amin, it can bring substantial improvement over shear only analysis, but only in combination with the shears, and not on its own. This is in good agreement with the comparative analysis of the power of the flexion $\mathcal F$ field and shears fields for mass reconstruction done in \cite{2010ApJ...723.1507P}, restricted to direct inversion methods. Second, the inclusion of size of galaxies into the analysis provides a density independent, scale independent, improvement factor of
\beq \label{improve}
\frac{N_\eff^\gamma}{N_\eff^{\gamma+ s}} = 1 + \lp \frac{\sigma_\gamma \bar s}{\sigma_s \alpha_s}\rp^2,
\enq
which is close to a $10\%$ improvement for the quoted numbers. Of course, the precise value depends on the dispersion parameters of the population considered.
\begin{center}
\begin{table} \caption{Dispersion parameters used in figure \ref{noiseratio}.}\label{paramtable}
\begin{tabular*}{0.3\textwidth}{cccc} 
 $\sigma_\gamma$ & $ \sigma_\mathcal F$ asec$^{-1}$ &$ \sigma_\mathcal G $ asec$^{-1}$ &  $\frac 1 {\alpha_s} \frac{ \sigma_s}{ \bar s}$ \\ \hline
 0.25 & 0.04 & 0.04 & 0.9 
 \end{tabular*}
\end{table}
\end{center}
\begin{center}
\begin{figure} 
  \includegraphics[width = \textwidth]{figs/NoiseRatio}
  \caption{The ratio of the effective noise to the level of noise considering the shears only, as function of angular scale. The dashed line considers the flexion fields alone. The dotted line shows the combination of the flexion fields with the shear fields,  and the solid line all these weak lensing probes combined. No correlations between the intrinsic values for each pair of probes have been considered.}
  \label{noiseratio}
\end{figure}
\end{center}
For the purpose of measuring cosmological parameters rather than mass reconstruction, more interesting are the actual values of the Fisher information matrices. Since with any combination of such probes, these matrices are proportional to each other at a single mode, it makes sense to define the efficiency parameter of the probe $i$ through
\beq
\epsilon_i(l) := \frac{C^\kappa(l)}{C^\kappa(l) + N^i_\eff(l)},
\enq
which is a measure of what fraction of the information contained in the convergence field is effectively catched by that probe. The information in the convergence field is, at a given mode $l$, counting the multiplicity of the mode,
\beq
F^\kappa_{\alpha\beta} = \frac 12 (2l + 1) \frac{\partial \ln C^\kappa(l)}{\partial\alpha}\frac{\partial \ln C^\kappa(l)}{\partial\beta},
\enq
and we have indeed that the total Fisher information in the observed fields is
\beq
\Fab^X = \sum_l  F^\kappa_{\alpha\beta}(l) \epsilon^2_i(l).
\enq
Therefore, according to the interpretation of the Fisher matrix approximating the expected constraints on the model parameters, the factor $\epsilon(l)$ is precisely equal to the factor of degradation in the constraints one would be able to put on any a parameter, with respect to the case of perfect knowledge of the convergence field at this mode.
It is not the purpose of this work to perform a very detailed study on the behavior of the efficiency parameter for some specific survey and the subsequent statistical gain, but its qualitative behavior is easy to see. This parameter is essentially unity in the high signal to noise regime, while it is the inverse effective noise whenever the intrinsic dispersion dominates the observed spectrum. Since information on cosmological parameters is beaten down by cosmic variance in the former case, the latter dominates the constraints. We can therefore expect from our above discussion the size information to tighten by a few percent constraints on any  cosmological parameter. On the other hand, while flexion becomes ideal for mass reconstruction purposes on small scales, it will be able to help inference on cosmological parameters only if the challenge of  very accurate theoretical predictions on the convergence power spectrum for multipoles substantially larger than $1000$ will be met.\newline\newline
To make these expectations more concrete, we evaluated the improvement in information on cosmological parameters performing a lensing Fisher matrix calculation for a wide, EUCLID-like survey, in a tomographic setting. For a data vector consisting of $n$ probes of the convergence field $\kappa_i$ in each redshift bin $i,\: i = 1,\cdots N$, it is simple to see following our previous argument, that the Fisher information reduces to
\beq
F_{\alpha\beta} = \frac 12  \sum_{l}\lp 2l + 1\rp \Tr \:C^{-1}\frac{\partial C}{\partial\alpha} C^{-1}\frac{\partial C}{\partial\beta},
\enq
where the $C$ matrix is given by
\beq \label{cmatrix}
C_{ij} = C^{\kappa_i \kappa_j}(l)  + \delta_{ij}N^i_\eff(l),\quad i,j = 1,N
\enq
with $N_\eff^i$ given by (\ref{noise}). The only difference between standard implementations of Fisher matrices for lensing, such as the lensing part of \cite{2004PhRvD..70d3009H}, being thus the form of the noise component.
we evaluated these matrices respectively for
\beq \label{shearonly}
N_\eff^i = \frac{\sigma^2_\gamma}{\bar n^i} = N^{\gamma,i}_\eff ,
\enq
which is the precise form of the Fisher matrix for shear analysis, for
\beq\label{shearsize}
\frac{1}{N_\eff^i} =\frac 1 {N_\eff^{\gamma,i}} + \frac 1 {N_\eff^{s,i}}
\enq
which account for size information, and
\beq\label{shearsizefg}
\frac{1}{N^i_\eff(l)} = \frac 1 {N_\eff^{\gamma,i}} + \frac 1 {N_\eff^{s,i}} + \frac 1 {N_\eff^{\mathcal F \mathcal G,i}(l)} ,
\enq
which accounts for the flexion fields as well.  We note that in terms of observables, these small modifications incorporate in its entirety the full set of all possible correlations between the fields considered. The values of the dispersion parameters involved in these formulae are the same as in table (\ref{paramtable}). Our fiducial model is a flat $\Lambda$CDM universe, with parameters $\Omega_\Lambda = 0.7$, $\Omega_b = 0.045$, $\Omega_m = 0.3, h = 0.7$, power spectrum parameters $\sigma_8 = 0.8, n = 1$, and Linder's parametrisation \citep{2003PhRvL..90i1301L} of the dark energy equation of state implemented as $\omega_0 = -1,w_a = 0$. The distribution of galaxies as function of redshift needed both for the calculation of the spectra and to obtain the galaxy densities in each bin was generated using the cosmological package iCosmo \citep{2008arXiv0810.1285R}, in a way described in \citep{2007MNRAS.381.1018A}. We adopted EUCLID-like parameters of $10$ redshift bins, a median redshift of $1$, a galaxy angular density of $40 / \textrm{amin}^2$, and photometric redshift errors of $0.03(1 + z)$.
\newline\newline
In figure \ref{figFOM}, we show the improvement in the dark energy Figure of Merit (FOM), defined as the square root of the determinant of the submatrix $\lp \omega_0,\omega_a\rp$ of the Fisher matrix inverse $F^{-1}_{\alpha\beta}$ ($\alpha$ and $\beta$ running over the set of eight parameters as described above), as function of the maximal angular mode $l_\max$ considered, while $l_\min$ being always taken to be 10. In perfect agreement with our discussion above, including size information (solid line) increases the FOM steadily until it saturates at a $10\%$ improvement when constraints on the dark energy parameters are dominated by the low signal to noise regime. Also, flexion becomes only useful in the deep non-linear regime, where however theoretical understanding of the shape of the spectra still leaves a lot to be desired.
\newline\newline
These results are found to be very insensitive to the survey parameters, for a fixed $\alpha_s$.  There are also only weakly model parameter independent, as illustrated in table \ref{ratiotable}, which shows the corresponding improvement in Fisher constraints,
\beq
\frac{\sigma^2}{\sigma^2_{\textrm{shear only}}} = \frac{F^{-1}_{\alpha\alpha}}{F^{-1}_{\alpha\alpha, \textrm{shear only}}},
\enq
at the saturation scale $l_\max = 10^4$.
These results are also essentially unchanged using either standard implementations of the halo model \citep[for a review]{2002PhR...372....1C} or the the HALOFIT \citep{2003MNRAS.341.1311S} non linear power spectrum.
\begin{center}
\begin{figure} 
  \includegraphics[width = \textwidth]{figs/Fom}
  \caption{The improvement of the dark energy FOM including size information (solid), as well as flexion $\mathcal F$ and $\mathcal G$ information (dotted), over the shear only analysis, as function of the maximal angular multipole included in the analysis.}
  \label{figFOM}
\end{figure}
\end{center}
\begin{center}
\begin{table} \caption{Ratio of the marginalised constraints $\sigma^2 / \sigma^2_{\textrm{shear only}} $ , for $l_\max = 10^4$. This first line considers the inclusion of the size information in the analysis, while the second the size as well as the flexion fields $\mathcal F$ and $\mathcal G$.}.\label{ratiotable}
\begin{tabular*}{0.45\textwidth}{|cccccccc|}
 $\Omega_{\Lambda}$ & $\Omega_b$ & $\Omega_m$  & $h$  & $n$ &  $\sigma_8$ & $w_0$ & $w_a$ \\  \hline
 0.90 & 0.96 & 0.90 & 0.95 & 0.95 & 0.90 & 0.90 & 0.90 \\
  0.88 & 0.96 & 0.89 & 0.95 & 0.93 & 0.88 & 0.88 & 0.88
 \end{tabular*}
\end{table}
\end{center}
%----------------------------------------------------------------
%----------------------------------------------------------------
\black
\section{Summary and discussion}\label{discussion}
We have shown how Jaynes'  Maximal Entropy Principle allows us to construct the Fisher information content on model parameters in a given data set in the form of equation (\ref{sumform}) or (\ref{fishermaxent}). This is done by making the key quantity the entropy of the distribution as function of the constraints that we put on it. These constraints form our knowledge of the statistical properties of the future data. \textbf{To the best of the authors knowledge,  equation (\ref{sumform}) or (\ref{fishermaxent}) are not to be found in this form in the literature. However, they cannot  be considered new, since as stated earlier, they can be easily gained from the Fisher information content of the exponential family of distributions \citep{Jennrich75,vandenbos07}, after the identification of the curvature of the entropy surface with the generalised inverse of the covariance matrix.} Especially, the maximal entropy distributions are precisely those for which the Cram\'{e}r-Rao 
 inequality is an equality, since the curvature of the entropy surface is the inverse correlation matrix between the model predictions. \textbf{Equation (\ref{fishermaxent}) also bears a strong formal similarity to the well known result  \cite[chap. 2]{Kullback} or \cite[chap. 6]{caticha08}, that the Fisher information can always be written as the curvature of the Kullback-Leibler divergence for distributions parametrised by the same set of parameters.}
\newline\newline
The Fisher matrices currently used in weak lensing or clustering can all be seen as special cases of this approach, namely equation (\ref{FPk}), when knowledge of the \textbf{statistical properties of the future data does not go beyond the two-point statistics}. Indeed, in the case that the model does not predict the means, and knowing that for discrete fields the spectral matrices, equation (\ref{spectralmatrix}), carry a noise term due to the finite number of galaxies, or, in the case of weak lensing, also due to the intrinsic ellipticities of galaxies, the amount of information in (\ref{FPk})  is essentially identical to the standard expressions used to predict the accuracy with which parameters will be extracted from power-spectra analysis.
\newline\newline
There is, however, a conceptual difference worth noting in that the standard approach is to pick an estimator for the power-spectra and assume that both the fields as well as the distribution of the estimators are Gaussian. The result is the amount of Fisher information there is in the power spectra, under the assumptions of Gaussian statistics for the estimators and the fields. In our approach, the only assumption is on the fields distribution. Our results do not depend on the way the information will be extracted, but shows the amount of Fisher information in the fields as a whole. 
\newline\newline
Of course, the maximal entropy approach, which tries to capture the relevant properties of $p_X$ through a sophisticated guess, gives no guaranties that its predictions are actually correct. Nevertheless, as discussed in section \ref{redundant}, it provides a systematic approach with which to update the probability density function in case of improved knowledge of the relevant physics.
\newline
\newline
Using this formalism we have investigated the combined Fisher information content of weak lensing probes up to second order in the shapes distortions, assuming model parameter independent noise. By having a look at the joint Shannon entropy of the fields, we have shown how the only effect of treating these observables jointly is to reduce the effective level of noise contaminating the convergence field, according to equations (\ref{noise}) and (\ref{Entropy2}), independently of the model parameters.
\newline\newline\indent
These are the key points of this paper that we would like to emphasize :
\begin{enumerate}
\item Equation (\ref{fishermaxent}) presents a measure of information content that depends only on the constraints put on the data and the physical model. It is written in terms of the curvature of Shannon's entropy surface for maximal entropy distributions. It can always be interpreted, regardless of the actual distribution of the parameters, and of the specific way the analysis will proceed, as the expected curvature of the $\chi^2$ surface to the full set of model predictions. Assumptions of Gaussianity are neither needed nor used at any point. 
%----------------------------------------------------------------
\item  Over a very wide range of scales, the probe of choice both for mass reconstruction or cosmological purposes are the ellipticity components of the galaxies. Flexion takes over only on the arcsecond scale. In combination with the ellipticities, it can lead to substantial increase in statistical power on the scale of the arcminute. From the cosmological point of view, we expect size information to contribute at the $10\%$ level of the total information content. The only key parameter is the combination (\ref{improve}) of the dispersion values and the permeability $\alpha_s$ of the population sizes to the convergence field. On the other hand, the prospects of including flexion in cosmological analysis are less clear. The most obvious drawback being the need for an accurate understanding of the non-linear power spectrum.
\item
Besides, our results render the inclusion of flexion and size information within more detailed Fisher matrix analysis for future dark energy experiments extremely simple, such as in the exhaustive approach combining the information galaxy density fields with shear fields in a tomographic setting of \citep{2009ApJ...695..652B}. From (\ref{multis}) follows namely that the inclusion of all the two-point correlations of these additional weak lensing probes can be accounted for by adapting the noise term $N_\eff$.
\end{enumerate}
%----------------------------------------------------------------
%----------------------------------------------------------------
\black
Possible developments of this work includes the relaxation of the main limitation of the results, for instance the assumption that the noise is independent of the model parameters. Also, we plan to show that the approach presented in the first part of this work can lead to quantitative evaluations in non Gaussian cases as well, when other observables than the first two moments are also considered. 

\section{Cram\'{e}r-Rao 
 inequality}\label{CramerRao bound}
In this section, we provide a unified derivation of the Cram\'{e}r-Rao inequality in the multidimensional case (based on \citep{Rao}) and its relation to maximal entropy distributions. We denote the vector of model parameters of dimension $n$ with
\beq
\vecalpha = \bem\alpha_1,\cdots,\alpha_n\enm
\enq
and a vector of functions of dimension $m$ the estimators
\beq
\hat {\mathbf D} = \lp \hat D_1,\cdots \hat D_m \rp,
\enq
with expectation values $D_i(\vecalpha)=  \av {\hat D_i(x)} $. 
In the following, we rely on Gram matrices, whose elements are defined by scalar products. Namely, for a set of vectors $\vecy_i$, the Gram matrix $Y$ generated by this set of vectors is defined as
\beq
Y_{ij} = \vecy_i \cdot \vecy_j.
\enq
Gram matrices are positive definite and have the same rank as the set of vectors that generate them. Especially, if the vectors are linearly independent, the Gram matrix is strictly positive definite and invertible. \newline
We adopt a vectorial notation for functions, writing scalar products between vectors as
\beq
f\cdot g \equiv \int dx\:p_X(x,\vecalpha) f(x) g(x),
\enq
with $p_X(x,\vecalpha)$ being the probability density function of the variable $X$ of interest.
In this notation, both the Fisher information matrix and covariance matrix are seen to be Gram matrices. We have namely that the Fisher information matrix reads
\beq
 F_{ {\alpha_i}{\alpha_j}} = f_{\alpha_i} \cdot f_{\alpha_j},\quad f_{\alpha_i}(x) = \frac{\partial \ln p_X(x,\vecalpha)}{\partial \alpha_i},
\enq
while the covariance matrix of the estimators is
\beq
C_{ij} = g_i\cdot g_j,\quad g_i(x,\vecalpha) = \hat D_i(x) - D_i(\vecalpha). 
\enq
For simplicity and since it is sufficently generic for our purpose, we will assume that both sets of vectors $f$ and $g$ are lineary independent, so that both matrices can be inverted. Note that we also have
\beq
\frac{\partial D_i}{\partial {\alpha_j}} = \int dx \:p_X(x,\vecalpha) \:\hat D_i(x) \frac{\partial \ln p_X(x,\vecalpha)}{\partial {\alpha_j}} = g_i\cdot f_{\alpha_j}.
\enq
\newline
The  Gram matrix $ G$ of dimension $\lp (m + n) \times (m + n) \rp$ generated by the set of vectors $\lp g_1,\cdots, g_m ,f_{\alpha_1},\cdots, f_{\alpha_n}\rp $ takes the form
\beq
G = \bem  C & \Delta \\  \Delta^T & F \enm , \quad \Delta_{i {\alpha_j}} = g_i \cdot f_{\alpha_j}
\enq
and is also positive definite due to its very definition. It is congruent to the matrix
\beq
 Y G Y^T = \bem  C - \Delta F \inv \Delta^T & 0 \\ 0 & F \enm,
\enq
with
\beq
Y = \bem 1_{m\times m} & - \Delta F^{-1} \\ 0 & 1_{n\times n} \enm.
\enq
Since two congruent matrices have the same number of positive, zero and negative eigenvalues respectively and since both $ F$ and $G$  are positive, we can conclude that
\beq
C \ge \Delta F \inv \Delta^T,
\enq 
which is the Cram\'{e}r-Rao 
 inequality. The lower bound on the amount of information is seen from the fact that for any matrix written in block form holds
\beq
\bem  C & \Delta \\  \Delta^T & F \enm\ge 0 \Leftrightarrow \bem F & \Delta^T \\  \Delta & C \enm \ge 0
\enq
and using the same congruence argument leads to the lower bound on information
\beq
F \ge \Delta^T C \inv \Delta.
\enq
Assume now that we have a probability density function such that this inequality
is in fact an equality, i.e.
\beq
F = \Delta^T C \inv \Delta.
\enq
By the above argument, the Gram matrix generated by
\beq
\lp f_{\alpha_1},\cdots, f_{\alpha_n}, g_1,\cdots, g_m\rp
\enq
is congruent to the matrix
\beq
\bem 0_{n \times n} & 0 \\ 0& C \enm
\enq
and has rank $m$. By assumption, the covariance matrix is invertible, such that the set $\lp g_1,\cdots, g_m \rp$ alone has rank $m$. It implies that each of the $f$ vector can be written as linear combination of the $g$ vectors,
\beq
f_{\alpha_i} = \sum_{j = 1}^{m} A_{j} g_j,
\enq
or, more explicitly,
\beq
\frac{\partial \ln p_X(x,\vecalpha)}{\partial {\alpha_i}} =  \sum_{j = 1}^{m} A_{ j}(\vecalpha) \left[\hat{ D_j}(x) - D_j(\vecalpha)\right],
\enq
where the key point is that the coefficients $A_j$ are independent of $x$. Integrating this equation, we obtain
\beq
\ln p_X(x,\vecalpha) = -\sum_{i = 1}^m \lambda_i(\vecalpha)\hat {D_i}(x) - \ln Z(\vecalpha) + \ln q_X(x)
\enq
for some functions $\lambda$ and $Z$ of the model parameters only, and a function $q_X$ of $x$ only. We obtain thus
\beq
p_X(x,\vecalpha) = \frac {q_X(x)} {Z(\vecalpha)} \exp\left(-\sum^m_{i=1} \lambda_i (\vecalpha)\hat {D}_i(x) \right).
\enq
This is precisely the distribution that we obtain by maximising the entropy relative to $q_X(x)$, while satisfying the constraints
\beq
D_i(\vecalpha) = \av{\hat D_i(x)},\quad i = 1,\cdots, m.
\enq 
Taking $q_X$ as the uniform distribution makes it identical with the formula in equation (\ref{MaxEnt}).
%----------------------------------------------------------------
%----------------------------------------------------------------
\section{Point fields}\label{pf}
The data consists in a set of numbers, at each position where a galaxy sit and a measurement was done. We use the handy notation in terms of Dirac delta function,
\beq
\phi(\vecx) = \sum_i \epsilon_i\delta^D(\vecx - \vecx_i),
\enq
where the sum runs over the positions $\vecx_i$ for which $\epsilon$ is measured. To obtain the spectral matrices, we need the Fourier transform of the field, which reads in our case
\beq
\tilde \phi(\vecl) = \sum_i \epsilon_i \exp\lp - i \vecl\cdot \vecx_i\rp. 
\enq
In this work, we assume that the set of points shows negligible clustering, so that the probability density function for the joint occurrence of a particular set of galaxy positions is uniform.\newline
We decompose in the following the wave vector $\veck$ on the flat sky in terms of its modulus and polar angle as
\beq
\vecl = l\bem \cos\phi_l \\ \sin \phi_l \enm.
\enq
\subsection{Ellipticities}
When the two ellipticity components are measured, we have two such fields $\phi_1,\phi_2$ at our disposal. For instance, the field describing the first component becomes
\beq \label{ff}
\tilde \phi_1(\vecl) = \sum_{i} \epsilon^1_i \exp\lp - i \vecl\cdot \vecx_i\rp.
\enq
We assume that the measured ellipticities trace the shear fields, in the sense that the measured components are built out of the shear at that position plus some value unrelated to it,
\beq \begin{split} \label{rel}
\epsilon^1_i &= \gamma_1(\vecx_i) + \epsilon^1_{\textrm{int},\:i}
\\
\epsilon^2_i &= \gamma_2(\vecx_i) + \epsilon^2_{\textrm{int},\:i}.
\end{split}
\enq
The vector $\vecv$ relating the spectral matrices of the ellipticities and the convergence
is then obtained by plugging (\ref{ff}) with the above relations (\ref{rel}) in its definition (\ref{specmatrix}), and using the relation between shears and convergence in equation (\ref{distortion}). The result is 
\beq
\vecv =\bar n_\gamma  \bem \cos 2\phi_l \\ \sin 2\phi_l\enm.
\enq
where $\bar n_\gamma$ is the number density of galaxies for which ellipticity measurements are available.
Under our assumptions of uncorrelated intrinsic ellipticities,  with dispersions of equal magnitude $\sigma_\gamma^2$ for the two components, the noise matrix $N$ becomes 
\beq
N = \bar n_\gamma \bem \sigma_\gamma^2 & 0 \\ 0 & \sigma_\gamma^2\enm.
\enq
The effective noise, given in equation (\ref{noise}) is readily computed
\beq
N^\gamma_\eff = \frac{\sigma^2_\gamma}{\bar n_\gamma}.
\enq
\subsection{Sizes}
As noted in the main text, the apparent sizes of galaxies are modified by lensing, in the following way,
\beq
s^i_{\obs} = s^i_{\textrm{int}}\lp 1 + \alpha_s \kappa\rp,
\enq for some coefficient $\alpha_s$ which is unity in pure weak lensing theory. Denoting the number of galaxies for which sizes measurements are available by $n_s$, and the mean intrinsic size of the sample by $\bar s_{\textrm{int}}$,
the spectrum of the size field reduces, under the assumption of uncorrelated intrinsic sizes, to
\beq
C^s(l) = \bar n_s^2 \bar s_{\textrm{int}}^2 \alpha_s^2 C^{\kappa}(l) + \bar n_s \sigma_s^2.
\enq
The vector $\vecv$ and matrix $N$ are now numbers,  that are read out from the above equation, to be
\beq \begin{split}
v &= \bar n_s\bar s_{\textrm{int}} \alpha_s, \\
N &= \bar n_s \sigma_s^2.
\end{split}
\enq
leading to the effective noise
\beq
N_\eff^s = \frac{1}{\alpha_s^2}\lp \frac{\sigma_s}{\bar s_\textrm{int}} \rp^2\frac 1 {\bar n_s}
\enq
\subsection{Second order, flexion}
Denoting with $\bar n_{\mathcal F}$ and $\bar n_{\mathcal G}$ the number of galaxies for which $\mathcal F$ and $\mathcal G$ are measured, the vectors linking the flexion to convergence are
\beq
\vecv^{\mathcal F} = -il\bar n_{\mathcal F}\bem \cos \phi_l \\ \sin \phi_l\enm\enq
and
\beq
\vecv^{\mathcal G} = -il\bar n_{\mathcal G}\bem \cos 3\phi_l \\ \sin 3\phi_l\enm.
\enq
Using again the assumption of uncorrelated intrinsic components, we have the four dimensional diagonal noise matrix 
\beq
N = \bem \bar n_\mathcal F \sigma^2_\mathcal F \cdot 1_{2x2}& 0 \\0  & \bar n_\mathcal G \sigma^2_\mathcal G\cdot 1_{2x2}\enm,
\enq
leading to the effective noise, this time mode-dependent,
\beq 
\frac 1 { N^{\mathcal F \mathcal G}_\eff} = l^2\left(\frac{\bar n_F}{\sigma_F^2} + \frac{\bar n_G}{\sigma_G^2}\right).
\enq
%----------------------------------------------------------------
%----------------------------------------------------------------



==> chapter2.tex <==
%\setprelude{\uppercase{A\scriptsize{n inconceivably numerous host of stars must be here arranged\\ together }\normalsize{[...],}\scriptsize{ because their free positions towards each other\\ would otherwise have presented irregular forms and not exact\\ figures}}\normalsize{.}
%\vspace{5truemm}\\
%\normalsize{Immanuel Kant, {\it Universal History and Theory of the Heavens} \cite{kant1755}}}

\chapter{Beyond the Gaussian: information in high order statistics}
\label{ch2}

\begin{center}
Foreword to chapter 2
\end{center}
%\section{Introduction}
The purpose of this chapter is to derive and present in a comprehensive manner the independents bits of Fisher information that are associated to the moment of a given order, for several important families of probability density functions, that spans a wide range of situations.  Fisher information and moments both are concept of prime importance in statistics and inference on model parameters \cite{fisher25,Rao,vandenbos07}. The general approach to decompose the Fisher information matrix in uncorrelated components according to an orthogonal system was shown in theorem 3.1 in \cite{Jarrett84}. It seems however that this procedure was not given further real attention. In these notes, we pursue these ideas, dealing with the system of moments, where the associated orthogonal system are polynomials.
\newline
More specifically, we will in a first step define for a probability distribution $p(x,\alpha ,\beta ,\cdots)$, $\alpha,\beta,\cdots$ any model parameters, coefficients $s_n(\alpha)$ which unambiguously represent the independent information content of the moment of order $n$ on $\alpha$. These coefficients can be used to reconstruct the Fisher information matrix order by order. We give in closed form these coefficients for several common classes of distributions.
\newline
In a second step, we use this decomposition to approach the indeterminate moment problem. Namely, the Fisher information content of a moments series can be less than the information content of the probability density function it originates from, if that function cannot be uniquely recovered from the series. Therefore, this loss of information is also a useful measure of the indeterminacy of the moment problem.
\newline
The content of this chapter has its origin\cite{2011ApJ...738...86C,Frommert11} in concrete problems in the field of cosmology, where moments, or their field analog the correlation functions play an important role for parameter inference. Maybe a bit unexpectedly, our results are apparently not to be found in the literature so far. We are certainly not advocating extraction of moments to be the way to perform inference on model parameters. Nonetheless, it often provides a convenient approach, or must sometimes be done out of necessity, and certainly allows useful insights into the problems at hand. The results we present allow oneself to evaluate in a quantitative manner the contribution of each successive moment to expected final constraints on the relevant parameters.  Besides, it provides an interesting link between parameter inference, orthogonal polynomials and the classical moment problem \cite{Simon97theclassical,Akhiezer65,Shohat63}
\newline
This chapter is built as follows : We begin in section \ref{generaltheory} with a brief review on the fundamentals of Fisher information and how this decomposition proceeds, and present the most relevant aspects of this expansion. This will allow us to introduce some notation. In section \ref{determ}, we present this exact decomposition for a few determinate probability density functions. For these, the amount of Fisher information of the moments is identical to the total amount. Beside the very simple case of the Gaussian distribution, we present this decomposition for the beta, gamma families as well as for an extended Poisson model, that was motivated by a study \cite{Frommert11}, where it was used a toy model for point sources emission. We then turn in section \ref{indeterm} to indeterminate probability density functions.  After dealing with the lognormal distribution, whose expansion we presented elsewhere already \cite{2011ApJ...738...86C}, we treat numerically the Weibull distribution and strectched exponential. For each of those we compare the information lost to the moment hierarchy to Stoyanov's dissimilarity index of associated Stieltjes classes \cite{Stoyanov04}.
%%%%%%%%%%
%\section{Brief review}
%%%%%%%%%%
%We first briefly review the concept of Fisher information and present the information inequality, also called Cramer-Rao bound, fundamental to this work. We refer to Fisher's original work \cite{fisher25} and the textbooks \cite{Rao,vandenbos07} for various expositions of this concept old about a century. With section (\ref{Decomposition in moments, orthogonal polynomials}) we introduce the decomposition of the Fisher information in uncorrelated pieces associated unambiguously to the independent information content of the moment of some order. This proceeds with the help of orthonormal polynomials. The basics of such a decomposition was introduced it seems in \cite{Jarrett84}. 
%We could not find however other works dealing with these issues. 
\section{Mathematical framework}
\label{generaltheory}
Consider a family of probability distributions $p(x,\theta)$\footnote{We are making here all the necessary regularity conditions for derivatives to exist, and the exchange of integration and differentiation to be possible.} depending on a set of model parameters $\theta = (\alpha,\beta,\cdots)$. The function
\beq
s(x,\alpha) = \frac{\partial \ln p(x,\theta)}{\partial \alpha}
\enq
is called the score function associated to $\alpha$. 
For any value of the model parameters, $p(x,\theta)$ is normalised to unity. For this reason, it holds true that the score function averages to zero,
\beq
\av{s(x,\alpha)} = 0.
\enq
The Fisher information matrix $F$ \cite{fisher25,Rao,vandenbos07} is then defined as the covariance matrix of the score functions :
\beq \label{defF}
F_{\alpha\beta} = \av{s(x,\alpha)s(x,\beta)}.
\enq
F is always a semi-positive definite matrix, though it may be singular in some cases. It is also additive for independent variables, and invariant under invertible transformations. It plays a major role in statistical inference due to the information inequality. For any set of unbiased estimators $\hat{ \mathbf O}$ aimed at extracting the vector $\mathbf O$, the following inequality between positive definite matrices\footnote{ $A \ge B$ means that $A-B$ is positive definite. In particular, the diagonal entries of $A$ (resp. $A^{-1}$) are larger (smaller) than those of $B$ ($B^{-1}$).\cite[chap. 7, e.g.]{0521386322} for many more properties.} holds : 
\beq \label{infoinequality}
F _{\alpha\beta} \ge \frac{\partial \mathbf O}{\partial \alpha} \Sigma^{-1} \frac{\partial \mathbf O}{\partial \beta},
\enq
where $\Sigma$ is the covariance matrix of the estimators,
\beq
\Sigma_{ij} = \av{\hat O_i \hat O_j} - O_iO_j.
\enq
The right hand side of equation (\ref{infoinequality}) can be seen to be the expected curvature of a $\chi^2$ fit to the estimates $\mathbf O$, around a best-fit value for which the $\chi^2$ is at a minimum. For this reason, the Fisher information matrix bounds in some way the accuracy with which the actual values of parameters can be extracted from $x$ with the help of unbiased estimators. If equality holds in equation(\ref{infoinequality}), its inverse $F^{-1}$ is an approximation to the covariance matrix of the parameters $\theta = (\alpha,\beta,\cdots)$ themselves, as obtained from the extraction of $\mathbf O$ from $x$. The right hand side of equation (\ref{infoinequality}) can be interpreted in general as the amount of Fisher information contained in the set $\mathbf O$, which is thus always less or equal the total amount of Fisher information in $p(x,\theta)$.
\newline
%\subsection{Decomposition in moments, orthogonal polynomials}\label{Decomposition in moments, orthogonal polynomials}
When the vector $\mathbf O$ are the moments themselves, $O_i = m_i = \av{x^i},\quad i = 1,\cdots N$,
it is possible to rewrite the information inequality in a more insightful form. Consider the set of polynomials orthogonal with respect to $p(x,\theta)$,
\beq \label{orthopol}
\begin{split}
P_n(x) &= \sum_{k = 0}^nC_{nk}x^k \\
\av{P_n(x)P_m(x)}  &= h_n\delta_{mn}, \quad n,m = 0,\cdots,N
\end{split}
\enq
where $h_n$ is some strictly positive number, equal to unity if the polynomials are orthonormal. Since the normalisation of many common orthogonal polynomials is not unity, we will the keep track of the terms $h_n$ in the following. Of course, the polynomials $\tilde P_n =P_n / \sqrt{h_n}$ are then orthonormal. We refer to \cite{Freud71,Szego39} for the theory of orthogonal polynomials. It is enough for our purpose to recall the reader that these can always be constructed from the first $2N$ moments, and are unique up to a sign, which we set by requiring the coefficient $C_{nn}$ of $x^n$ in $P_n$ to be positive.
The key point  for our purposes is to realise that the inverse covariance matrix between the moments can be written \footnote{This can be seen expanding the normalisation condition given in equation (\ref{orthopol}) in terms of the triangular matrix $C$.}
\beq \label{sigmaP}
\lb \Sigma^{-1} \rb_{ij} = \sum_{n= 0}^N\frac{C_{in}C_{jn}}{h_n},\quad i,j = 1,\cdots N.
\enq
This identity allow us to express the Fisher information content of the moments in the form of a sum of uncorrelated pieces : using (\ref{sigmaP}), it holds
\beq \label{chi2}
\sum_{i,j = 1}^N \frac{\partial m_i}{\partial\alpha}\Sigma^{-1}_{ij}\frac{\partial m_j}{\partial \beta} = \sum_{n = 1}^Ns_n(\alpha)s_n(\beta).
\enq
We defined there the information coefficients
\beq \label{def}
s_n(\alpha) = \frac{1}{\sqrt{h_n}}\sum_{k = 1}^nC_{nk}\frac{\partial m_k}{\partial \alpha}, \quad n \ge 1
\enq
and similarly for any model parameter. The matrix $s_N(\alpha)s_N(\beta)$
is therefore the part of the Fisher information in the $N$th moment
that was not contained in the moments of lower order.\newline
These coefficients have a straightforward interpretation. They can be namely written as
\beq\label{sn}
s_n(\alpha) = \av{s(x,\alpha)\tilde P_n(x)},
\enq
which we will take as the definition of $s_n(\alpha)$. This can be seen from expanding $P_n(x)$ in terms of the matrix $C$, and noting that $s(x,\alpha)p(x,\theta) = \partial_\alpha p(x,\theta)$, recovering \eqref{def}. In other words, $s_n(\alpha)$ is nothing else than the component of the corresponding score function parallel to the orthonormal polynomial of order $n$.
%We note that for any $s_n(\alpha)$ is invariant under any linear transformation of the field (provided the mapping is independent of $\alpha$). Given
%$y = ax+ b$, with probability density function
%\beq
%p_Y(y,\alpha)dy = p\lp \frac{y-b}{a},\alpha\rp dx
%\enq
%the polynomials $Q_n$ orthonormal to $p_Y(y,\alpha)$ are given by
%\beq
%Q_n(y) = \frac{1}{\sqrt{h_n}}P_n\lp \frac{y-b}{a}\rp. 
%\enq
%On the other hand the score function transforms the very same way, $s_Y(y,\alpha) = s((y-b)/a,\alpha)$, so that the right hand side of equation (\ref{sn}) and thus $s_n(\alpha)$ stay unchanged.
%\newline\newline
It follows immediately from equation (\ref{sn}) that the Fisher information content of the moments depends on how well the score functions can be approximated through polynomials. With increasing $N$, one expects the score function to be better and better reproduced by the series
\beq
s_{\le N}(x,\alpha) := \sum_{n  =1}^Ns_n(\alpha)P_n(x).
\enq
In general, the following matrix inequality holds
\beq
\begin{split}
0 &\le \av{ \lp s(x,\alpha) - s_{\le N}(x,\alpha)\rp\lp s(x,\beta) - s_{\le N}(x,\beta)\rp } \\&
= F_{\alpha\beta} -  \sum_{i,j = 1}^N \frac{\partial m_i}{\partial\alpha}\Sigma^{-1}_{ij}\frac{\partial m_j}{\partial \beta}.
\end{split}
\enq
Especially, for any parameter $\alpha$ holds
\beq \label{residuals}
 \av{\lp s(x,\alpha) - s_{\le N}(x,\alpha)\rp^2} = I(\alpha) -  \sum_{i,j = 1}^N \frac{\partial m_i}{\partial\alpha}\Sigma^{-1}_{ij}\frac{\partial m_j}{\partial \alpha},
\enq
where $I(\alpha) := F_{\alpha\alpha}$ is the Fisher information on $\alpha$. The bits of Fisher information that are absent from the set of moments $m_1$ to $m_N$ are thus precisely the mean squared error of the fit of the score function through polynomials throughout the range of $p(x,\theta)$.
\newline
Especially, if the score function is itself a polynomial, of degree $N$, for each values of the parameters, then only the first $N$ of these coefficients are possibly non-zero. A finite number of moments do catch all the Fisher information content of $p(x,\theta)$ in this case. In fact, the reverse statement is also true. This can be understood in the framework of orthodox statistics : in this case $p(x,\theta)$ can be shown to be of the exponential type, where a finite number of sufficient statistics exist \cite{1936PCPS...32..567P,koopman36}. In a more bayesian point of view, these distributions can also be seen as precisely those that maximises Shannon entropy for fixed values of the first $N$ moments. See \cite{RePEc:spr:metrik:v:41:y:1994:i:1:p:109-119,jaynes2003}
The ubiquitous example of this family being of course the normal distribution, which we will treat first.
\newline
We define for further reference the matrix $ F_{\le N}$ through its matrix elements,
\beq\label{Fn}
\lb F_{\le N} \rb_{\alpha\beta} := \sum_{n= 1}^Ns_n(\alpha) s_n(\beta).
\enq
We stress that $F_{\le N}$ is, strictly speaking, associated to a moment series rather than a probability density function. These matrices are namely identical for different distributions having the same moment series.
\subsection{The Christoffel-Darboux kernel as an information matrix}
%%%%%%%%%%%%%%%%%%%%%
To conclude, it is interesting to see what the is interpretation of the orthogonal polynomials themselves, in this information theoretic framework. To this aim, consider that the model parameter of interests are the values of the probability density themselves, allowing complete freedom in its shape. Consider for simplicity discrete values $x_i$, the index $i$ in some infinite set, occurring with probabilities
\beq
p(x_i): = p_i := \frac{q_i}{Z},\quad Z = \sum_i q_i
\enq 
the model parameters being the set of $q_i$. Simple calculations lead to the following expression for the Fisher information matrix elements on the parameters $q_i,q_j$,
\beq
F_{ij}= \frac 1 {Z^2}\lp \frac{ \delta_{ij}} {p_i}  -1 \rp.
\enq
On the other hand, we have $\partial m_k/ \partial q_i = (x_i^k - m_k)/Z$, leading to
\beq
s_n(q_i) = \frac 1 Z P_n(x_i).
\enq
Therefore, $P_n(x_i)$ is directly proportional to the Fisher information content of the $n$th moment on the probability of $x_i$.
Also, the Christoffel-Darboux kernel, defined as
\beq
K_N(x_i,x_j) = \sum_{n = 0}^NP_n(x_i)P_n(x_j)
\enq
can be given some simple interpretation. We have namely from these relations that the information escaping the first $N$ moments is given by
\beq
F_{ij} - \lb F_{\le N} \rb_{ij} = \frac 1 {Z^2} \lp  \frac{\delta_{ij}}{p_i} -  K_N(x_i,x_j)\rp.
\enq
In accordance with our discussions above, for determinate moment problems, this expressions tends to zero as $N \rightarrow \infty$.  This can be seen from the fact that in this case, from Riesz theorem, the reproducing property holds
\beq
\sum_i p(x_i)\lb f(x_i) - \sum_{n = 0}^N \lp \sum_{k} p(x_k) f(x_k) P_n(x_k)\rp P_n(x_i) \rb^2  \rightarrow 0,
\enq
for any function $f(x_i)$ that is square summable with respect to $p(x_i)$.
This implies
\beq
\sum_{k}p(x_k)f(x_k) K_N(x_k,x_i) \rightarrow f(x_i)
\enq
for any such function and therefore
\beq
K_N(x_i,x_k) \rightarrow \frac{\delta_{ij}}{p(x_k)}.
\enq
\clearpage\newpage
\def\apj{The Astrophysical Journal}                 % Astrophysical Journal
%% DET
\section{Some exactly solvable models for determinate measures}\label{determ}
In general, it follows from the above considerations that the moments will form efficient probes of the model parameters whenever the score functions can be well approximated over the range of $p(x,\theta)$ through polynomials of low order. If this is not the case, then one may need to go very deep the moment hierarchy in order to catch the information, or information may escape the hierarchy.
A sufficient criterium for the moment hierarchy to possess the same amount of information as the probability density function itself is that the moment problem associated to the moment series is determinate, i.e. that the function can be uniquely recovered from the series. In this case, by a well known theorem due to M. Riesz, \cite{Riesz23}, the orthogonal polynomials form a complete set. Therefore, the square residual in equation \eqref{residuals} goes to zero for $N \rightarrow \infty$. For the probability density functions dealt with in this section, we thus have
\beq
\lim_{N \rightarrow \infty} F_{\le N} = F.
\enq
%\input{normal}
%%%%%%%%%% NORMAL %%%%%%%%%
\subsection{Normal distribution}\label{normal}
%%%%%%%%%% NORMAL %%%%%%%%%
The normal distribution provides us a very simple test case of the approach. Its probability density function is
\beq
p(x,\mu,\sigma^2) = \frac{1}{\sqrt{2\pi}\sigma}\exp\lp -\frac 12 \frac{\lp x - \mu\rp^2}{\sigma^2} \rp.
\enq
Its Fisher information matrix is well known,
\beq\label{Fgauss}
F = \bem \frac{1}{\sigma^2} &  0 \\  0 & \frac{1}{2\sigma^4} \enm.
\enq
The information coefficients take the form
\beq \label{smuG}
s_1(\mu) = \frac 1 \sigma, \quad s_n(\mu) = 0, \quad n \ne 1,
\enq
and
\beq\label{ssigG}
s_2(\sigma^2) =  \frac{1}{\sqrt{2}\sigma^2},\quad s_n(\sigma^2) = 0, \quad n \ne 2.
\enq
We recover already the full matrix with the first two moments, $F_{\le 2} = F$. The matrix is diagonal 
because there is no order $n$ for which both coefficients $s_n(\mu)$ and $s_n(\sigma^2)$ do not vanish.
%%%% DERIVATION NORMAL %%%%%
\paragraph{Derivation :}
It is easily seen that the score function $\partial_\mu \ln p$ is a polynomial of first order in $x$. This implies immediately that only $s_1(\mu)$ is non-zero. For any probability density function and parameter $\alpha$, it holds from \eqref{def} that
\beq
s_1(\alpha) = \frac{\partial m_1}{\partial \alpha}\frac 1 \sigma,
\enq
which proves \eqref{smuG}. Very similarly, the score function associated to $\sigma^2$ is a polynomials second order, such that only the first two coefficients can possibly be non-zero. However, $s_1(\sigma^2)$ vanishes since $\sigma^2$ does not impact the mean. Finally, $s_2(\sigma^2)$ can be gained by noting that the polynomials orthogonal to the normal 
distribution are the Hermite polynomials \cite{Szego39},
\beq
P_n(x) = H_n\lp \frac{x-\mu}{\sigma}\rp,
\enq
with normalisation $h_n = 1 / n! $. From $H_2(x) = x^2 - 1$
and equation (\ref{def}) follows $C_{22} = 1 / \sigma^2$ and $s_2(\sigma^2) = \frac{1}{\sqrt{2}\sigma^2}.$
%In other words, we have
%\beq
%\frac{\partial \ln p }{\partial \sigma^2} = \frac{1}{2\sigma^2} H_2\lp  \frac{x-\mu}{\sigma}\rp.
%\enq
%%%% END DERIVATION NORMAL %%%%%
%%%%%%%%%%  BETA %%%%%%%%%
\subsection{Beta distribution}\label{beta}
%%%%%%%%%% BETA %%%%%%%%%
The beta distribution is defined as
\beq
p(x,\alpha,\beta) = \frac{x^{\alpha - 1}\lp 1 - x\rp ^{\beta-1}}{B(\alpha,\beta)},\quad 0 < x < 1,\:\:\alpha,\beta > 0
\enq
where $B(\alpha,\beta)$ is the beta integral, which will also enter the following section on the gamma distribution. It has the well known representation in terms of the gamma function $\Gamma$,  $B(\alpha,\beta) = \Gamma(\alpha)\Gamma(\beta) / \Gamma(\alpha + \beta)$.
The full Fisher information matrix can be conveniently expressed in terms of the second derivative of the logarithm of the gamma function, called the digamma function $\psi_1$ \cite[p. 258-260]{abramowitz70a},
\beq \label{Fbeta}
F = 
\bem 
\psi_1(\alpha) & 0 \\ 0 & \psi_1(\beta)
\enm
- \psi_1(\alpha + \beta)
\bem 1 & 1 \\1 & 1
\enm,
\enq
Our derivation of the information coefficients associated to $\alpha$ and $\beta$, based on the explicit expressions of the orthogonal polynomials, in this case the Jacobi polynomials, is rather lengthy. We defer it to the appendix. The result is
\beq
s_n(\alpha) = - \frac {(-1)^{n}}{n} \lp \frac{(\beta)^{(n)}n!}{(\alpha)^{(n)}(\alpha + \beta)^{(n)}} \rp^{1/2} \lp \frac{2n + \alpha + \beta -1}{n + \alpha + \beta -1} \rp^{1/2}.
\enq
and
\beq
s_n(\beta) = - \frac {1}{n} \lp \frac{(\alpha)^{(n)}n!}{(\beta)^{(n)}(\alpha + \beta)^{(n)}} \rp^{1/2} \lp \frac{2n + \alpha + \beta -1}{n + \alpha + \beta -1} \rp^{1/2},
\enq
where $\lp x \rp^{(n)} := x(x+1)\cdots (x + n -1)$ is the rising factorial. For the symmetric case $\alpha = \beta = 1/2$, these expressions simplify considerably. We have namely
\beq
s_n(\alpha) = (-1)^{n-1}\frac{\sqrt 2}{n},\quad s_n(\beta) = -\frac{\sqrt 2}{n}.
\enq
Since $\psi_1(1/2) = \pi^2 / 2$ and $\psi_1(1) = \pi^2 / 6$, a short calculation shows that we recover indeed, summing these coefficients, the full matrix given  in \eqref{Fbeta}
\beq
\left. F \right|_{\alpha = \beta = 1/2} = \frac{\pi^2}{6} \bem 2 & - 1 \\ -1  & 2 \enm.
\enq  
%%%%%%%%%%  GAMMA %%%%%%%%%
\subsection{Gamma distribution}\label{gamma}
%%%%%%%%%% GAMMA %%%%%%%%%
The gamma distribution form a two parameter family,
\beq
p(x,\ln \theta,k) := \frac{e^{-x/\theta}}{\theta^k\Gamma(k)}x^{k-1} \quad k,\theta > 0,\quad x > 0.
\enq
where $\Gamma(k)$ is the gamma function. 
The calculation of the Fisher information matrix associated to $\ln \theta$ and $k$ is not difficult. Again, the trigamma function shows up,
\beq \label{Fgamma}
F = \bem k  & 1    \\ & \\ 1   & \psi_1(k) \enm. 
\enq
\newcommand{\lag}[2]{L_{#1}^{(#2)}}
The information coefficients are evaluated below, with the result
\beq
s_1(\ln\theta) = \sqrt{k},\quad s_n(\ln \theta) =0 ,\quad n \ne 1,
\enq
and
\beq
s_n( k) = (-1)^{n-1}\sqrt{ \frac{ B(k,n)}{n}}.
\enq
As a consistency check, we see that since $s_1( k) = \frac{1}{\sqrt k}$, we recover trivially the $\ln \theta \ln \theta$ and $\ln \theta k$ elements of the matrix  (\ref{Fgamma}).
Its $kk$ element implies that the following identity must hold,
\beq
\sum_{n = 1}^{\infty} \frac{B(k,n)}{n} =  \psi_1(k),\quad k > 0,
\enq
which reduces for $k = 1$ to Euler's famous formula $\sum_{n = 1}^\infty \frac{1}{n^2} = \frac{\pi^2}{6}$. The above identity can of course be proven by much more direct methods.
%%%% DERIVATION GAMMA %%%%%
\paragraph{Derivation :}
The polynomials associated to that distribution are the generalized Laguerre polynomials $L_n^{(k-1)}$[p.775]\cite{abramowitz70a} . More precisely, we have
\beq
\int_0^\infty t^{k-1} e^{-t} \lag n {k-1} (t)\lag m {k-1}(t) = \frac{\Gamma(n + k)}{n!}\delta_{mn}.
\enq
For this reason, the polynomials orthogonal to the gamma distribution are
\beq
P_n(x) := \lag n {k-1}\lp \frac{x}{\theta} \rp,
\enq
with normalisation
\beq \label{norm}
h_n = \frac{\Gamma(n + k)}{\Gamma(k)}\frac{1}{n!} = \frac 1 n \frac 1 {B(k,n)}. 
\enq
They have the explicit matrix elements $C_{ni}$\footnote{We added the factor $(-1)^n$, in accordance with our convention of having a matrix element $C_{nn}$ positive.},
\beq 
C_{ni} = (-1)^{n-i} \bin {n+k-1}{n-i} \frac{\theta^{-i}}{i!}.
\enq
The moments of the gamma function are given by
\beq
m_n = \theta^n\frac{\Gamma(n + k)}{\Gamma(k)}.
\enq
The Fisher information on $\theta$ is the simplest. It holds namely that the score function associated to $\theta$ is a polynomial first order in $x$, and therefore that only $s_1(\ln \theta)$ is non-zero. It follows
\beq
s_1(\ln\theta) = \sqrt{k},\quad s_n(\ln \theta) =0 ,\quad n \ne 1.
\enq
The calculation of $s_n( k)$ requires a little bit more work, but we can make use of previous results of section \ref{beta}. The derivatives of the moments with respect to $k$ are given by
\beq
\frac{\partial \ln m_n}{\partial k} = \psi_0(k + n) - \psi_0(k).
\enq
Using the representation (\ref{def}), together with 
\beq
\begin{split}
\bin {n + k -1}{n -i}\frac{1}{i!}\frac 1 {\Gamma(k + i)} = \frac{\Gamma(n + k)}{\Gamma(n + 1)} \bin n i.
\end{split}
\enq
one obtains the following expression
\beq
\begin{split}
s_n(k)  &=  \frac {1} { \sqrt {n\:B(k,n)}}\sum_{i = 0}^n (-1)^{n-i} \bin ni \lp  \psi_0(k + i) - \psi_0(k) \rp.
\end{split}
\enq
The sum is precisely the function $f_q(t)$ defined in (\ref{defft}), evaluated a $t = 1$ and $k = q$, and that we proved in (\ref{ftbeta}) to be a representation of the beta function,
\beq
f_k(1) = (-1)^{n-1} B(k,n).
\enq
We conclude therefore
\beq
s_n( k) = (-1)^{n-1}\sqrt{ \frac{ B(k,n)}{n}}.
\enq
%%%% END DERIVATION GAMMA %%%%%
%%%%%%%%%%  POISSON %%%%%%%%%
\subsection{Poisson distribution}\label{poisson}
%%%%%%%%%%  POISSON %%%%%%%%%
Consider the probability density function
\beq
p(x,\mu,\ln A) = \sum_{n = 0}^\infty e^{-\mu} \frac{\mu^n}{n!} \delta^D(x - An),\quad \mu, A > 0
\enq
with $\delta^D$ the Dirac delta function. This is the usual Poisson law, together with some amplitude $A$ that is left free. If $A$ is set to unity, we recover the Poisson law.
%It was used as a toy model to describe the observation of radio emission from a number $n$ of point sources all radiating at the same amplitude $A$.
\newline
This is a peculiar situation in terms of Fisher information. Unlike the previous situations, the parameter $A$ impacts indeed the range of $x$. The Fisher information on $A$ is not well defined in the form of equation (\ref{defF}), formally infinite.
\newline
Even though the Fisher information matrix is not well defined, the information coefficients as given in equations (\ref{def}) or (\ref{sn}) are, and so are their interpretation (\ref{chi2}) in terms of the expected curvature of a $\chi^2$ fit. 
The result is
\beq
s_1(\ln \mu) = \sqrt{\mu},\quad s_n(\ln \mu) = 0,\quad n \ne 1.
\enq
and
\beq
\label{snlnA}
\begin{split}
s_1(\ln A) &= \sqrt{\mu}, \quad s_n(\ln A) = (-1)^n \frac{\sqrt {n!}}{n(n-1)}\mu^{1-n/2},\quad n \ge 2 .
\end{split}
\enq
Note that it is compatible with the fact that the Fisher information on $A$ is infinite. For any $\mu$ the sum
\beq
\sum_{n = 1}^\infty s_n^2(\ln A)
\enq
is divergent. The turnover of the coefficients occurs around $n \approx \mu$ where they start to increase. Atypically, the higher order the moment the most interesting it becomes for inference on $A$ in this model.
%%%% DERIVATION POISSON %%%%%
\paragraph{Derivation :}
Consider the Charlier polynomials \cite[pp.788]{abramowitz70a}, defined by
\beq \label{Charlier}
c_n(x) := \sum_{k = 0}^{n}(-1)^{n-k}\bin nk \mu^{-k}(x)_k,
\enq
where
\beq
x(x-1)\cdots(x-m+1) =: (x)_m
\enq
is the falling factorial. These are the polynomials orthogonal with respect to the Poisson distribution with intensity $\mu$. Clearly, the polynomials
\beq \label{Ppoisson}
P_n(x) := c_n\lp \frac x A\rp
\enq
are then the polynomials orthogonal to $p(x,\mu,\ln A)$. The normalization is
\beq \label{normalisation}
h_n = \frac{n!}{\mu^n}.
\enq
On the other hand, the moments are given by $m_n =  A^nm^P_n$,
where $m^P_n$ is the $n$th moment of the Poisson distribution.
For this reason, it holds that $\frac{\partial m_n}{\partial \ln A} = n \:m_n$.
This equation, together with (\ref{Ppoisson}) implies that the information coefficients on $\ln A$ are independent of the actual value of $A$, since $C_{nk} \propto A^{-k}$ and $m_k \propto A^k$. So are the coefficients $s_n(\ln \mu)$. We can therefore from now on safely chose $A = 1$ as the fiducial value, and work with the usual Poisson distribution and associated Charlier polynomials.
\newline
The coefficients associated to $\ln \mu$ are the simplest to obtain. It is not difficult to see that the score function associated to $\ln \mu$ of the Poisson distribution is a polynomial of first order. We obtain $s_1(\ln \mu) = \sqrt{\mu}$
and $s_n(\ln \mu) = 0,\quad n \ne 1$.
Turning to $\ln A$, we need to evaluate
\beq
s_n(\ln A) =\frac{\mu^{n/2}}{\sqrt{n!}} \sum_{k = 0}^n C_{nk}\:k \:m_k.
\enq 
The derivation we propose uses extensively the technique of generating functions \cite{Wilf_1994}, and is a variation on the following theme : consider the known expression for the factorial moments of the Poisson distribution,
\beq\label{facmoment}
\av{n(n-1)\cdots (n-m +1)}  = \mu^m.
\enq
Even though it may appear mysterious at first sight, a simple way to prove this identity is to notice
\beq
\av{n(n-1)\cdots (n-m +1)}  =  \left.\frac{d^m}{dt^m}G(t)\right|_{t = 1},\quad G(t) := \sum_{n = 0}^{\infty}p(n)t^n,
\enq
where $G(t)$ is called the probability generating function, and to try and evaluate the right hand side. This is indeed very convenient, since the probability generating function of the poisson law takes a very simple form,
\beq
G(t) =  e^{-\mu}\sum_{n = 0}^{\infty}\frac{\mu^n}{n!}t^n  = e^{\mu \lp t -1\rp }.
\enq
The derivatives are trivial to evaluate, proving (\ref{facmoment}). We will need the following result, that comes out directly from an essentially identical argument,
\beq \label{avfallingfactorial}
\av{(an)_m}  = \left.\frac{d^m}{dt^m}e^{\mu(t^a-1)}\right|_{t = 1},
\enq
where $a$ is some number.
\newline\newline
We now turn to the evaluation of
\beq
\sum_{k = 0}^nC_{nk}k\:m_k.
\enq
This sum can be written as the first derivative with respect to $a$ evaluated at $a = 1$ of the following expression
\beq
\av{c_n(ax)} = \sum_{k = 0}^\infty  \frac{e^{-\mu}\mu^k}{k!}c_n(ak),
\enq
as can be seen directly from an expansion of the Charlier polynomials $c_n$ in terms of the coefficients $C_{nk}$. Using equation (\ref{Charlier}) and our result (\ref{avfallingfactorial}), we obtain
\beq \label{eq}
 \sum_{k = 0}^nC_{nk}k\: m_k = e^{-\mu} \sum_{k = 0}^n(-1)^{n-k}\mu^{-k}\bin nk \left.\frac{d}{da}\frac{d^k}{dt^k}\exp\lp \mu t^a \rp\right|_{t,a= 1}.
\enq
The derivative with respect to $a$ is easily performed :
\beq
\left.\frac{d}{da}\exp\lp \mu t^a \rp\right|_{a= 1} =\mu\:  e^{\mu t} \:t \ln t.
\enq
Also, using Leibniz rule for derivatives of products, we can write
\beq
\left. \frac{d^k}{dt^k}\exp\lp \mu t \rp \:t \ln t \right |_{t= 1} = e^\mu\sum_{i = 0}^k \bin  k i \mu^{k-i} \left.\frac{d^i}{dt^i} \:t \ln t\right|_{t = 1}.
\enq
The factor of $\mu^k$ cancels in equation (\ref{eq}), so that
\beq
 \sum_{k = 0}^nC_{nk}k\: m_k  = \mu \sum_{k =0}^{n} \sum_{i =0}^{k}\bin nk \bin ki (-1)^{n-k}\mu^{-i}\left.\frac{d^i}{dt^i} \:t \ln t\right|_{t = 1}.
\enq
From the properties of the binomial coefficients follows that the sum over $k$ is just $(-1)^n\delta_{ni}$. Therefore,
\beq
s_n(\ln A) =\mu \frac{\mu^{-n/2}}{\sqrt {n!}} \left.\frac{d^n}{dt^n} \:t \ln t\right|_{t = 1}.
\enq
The derivatives are easily computed :
\beq
\left.\frac{d^n}{dt^n} \:t \ln t\right|_{t = 1} = \begin{cases} 0 & n = 0 \\ 1 & n = 1 \\ (-1)^n(n-2)! & n \ge 2 \end{cases}
\enq
with the final result given in equation \eqref{snlnA}.
%%%% END DERIVATION POISSON %%%%%
\section{Indeterminate measures}\label{indeterm}
%%%%%%%%%%  INDETERM  %%%%%%%%%
We now turn to indeterminate distributions, i.e. those that cannot be uniquely recovered from their moments.
In this case, the Fisher information content of the moments will generally not converge to the total amount. In this respect, the limit
\beq
\lim_{N \rightarrow \infty} \frac{\sum_{n = 1}^{N}s_n^2(\alpha) }{I(\alpha)},
\enq
a number in $(0,1]$, may be thought of as an indirect measure of the amount of indeterminacy of the moment problem. A value of unity means that the moments do carry the same information on the parameter $\alpha$ as the probability density function, while for values close to zero a large amount of information on $\alpha$ is not present in the hierarchy.  The quantity $\sqrt{\epsilon(\alpha)}$ has via the information inequality the interpretation of the ratio of the expected constraints on $\alpha$ by extraction of the full set of moments to the best constraints achievable with the help of unbiased estimators of $\alpha$.
When more than one parameter are of interest, this definition is not really satisfactory anymore, since it is tied  to $\alpha$ exclusively. One can get around this by defining a ratio of determinants,
\beq
\epsilon := \lim_{N \rightarrow \infty} \epsilon_N = \lim_{N \rightarrow \infty}  \det F_{\le N}  / { \det  F   },
\enq
where $F_{\le N}$ was defined in equation \eqref{Fn}. Clearly, $\epsilon_N$ is the cumulative efficiency to catch the information. Since the matrices in the numerator and denominator do transform in the same way under any smooth reparametrisation of the parameters, or coordinates, of the family, this ratio is left unchanged under such transformations. Thus, $\epsilon$  and $\epsilon_N$ are well defined quantities associated to that family of distributions, independently of the chosen coordinates. 
\newline
Naively, one may expect this lost information to reflect in some way the freedom there is in the choice of a distribution with the very same series of moments. We will therefore compare our results to a measure of this freedom, $D_S$, that was proposed recently \cite{Stoyanov04}
 as the index of dissimilarity of a Stieltjes class S. A Stieltjes class is a family of  probability density functions of the form
 \beq
 p_\delta(x) = p(x)\lp1 + \delta h(x)\rp,\quad |h(x)| \le 1,\:\: |\delta| \le 1,
 \enq
 all having the same moment series as the central probability density function $p$.
 The index $D_S$, defined as
 \beq
 \int dx \:p(x) |h(x)|,
 \enq
 in $[0,1]$ is the maximal distance between two members of the class, being zero for determinate moment problems, where $h$ must identically vanish.
 \newline
 We will consider three types of probability density functions, the lognormal, which is indeterminate for any values of its parameter space, as well as the Weibull distribution and the stretched exponential, which are indeterminate solely for parts of their parameter range.
For these last two distributions we could not find in all cases exact analytical expressions for the coefficients $s_n$. We generated them therefore numerically, using a fine discretization procedure to obtain the orthogonal polynomials, following the exposition in \cite{Gautschi04}.
\subsection{Lognormal distribution}\label{lognormal}
%%%%%%%%%%  LOGNORMAL %%%%%%%%%
The lognormal distribution has the following functional form,
\beq
p(x,\mu_Y,\sigma_Y) = \frac{1}{\sqrt{2\pi}\sigma_Y}\frac 1 x \exp\lp -\frac1 2 \frac{\lp\ln x - \mu_Y\rp^2 }{\sigma_Y^2} \rp.
\enq
The parameters $\mu_Y$ and $\sigma_Y^2$ are the mean and the variance of $ y = \ln x$ which is normally distributed. They are related to the mean $\mu$ and variance $\sigma^2$ of $x$ by the relations
\beq
\begin{split}
\mu_Y &= \ln \mu - \frac 12 \ln \lp 1 + \frac{ \sigma^2}{ \mu^2} \rp \\
\sigma^2_Y &= \ln \lp 1 + \frac{\sigma^2}{\mu^2} \rp.
\end{split}
\enq
The only relevant parameter for our purposes is the reduced variance $\sigma^2 / \mu^2$, in terms of which our results can be expressed. The information coefficients associated to the parameters $\ln \mu$ and $\sigma^2 / \mu^2$ we already derived in \cite{2011ApJ...738...86C}, with the help of $q$-series. These are given by 
\beq\label{snln}
\begin{split}
s_n(\ln \mu)& = (-1)^{n-1} \lp  \frac{q^n}{1-q^n} \rp^{1/2} \sqrt{\pochh q q {n-1}} \\
s_n(\sigma^2 / \mu^2) &= q(-1)^n\lp  \frac{q^n}{1-q^n} \rp^{1/2} \sqrt{\pochh q q {n-1}} \lp\sum_{k = 1}^{n-1} \frac{q^k}{1-q^k} \rp.
\end{split}
\enq
In these equations,
\beq
q = \frac{1}{1 + \sigma^2/\mu^2}
\enq
and
\beq
\pochh q q n = \prod_{k = 1}^n\lp 1 -q^k \rp
\enq
is the q-Pochammer symbol \cite{Andrews99}.
According to the chain rule of derivation, we obtain $s_n(\mu_Y) = s_n(\ln \mu)$ and $s_n(\sigma_Y^2) = \frac 12(s_n(\ln \mu) + s_n(\sigma^2/\mu^2))$. On the other hand, since $\ln x$ is normally distributed, the total Fisher information matrix $F$ associated to $\mu_Y$ and $\sigma^2_Y$ is diagonal with $1/\sigma^2_Y$ and $1/ 2\sigma^4_Y$ as diagonal elements. It follows that in these coordinates  $\det F = 1/(2\sigma^6_Y)$.
\newline
The Stieltjes class we consider is set by
\beq \label{Stln}
h(x) = \sin\lb \frac{2\pi}{\sigma_Y^2} \lp \ln x - \mu_Y \rp \rb.
\enq
Others are given in \cite{Heyde63} but are equivalent to a uninteresting rescaling of $\sigma_Y$.
After an obvious variable substitution, the dissimilarity index becomes
\beq \label{DSln}
D_S = \frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty \exp \lp-\frac{x^2}{2} \rp\left | \sin\lp \frac{2\pi}{\sigma_Y}x \rp\right|\: dx. 
\enq
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=10cm]{figs/lnnormal}
\caption{Solid lines : the cumulative efficiency $\epsilon_N$, for $N = 2,5,10,15$ and $1000$, from bottom to top, as function of the reduced variance of the lognormal distribution. Dashed : The dissimilarity index for the Stieltjes class given in  equation \eqref{Stln}.}
\label{fig:ln}
\end{center}
\end{figure}
In figure \ref{fig:ln}, we show the cumulative efficiency $\epsilon_N$, for $N = 2,5,10,15$ and $1000$ for the lognormal family, evaluated with the exact expressions given in \eqref{snln}, solid lines from bottom to top, together with the dissimilarity index $D_S$, shown as the dashed line, evaluated by numerical integration of equation \eqref{DSln}.
It is not difficult to see from the above expressions that the coefficients $s_n$ decay exponentially for large $N$, such that the convergence is rather quick over the full range.
We observe a very sharp transition in $\epsilon$ as  soon as the reduced variance approaches unity, from a regime where the entire information content is within the second moment, as for the normal distribution (and thus where the indeterminacy of the moment problem is irrelevant for parameter estimation),  to the opposite regime where all moments completely fail to capture the information. This cutoff is discussed in more details in \cite{2011ApJ...738...86C}.  On the other hand. the index $D_S$ is seen to be remarkably constant over the range shown, equal to its limiting values for $\sigma_Y \rightarrow 0$, which can be evaluated from \eqref{DSln} to be $2/\pi$.
%%%%%%%%%%  WEIBULL  %%%%%%%%%
\subsection{Weibull distribution}
%%%%%%%%%%  WEIBULL  %%%%%%%%%
We consider now the Weibull distribution with shape parameter $k$ and scale parameter $\lambda$,
\beq
p(x,\lambda,k)= \frac k \lambda  \lp\frac{x}{\lambda}\rp^{k-1}e^{- (x/\lambda) ^k}, \quad x,\lambda,k > 0.
\enq
The variable $x$ can be seen as a power of an exponentially distributed variable with intensity unity, $
p(t) = e^{-t}$, for $ t =  \lp \frac x \lambda \rp^{k}$. It is known that the moment problem  associated to the moments of $x$ is determinate for $k \ge 1/2 $ and indeterminate  for $k < 1/2$ \cite[section 11.3 e.g.]{Stojanov87}. A Stieltjes class in the latter regime is provided in the same reference, which after some algebraic manipulations reduces to
\beq \label{StW}
h(x) = \sin \lp c_k (x/\lambda)^k - k\pi \rp,\quad c_k= \tan\lp  k \pi \rp,
\enq
The index $D_S$ becomes
\beq
D_S = \int_0^\infty e^{-t} \left| \sin \lp c_k \: t - k\pi\rp  \right|\:dt.
\enq
It is interesting to note that this integral can be performed analytically, for instance with the help of partial integration, with the result
\beq
D_S = \sin\lp k\:2\pi\rp \frac{e^{-k\pi / c_k}}{1 - e^{-\pi/c_k}}.
\enq
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=10cm]{figs/Weibull}
\caption{Solid lines : the cumulative efficiencies $\epsilon_N$, for $N = 2,5,10,25$, from bottom to top, as function of $\sigma/\mu$ for the Weibull distribution. Dashed : The dissimilarity index for the Stieltjes class given in  equation \eqref{StW}. The vertical dashed line, corresponding to $k = 1/2$, separates the regimes of determinacy and indeterminacy of the associated moment problem.}
\label{fig:W}
\end{center}
\end{figure}
We evaluated $\epsilon_N$ using the convenient coordinates  $\ln \lambda$ and $\ln k$, and the associated $F_{\le N}$ numerically. It is not difficult to see that $\epsilon_N$ is independent of $\lambda$. The full information matrix for these parameters can be evaluated analytically, with the result $\det F = k\pi^2/6$.  The results for $\epsilon_N$ are shown in figure \ref{fig:W}, that we present as for the lognormal as function of the reduced variance
\beq
\frac \sigma \mu = \lp \frac{\Gamma \lp 1 + 2/k \rp}{\Gamma^2 \lp 1 + 1/k \rp} - 1 \rp^{1/2}.
\enq
The dashed vertical line corresponding to $k = 1/2$ separates the two regimes where, on the left, $\epsilon$ is unity and $D_S$ zero since the moment problem is determinate, and on the right, where the moment problem is indeterminate. The scale $\sigma/ \mu = 1$ corresponds to $k = 1$.\newline
While the decay of $\epsilon_N$ is also very sharp in the indeterminate regime, very slow convergence of $\epsilon_N$ is seen to occur in the large reduced variance regime unlike for the lognormal distribution. This also in the region $1 < k <2 $, which corresponds to the phase where the Weibull distribution goes from a unimodal to a monotonically decreasing distribution, but $\epsilon$ still is unity, since the moment problem still is determinate. For instance, for $k = 1$, the following exact result can be gained with the same methods as exposed in this paper,
\beq
\left. \epsilon_N \right|_{k = 1} = \lp \sum_{n = 1}^{N-1}\frac 1 {n^2}  \rp\frac 6 {\pi^2}.
\enq
%%%%%%%%%% Stretched exp. %%%%%%%%%%%%%
\subsection{Stretched exponential function}
%%%%%%%%%% Stretched exp. %%%%%%%%%%%%%
Finally, we treat the case of the stretched exponential,
\beq
p(x,\lambda,k) =  \frac{k}{\lambda \Gamma(1/k)} e^{-(x/\lambda)^k}.
\enq
Just as for the Weibull distribution, the moment problem  associated to the moments of $x$ is determinate for $k \ge 1/2 $ and indeterminate  for $k < 1/2$ \cite[section 11.4]{Stojanov87}
A Stieltjes class is given by
\beq \label{StS}
h(x) = \sin\lp c_k (x/\lambda)^k\rp,\quad x \ge 0,\:k > 0
\enq
where $c_k$ is as above given by $c_k = \tan \lp k \:\pi\rp$.
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=10cm]{figs/Stretchexp}
\caption{Solid lines : the cumulative efficiencies $\epsilon_N$, for $N = 2,5,10,25$, from bottom to top, as function of the inverse shape parameter $1/k$ of the stretched exponential. Dashed : The dissimilarity index for the Stieltjes class given in  equation \eqref{StS}. The vertical dashed line at $k = 1/2$ separates the regimes of determinacy and indeterminacy of the associated moment problem.}
\label{fig:S}
\end{center}
\end{figure}
Numerical evaluation of $\epsilon_N$, and of the dissimilarity index is shown in fig \ref{fig:S}. As for the Weibull distribution, these results are independent of the scale parameter $\lambda$.
%%%%%%%%%%%%%%%%%%%%%


\section{Derivation for the beta distribution}\label{appendixbeta}
In the following we will need the first two derivatives of the logarithm of the gamma function. These are called the digamma $\psi_0$ and trigamma $\psi_1$ functions respectively \cite[p. 258-260]{abramowitz70a},
\beq
\begin{split} \label{ditrigamma}
\psi_0(x) &= \frac{d}{dx}\ln \Gamma(x) \\
\psi_1(x) &= \frac{d^2}{dx^2}\ln \Gamma(x).
\end{split}
\enq
The Fisher information matrix can be gained by noting that by differentiation under the integral sign, we have
\beq
\begin{split}
\Fab = \frac{\partial^2\ln B(\alpha,\beta)}{\partial\alpha\partial\beta} .
\end{split}
\enq
Using the representation (\ref{betagamma}), we conclude that
\beq
F = 
\bem 
\psi_1(\alpha) & 0 \\ 0 & \psi_1(\beta)
\enm
- \psi_1(\alpha + \beta)
\bem 1 & 1 \\1 & 1
\enm.
\enq
To obtain the information coefficients $s_n(\alpha)$ and $s_n(\beta)$. It turns out it is more convenient to start with $s_n(\beta)$. $s_n(\alpha)$ will then be gained effortlessly by looking at the symmetry of the problem.
\newline\newline
From the definition of the beta integral (\ref{betaintegral}), the moments of the beta distribution are given by
\beq
m_k = \frac{B(\alpha + k, \beta)}{B(\alpha,\beta)}.
\enq
The derivatives of the moments with respect to $\beta$ are given by
\beq \label{dermoments}
\begin{split}
%\partial_\alpha \ln m_k& = \psi_0(\alpha + k) - \psi_0(\alpha + \beta + k) - \psi_0(\alpha) + \psi_0(\alpha + \beta) \\
\partial_\beta \ln m_k &= - \psi_0(\alpha + \beta + k) +  \psi_0(\alpha + \beta).
\end{split}
\enq
\newcommand{\Jac}[2]{P_n^{(#1-1,#2 - 1)}}
\newcommand{\Gj}[2]{G_n^{(#1,#2)}}
The orthogonal polynomials are the Jacobi polynomials $\Gj \alpha \beta (x)$ \cite[page 774]{abramowitz70a}. Instead of the parameters $p,q$ used in \cite{abramowitz70a}, we stick to $\alpha$ and $\beta$, which are more appropriate for our purposes \footnote{We have in the notation of  \cite{abramowitz70a} $q = \alpha, p = \alpha + \beta -1$}. These polynomials are proportional to the Jacobi polynomials $\Jac \alpha \beta (2x -1)$ \cite[chap. IV]{Szego39}, orthogonal on the interval $(-1,1)$.
Their matrix elements of $G_n$ are given expliclity by
\beq
C_{nk} = \frac{\Gamma(\alpha + n)}{\Gamma(\alpha + \beta + 2n - 1)} (-1)^k\bin nk \frac{\Gamma(\alpha + \beta + k +n -1 )}{\Gamma(\alpha + k)}.
\enq
We first note the following relation,
\beq \label{cnkmk}
C_{nk}m_k = \frac{\Gamma(\alpha + n)\Gamma(\beta)}{\Gamma(2n + \alpha + \beta -1)B(\alpha,\beta)} (-1)^{n-k}\bin nk  \lp \alpha + \beta + k\rp^{(n-1)},
\enq
where
\beq
(x)^{(n)} = x(x+1)\cdots(x + n - 1)
\enq
is the rising factorial. Since $s_n(\beta)$ is given by
\beq\label{s_nb}
s_n(\beta) = \sum_{k = 0}^n C_{nk}m_k \partial_\beta \ln m_k,
\enq
the evaluation of the following sum is necessary, 
\beq
A_n(q) :=\sum_{k = 0}^n\bin nk (-1)^{n-k}\lp q + k\rp^{(n-1)} \lp \psi_0(q + k) - \psi_0(q) \rp,\quad q := \alpha + \beta > 0.
\enq
The following paragraphs are dedicated to the lengthy but straightforward proof of the following result,
\beq\label{anq}
A_n(q) = \frac{(n -1) !}{q + n -1}.
\enq
The proof consists of a number of steps.
\paragraph{Step 1 :} 
Using an always useful trick, we turn the rising factorial in the sum into a power and differentiate. From
\beq
(q + k)^{(n-1)} = (q + k)\cdots (q + k + n - 2) = \left.\frac{d^{n-1}}{dt^{n-1}} \right|_{t = 1} t^{k + q  + n - 2},
\enq
follows
\beq
\begin{split}
A_n(q) &= \left.\frac{d^{n-1}}{dt^{n-1}}\right|_{t = 1}  t^{q + n-2} \sum_{k = 0}^n\bin nk (-1)^{n-k}t^k (\psi(q + k) - \psi(q)) \\
&=:\left.\frac{d^{n-1}}{dt^{n-1}}\right|_{t = 1}  t^{q + n-2} f_q(t). \label{defft}
\end{split}
\enq
We then perform the derivatives can be performed using the Leibniz rule. Since
\beq
\left.\frac{d^{n - 1 - m}}{dt^{n-1-m}}\right|_{t = 1}  t^{q + n-2} = \frac{\Gamma(q + n - 1)}{\Gamma(q + m)},
\enq
one obtains
\beq \label{Anq}
A_n(q) = \Gamma(q + n -1)\sum_{m= 0}^{n-1}\bin {n-1}{m} \frac{ f_q^{(m)}(t = 1) }{\Gamma(q + m)}.
\enq
\paragraph{Step 2}
To obtain $f_q^{(m)}(1)$, we first construct an integral representation of the function $f_q(t)$. From the relation \cite[theorem 1.2.7]{Andrews99}
\beq
\psi_0(q + 1) = \frac 1 q + \psi_0(q)
\enq
of the digamma function, we note that
\beq
\psi_0(q + k) - \psi_0(q) = \sum_{j = 0}^{k-1}\frac{1}{q + j}.
\enq
Writing
\beq
\frac 1 {q + j } = \int_0^{1} dx\: x^{q + j -1},
\enq
the sum over $j$ becomes a geometric series.
We obtain therefore,
\beq
\psi_0(q + k) - \psi_0(q) = \int_0^1dx\:x^{q-1}\frac{1 - x^k}{1-x}.
\enq
We can now perform the sum over $k$ in $f_q(t)$. We have indeed
\beq
\sum_{k = 1}^{n}\bin nk (-1)^{n-k} t^k (1-x^k) = (t-1)^n + (-1)^n (1 - tx)^n.
\enq
It follows immediately
\beq \label{ftbeta}
f_q(t) = \int_0^1dx\: x^{q-1}\frac{(t-1)^n -(-1)^n(1-tx)^n}{ 1- x}.
\enq
We only need derivatives of that function evaluated at $t = 1$. The order of each derivative is $< n$. For this reason the term $(t-1)^n$ in this expression actually plays no role. Each such derivative is thus a beta integral :
\beq\label{bb}
f_q^{(m)}(1) = (-1)^{n + m - 1}n\cdots (n - m + 1)B(q + m, n - m),\quad m < n.
\enq
\paragraph{Step 3 :}
To go further, we use the following property of the beta integral,
\beq
B(x,y) = \frac{(x + y)^{(n)}}{(y)^{(n)}}B(x,y +n), 
\enq
which can be seen from its representation in terms of the gamma function, or from its integral representation \cite[page 5]{Andrews99}. Two applications of this rule leads to
\beq
B(q + m,n - m) =  B(q,n)\frac{(q)^{(m)}}{m !}\frac{1}{\bin {n-1} m}.
\enq
By combining this relation with (\ref{bb}), and using
\beq
(q)^{(m)} = \frac{\Gamma(q + m)}{\Gamma(q)},
\enq
we have shown
\beq
f^{(m)}(1) = (-1)^{n + m -1}B(q,n) \frac{\Gamma(q+m)}{\Gamma(q)} \bin n m \frac{1}{\bin {n-1}m }.
\enq
This form is very convenient, since many terms now cancel in equation (\ref{Anq}). We obtain
\beq
A_n(q) = -\underbrace{B(q,n)\frac{\Gamma( n + q -1)}{\Gamma(q)}}_{\frac{(n-1)!}{n + q -1}} \sum_{m = 0}^{n-1}\bin nm (-1)^{n-m}.
\enq
The sum over $m$ would vanish would it run up to $n$. Its value is therefore minus the $m = n$ term, which is unity. It follows
\beq
A_n(q) = \frac{(n-1)!}{n + q -1},
\enq
which was to be proved.
\newline\newline
Getting $s_n(\beta)$ requires now only to keep track of the normalization.
The normalization of the Jacobi polynomials $G_n$ \cite{abramowitz70a} is 
\beq
h_n  = \frac{n!}{B(\alpha,\beta)} \frac{\Gamma(\alpha + n)\Gamma(\alpha + \beta -1 + n)\Gamma(\beta + n)}{(\alpha + \beta - 1 + 2n)\Gamma^2(\alpha + \beta  -1 + 2n)}.
\enq
(Note that there is a additional factor of $1/B$ with respect to \cite{abramowitz70a} since there the measure is not normalized to unit integral).
We have from equations (\ref{dermoments}), (\ref{cnkmk}), (\ref{s_nb}) and (\ref{anq}) together with some algebra
%\beq
%s_n(\beta) = \frac{1}{\sqrt {h_n}}\frac{\Gamma(\alpha + n) \Gamma(\beta)}{\Gamma(2n + \alpha + \beta -1)B(\alpha,\beta)}\frac{(n-1)!}{q + n - 1}.
%\enq
\beq
s_n(\beta) = - \frac {1}{n} \lp \frac{(\alpha)^{(n)}n!}{(\beta)^{(n)}(\alpha + \beta)^{(n)}} \rp^{1/2} \lp \frac{2n + \alpha + \beta -1}{n + \alpha + \beta -1} \rp^{1/2}.
\enq
Tedious calculations are not needed to get $s_n(\alpha)$, but symmetry considerations are enough.
The Jacobi polynomials obeys the symmetry relation,
\beq
\Jac \alpha \beta(-x) = (-1)^n\Jac \beta \alpha (x),
\enq
and therefore
\beq
\Gj \alpha\beta(1-x) = (-1)^n\Gj \beta \alpha (x).
\enq
It is then not difficult\footnote{for instance from the representation (\ref{sn}) } to see that $s_n(\alpha)$ is proportional to $s_n(\beta)$ with $\alpha$ and $\beta$ exchanged.
We conclude
\beq
s_n(\alpha) = - \frac {(-1)^{n}}{n} \lp \frac{(\beta)^{(n)}n!}{(\alpha)^{(n)}(\alpha + \beta)^{(n)}} \rp^{1/2} \lp \frac{2n + \alpha + \beta -1}{n + \alpha + \beta -1} \rp^{1/2}.
\enq




==> chapter3.tex <==
%\setprelude{\uppercase{A\scriptsize{n inconceivably numerous host of stars must be here arranged\\ together }\normalsize{[...],}\scriptsize{ because their free positions towards each other\\ would otherwise have presented irregular forms and not exact\\ figures}}\normalsize{.}
%\vspace{5truemm}\\
%\normalsize{Immanuel Kant, {\it Universal History and Theory of the Heavens} \cite{kant1755}}}

\chapter{Application to the cosmological matter density and convergence field}
\label{ch3}

\begin{center}
Parts of ...
\end{center}


\section{Introduction \label{introduction}}
The cosmological matter density field is becoming more and more directly accessible to observations with the help of weak lensing  \citep{1992grle.book.....S,2001PhR...340..291B,2003ARA&A..41..645R,2006astro.ph.12667M}. Its statistical properties are the key element in trying to optimize future large galaxy surveys aimed at answering actual fundamental cosmological questions, such as the nature of the dark components of the universe \citep{2009Natur.458..587C,2008ARA&A..46..385F}. To this aim, Fisher's measure of information on parameters \citep{fisher25,Rao,vandenbos07} has naturally become of standard use in cosmology. It provides indeed an handy framework, in which it is possible to evaluate in a quantitative manner the statistical power of some experiment configuration aimed at some observable \citep[e.g.]{1997ApJ...480...22T,Tegmark97,1999ApJ...514L..65H,2004PhRvD..70d3009H,2007MNRAS.381.1018A,2007MNRAS.377..185P,2006astro.ph..9591A,2009ApJ...695..652B}. Such studies are in the vast majority of cases limited to Gaussian probability density functions, or perturbations therefrom, and deal mostly with the prominent members of the correlation function hierarchy \citep{1980lssu.book.....P}, or equivalently their Fourier transforms the polyspectra, such as the matter power spectrum.
\newline\noindent
The approach via the correlation function hierarchy is very sensible in the nearly linear regime for at least two reasons. First, in principle, the correlations are the very elements that cosmological perturbation theory is able to predict in a systematic manner (see \citep{2002PhR...367....1B} for a review, or the more recent \citep{2011PhRvD..83h3518M} and the numerous references in it). Second, primordial cosmological fluctuations fields are believed to be accurately described by the use of Gaussian statistics. It is well known that the correlations at the two-point level provide a complete description of Gaussian fields. It is therefore natural to expect this approach to be adequate throughout the linear and the mildly non linear regime, when departures from Gaussianity are small.
\newline\noindent
Deeper in the non linear regime, fluctuations grow substantially in size, and tails in the matter probability density function do form. A standard prescription for the statistics of the matter field in these conditions is the lognormal distribution, various properties of which are discussed in details in an astrophysical context in \citep{1991MNRAS.248....1C}. It was later shown to be reproduced accurately, both from the observational point of view as well as in comparison to standard perturbation theory and N-body simulations \citep{1995ApJ...443..479B,1994A&A...291..697B,2001ApJ...561...22K,2000MNRAS.314...92T,2005MNRAS.356..247W}, in low dimensional settings. More recently, it was used as a starting point for a tentative of a better description of clustering \citep{2010arXiv1012.3168K}.  The lognormal assumption is also very much compatible with numerical works \citep{2009ApJ...698L..90N,2011ApJ...731..116N} showing that the spectrum of logarithm of the field $\ln 1 + \delta$ carries much more  information than the spectrum of $\delta$ itself. The first evaluation of the former within the framework of perturbation theory appeared recently \citep{2011arXiv1103.2166W}.
\newline\noindent
Lognormal statistics \citep[for a textbook presentation]{Aitchison57} are not innocuous. More specifically, the lognormal distribution is only one among many distributions that leads to the very same series of moments. This fact indicates that, going from the distribution to the moments, one may be losing information in some way or another. A fundamental limitation of the correlation function hierarchy in extracting the information content of the field in the non linear regime could therefore exist, if its statistics are indeed similar to the lognormal. This important fact was already mentioned qualitatively in \citep{1991MNRAS.248....1C}, but it seems no quantitative analysis is available at present.
\newline\noindent
 It is the purpose of this paper to provide first answers to these issues, in terms of Fisher information, looking at the details of the structure of the information within the lognormal field. It is built out of two main parts. \newline\newline
The first deals exclusively with the case of a single lognormal variable, illustrating the main aspects we want to point out in this work. We begin by presenting how to identify the independent bits of information that are contained in the successive moments of a distribution, with the help of orthogonal polynomials. We discuss the properties of this decomposition that are relevant for our purposes. The procedure is very similar to the decompositions presented in \citep{Jarrett84}, to which we refer for a more complete discussion on the properties of such expansions. In a second step, we perform this decomposition for the lognormal distribution, which can be obtained exactly at all order in terms of $q$-series, due to its convenient analytical properties.  It contains one of our main results, presented in figure \ref{fig1} : when the variance of the fluctuations of the lognormal distribution reaches unity, essentially the entirety of its information \footnote{Throughout this work, by 'information' is meant  more rigorously Fisher information.} content cannot be accessed anymore through a study of its moments, even if  the complete series of moments could be extracted. We then delve a little bit more into the details of that phenomenon, and show that this is due to the inability of polynomials to reproduce the logarithm function, leading to missing bits of information in the part of the distribution describing the underdense regions. Finally, we perform a comparison of our results for the lower order moments with results \citep{1994A&A...291..697B} from standard perturbation theory, and find good agreement over several orders of magnitude in the variance.
\newline\newline
The second part extends the analysis to the multivariate lognormal distribution, and to the continuous limit of the lognormal field. The decomposition of the information into uncorrelated pieces is conceptually identical. Due to the highly increased formal complexity, the explicit expressions for the information content of the $n$-points correlations are however of less practical use. We therefore focus on two simpler situations that can be dealt with analytically, dealing with the extraction of the mean of a lognormal field and two point correlations.\newline \newline
We then summarise the results, and conclude with a discussion on the conditions for the correlation function hierarchy to form a complete or incomplete, efficient or inefficient set of probes of a random field. The appendix contains a short series of technical details regarding the material presented in the main text.
\newline\indent
\section{One variable}
%\subsection{Notation and conventions}
For a variable $X$, with probability density function $p(x,\alpha)$, $\alpha$ any parameter, we are assuming that all moments exist, write for them
\beq
m_n =  \av{x^n},\quad n  = 0,1,\cdots
\enq
and the associated covariance matrix with
\beq
\Sigma _{ij} = m_{i+j}- m_im_j
\enq
Since $p(x,\alpha)$ is normalised to unity for any value of the parameter, we have
\beq
\frac{\partial m_0}{\partial \alpha} =  0 = \av{s(x,\alpha)},
\enq
where $s(x,\alpha)  = \partial_\alpha \ln p(x,\alpha) $ is the score function.
Fisher's measure of information \citep{fisher25,vandenbos07} on the parameter $\alpha$ is then defined as the variance of the score function
\beq
F_\alpha = \av{ s^2(x,\alpha)}.
\enq
The Fisher information density
\beq \label{infdensity}
s^2(x,\alpha)p(x,\alpha)dx = \frac{\lp \partial_\alpha p(x,\alpha) \rp^2}{p(x,\alpha)}dx
\enq
is the amount of information associated to observations of realizations of the variable in the range $\lp x,x+dx \rp$. $F_\alpha$ itself has gotten through the Cram\'er-Rao inequality \citep{Rao} the widespread interpretation in cosmology of approximating the error bars the experiment under consideration will be able to put on the parameter $\alpha$ \citep[e.g.]{1997ApJ...480...22T}.
\subsection{Fisher information and orthogonal polynomials \label{s1}}
The decomposition of the information in independent pieces associated to each moment relies on the approximation of the score function through orthonormal polynomials. For each natural number $n$, $P_n$ is a polynomial of degree $n$ and
\beq \label{ortho}
\av{P_m(x)P_n(x)} = \delta_{mn}.
\enq
These polynomials  can always be constructed for a given distribution and are unique up to a sign, which is fixed by requiring the coefficient of $x^n$ in $P_n$ to be positive.  We refer to the textbooks \citep{Szego39,Freud71} for the general theory of orthogonal polynomials. These polynomials can be written in the monomial basis with the help of a triangular transition matrix $C$ that we will use later on,
\begin{equation} \label{cmatrix}
P_n(x)= \sum_{m = 0}^n\:C_{nm}\:x^m.
\end{equation}
According to equation (\ref{ortho}), it holds that the non constant orthogonal polynomials average to zero. As the value of the model parameter changes,  these averages take non vanishing values, at a rate which is equal to the component of the score function parallel to these polynomials :
\beq \label{scoeff}
\frac{\partial \av{P_n(x)}}{\partial \alpha}  = \av{s(x,\alpha) P_n(x)} =: \ca n,
\enq
where the relation $\partial_\alpha p(x,\alpha) = s(x,\alpha)p(x,\alpha)$ was used.
We argue that $s_n^2$ is precisely the independent information content of the moment of order $n$. This can be seen as the following. For any natural number $n$, it is not difficult to show that the inverse covariance matrix of size $n$ is given by
\beq
\lb \Sigma^{-1}\rb_{ij} = \lb C^TC \rb_{ij},\quad i,j = 1,\cdots,n.
\enq
Therefore, noting that from equation (\ref{cmatrix}) and from the definition (\ref{scoeff}) of the information coefficients $s_n$ we can write
\beq \label{scoeff2}
s_n = \sum_{k = 1}^nC_{nk}\frac{\partial m_k}{\partial \alpha},
\enq
the following relation holds,
\beq \label{infn}
\sum_{i = 1}^n s_i^2 =  \sum_{i,j = 1}^n\frac{\partial m_i}{\partial \alpha}\lb \Sigma^{-1}\rb_{ij}\frac{\partial m_j}{\partial\alpha}.
\enq
This expression, weighting the sensitivity of the moments to the parameter by the covariance matrix, is the amount of information present in the first $n$ moments, taking all correlations into account. For instance, this is exactly the amount of information available, if the first $n$ moments were to be extracted, with the help of unbiased, Gaussian distributed estimators \citep[e.g.]{1997ApJ...480...22T}. Also, it is simple to show that these coefficients are invariant under any linear transformation of the field. This allow us to identify unambiguously the $n$th squared coefficient as the independent bits of information contained in the moment of order $n$.
\newline\newline
If the set of orthonormal polynomials forms a complete basis, the partial sums
\beq \label{series}
\sum_{n = 1}^N s_nP_n(x)
\enq
will tend, with increasing $N$, to reproduce accurately the score function. By Parseval identity, the full amount of Fisher information can be written as
\beq
F_\alpha = \sum_{n = 1}^\infty s_n^2.
\enq
This last equation implies that the information contained in the full set of moments is identical to the total amount of information.
This is certainly in perfect agreement with expectations. A well known result due to M. Riesz \citep{Riesz23} in the theory of moments states namely that if the moment problem associated to the moments $\left \{m_i \right\}_{i = 0}^\infty$ is determinate, (i.e. the distribution giving rise to these moments is uniquely determined by their values), then the set of associated orthonormal polynomials is complete. Since the distribution is uniquely determined, common sense would require then the total amount of information contained in the distribution to be the same as the one contained in the full set of moments.
\newline\newline
However, moment problems are not always determinate, and orthonormal polynomials associated to weight functions do not always form complete sets. Therefore, the series
\beq
f_\alpha := \sum_{n = 1}^\infty s_n^2
\enq
may not always converge to the total amount of Fisher information, and, if not, will always underestimate it. We have namely, instead of Parseval's identity, the Bessel inequality,
\beq \label{MSE} \begin{split}
0 & \le \av{\: \lp \sum_{n = 1}^\infty \ca n P_n(x) - s(x,\alpha) \rp^2} \\
&= F_{\alpha} - f_\alpha.
\end{split}
\enq
In words, the mean squared error in approximating the score function with polynomials is the amount of Fisher information absent from the full set of moments. As emphasized already in a astrophysical context by \citep{1991MNRAS.248....1C} and stated in our introduction the moments of the lognormal distribution are precisely an example of an indeterminate moment problem. In fact, a whole family of distribution, given explicitly in \citep{Heyde63}, do have the very same series of moments. In light of these considerations, our subsequent results cannot be considered as surprising.
\newline Before turning to the actual calculation of the coefficients $s_n$ of the lognormal distribution, let us just state that when the score function is itself a polynomial, it is clear that the series (\ref{series}) actually terminates,
\beq
s_k = 0 ,\quad k > n  
\enq
where $n$ is the order of the polynomial representing the score function. The prime example being the Gaussian distribution, for which $n = 2$, with associated orthonormal polynomials the Hermite polynomials. The well known fact that the mean and the variance of the Gaussian distribution carry all of the information becomes within our framework that only the coefficients $s_1$ and $s_2$ are non-zero. % For further reference, we give the two information coefficients for the Gaussian distribution with mean $\mu$ and variance $\sigma^2$,
%\beq
%\begin{split}
%s_1 &= \frac 1 {\sigma}\frac{\partial \mu}{\partial \alpha} \\
%s_2 &= \frac 1{\sqrt 2} \frac 1 { \sigma^2} \frac{\partial \sigma^2}{\partial \alpha},
%\end{split}
%\enq
%leading indeed to the standard expression for the Fisher information of the Gaussian distribution
%\beq \label{fgauss}
%F_\alpha = \frac{1}{\sigma^2}\lp \frac{\partial \mu }{\partial \alpha} \rp^2 +  \frac{1}{2\sigma^4}\lp \frac{\partial \sigma^2 }{\partial \alpha} \rp^2.
%\enq
\subsection{Basic properties of the lognormal distribution}
The variable $X$ has a lognormal distribution when $Y = \ln X$ is a normal variable, with mean $\mu_Y$ and variance $\sigma^2_Y$. The dependency on a model parameter $\alpha$ can enter one or both of these parameters.
The moments of $X$ are given by Gaussian integrals and read explicitly
\beq \label{moments}
m_n =  \exp \lp n\mu_Y + \frac 12 n^2\sigma^2_Y\rp.
\enq
The mean and variance of $Y$ relate therefore to the mean $\mu$ and variance $\sigma^2$ of $X$ according to
\beq \label{rel}
\begin{split}
\sigma^2_Y &= \ln \lp 1 + \sigma^2_\delta \rp \\
\mu_Y &= \ln \mu - \frac 12 \ln \lp 1 + \sigma^2_\delta \rp,
\end{split}
\enq
where $\sigma^2_\delta$ is the variance of the fluctuations of $X$,
\beq
\sigma_\delta^2 = \frac{\sigma^2}{\mu^2}.
\enq
Since $Y$ is has a Gaussian distribution and Fisher's measure is invariant under invertible transformations, the total Fisher information content of $X$ is given by the well known expression for the Gaussian distribution,
\begin{equation} \label{exactlnnormal}
F^X_{\alpha} = \frac{1}{\sigma^2_Y}\lp \frac{\partial \mu_Y}{\partial \alpha} \rp^2 + \frac 1 {2\sigma^4_Y} \lp \frac{\partial \sigma^2_Y}{\partial \alpha} \rp^2.
\end{equation}
The key parameter throughout this part of this work  will be the quantity $q$, defined as
\beq
q := e^{-\sigma^2_Y} = \frac{1}{1 + \sigma^2_\delta}. 
\enq
Note that $q$ is strictly positive and smaller than unity.  The regime of small fluctuations, where the lognormal distribution is very close to the Gaussian distribution is described by values of $q$ close to unity. Deep in the non linear regime, it tends to zero. These two regimes are conveniently separated at $q = 1/2$, corresponding to fluctuations of unit variance. We note the following convenient property of the moments for further reference,
\beq \label{separability}
m_{i + j} = m_im_j \:q^{-ij}.
\enq
\subsection{Information coefficients}
From equations (\ref{scoeff2}), (\ref{moments}), and (\ref{rel}), we see that the $n$-th information coefficient $s_n$ is given by
\beq \label{infcoeff} \begin{split}
s_n &= \frac{\partial \ln \mu}{\partial \alpha} \sum_{k = 0}^n C_{nk}\:m_k \:k \\
&+ \frac 1{2\lp 1 + \sigma^2_\delta\rp}\frac{\partial \sigma^2_\delta}{\partial \alpha} \sum_{k = 0}^n C_{nk}\:m_k \:k(k-1). 
\end{split}
\enq
Evaluation of the above sums can proceed in different ways. Notably, it is possible to get an explicit formula for the orthonormal polynomials, and therefore of the matrix $C$, for the lognormal distribution. These are essentially the Stieltjes-Wigert polynomials \citep{Wigert23,Szego39}. We will namely use their specific form later in this work, though they are not needed for the purpose of evaluating (\ref{infcoeff}). We proceed with the following trick : we introduce the $q$-shifted factorial , also called $q$-Pochammer symbol \citep[ section 10]{Kac02,Andrews99}, as
\beq
\pochh t q n = \prod_{k = 0}^{n-1}\lp 1 - tq^k\rp,\quad \pochh t q 0  := 1
\enq
%and the Gaussian binomial coefficient as
%\beq
%\binq n k q = \frac{\pochh q q n }{\pochh q q k \pochh qq {n-k}}.
%\enq
%These are the building blocks of the Cauchy binomial theorem, which we state for future reference,
%\begin{equation} \label{Cauchybinomialtheorem}
%\pochh t q n = \sum_{k = 0}^n \binq n k q q^{k(k - 1)/2}(-t)^k,
%\end{equation}
%which is a generalisation of the more usual binomial expansion of $(1 - t)^n$, to which it reduces when $q$ approaches unity. The transition matrix to the monomial basis reads
%\beq
%C_{nk}\:x^k =  \lp -1\rp^{n + k} \frac{q^{n/2}}{\sqrt{\pochh q q n}} q^{k^2} \binq n k q \lp \frac{x }{\mu}\rp^{k} ,
%\enq
%and satisfies the important relation, using relations (\ref{moments}) and (\ref{Cauchybinomialtheorem})
%\begin{equation}\label{cauchylog}
%\sum_{k = 0}^n C_{nk}\:m_k \:t^k = \pochh t q n.
%\end{equation}
$t$ a real number, and prove in the appendix that the following curious identity holds,
\beq \label{lemma}
\av{P_n(tx)} =(-1)^n\frac{q^{n/2}}{\sqrt{ \pochh qqn }} \pochh t q n.
\enq
By virtue of
\beq
\av{P_n(tx)} = \sum_{k = 0}^nC_{nk}\:m_k\:t^k.
\enq
it follows from our identity (\ref{lemma}) that the sums given in the right hand side of equation (\ref{infcoeff}) are proportional to the first, respectively the second derivative of the $q-$Pochammer symbol evaluated at $t = 1$. Besides, matching the powers of $t$ on both sides of equation (\ref{lemma}) will provide us immediately the explicit expression for the matrix elements $C_{nk}$.
\newline
\newline\newline
We distinguish explicitly two situations, labelled by an index $a$ taking values $\mu$ or $\sigma$, where only one of the two parameters of the lognormal distribution actually depends on $\alpha$. The general case being reconstructed trivially from these two. 
\paragraph{case $a = \mu$} We assume in this case that the parameter enters the mean of the distribution only,
\beq
\frac{\partial \sigma^2_\delta}{\partial \alpha} = 0
\enq
From (\ref{infcoeff}), we see that the derivative of  $\mu$ with respect to $\alpha$ only plays the role of an overall normalization constant. Since we will deal exclusively with ratios, it is irrelevant for our purposes.  We choose for convenience
\beq
\quad \frac{\partial \ln \mu}{\partial \alpha} = 1.
\enq
The total amount of information in the distribution becomes, from (\ref{exactlnnormal}) and (\ref{rel}),
\beq \label{Fmuex}
F_\alpha^\mu := \frac{1}{\ln \lp  1 + \sigma^2_\delta\rp}.
\enq
\paragraph{case $a = \sigma$}The parameter enters the variance of the distribution only, and we pick again a convenient normalization of its derivative
\beq
\frac 1{2\lp 1 + \sigma^2_\delta\rp} \frac{\partial \sigma^2_\delta}{\partial \alpha} = 1,\quad \frac{\partial \ln \mu}{\partial \alpha} = 0.
\enq
This situation is the most common in cosmology, for instance for any model parameter entering the matter power spectrum.
The exact amount of information becomes, again from (\ref{exactlnnormal}) and (\ref{rel}),
\beq \label{Fsigex}
F_\alpha^\sigma := \frac 1 {\ln \lp  1 + \sigma^2_\delta\rp}\lp 1  + \frac 2 {\ln\lp 1 + \sigma^2_\delta\rp} \rp.
\enq
\newline\newline
In both of these situations, we obtain the information coefficients (\ref{infcoeff}) by differentiating once, respectively twice, our relation (\ref{lemma}) with respect to the parameter $t$, and evaluating these derivatives at $t = 1$. The result is, in the $a = \mu$ case,
\begin{equation} \label{anbn}
\begin{split}
 s_n^\mu  = (-1)^{n-1}\sqrt{ \frac{q^n}{1 - q^n}\pochh q q {n-1} }
 \end{split}
 \end{equation}
 and for $a = \sigma$,
 \begin{equation}\label{Ansigma}
 \begin{split}
 s_n^\sigma  =  - 2s_n^\mu \lb \sum_{k = 1}^ {n-1} \frac{q^k}{1 - q^k}\rb ,\quad n > 1 
\end{split}
\end{equation}
whereas $s_{n = 1}^\sigma$ is easily seen to vanish from its definition.
%-----------------------------------------------------------------------------------------------
\newline\newline
\subsection{Incompleteness of the information in the moments}
The series
\beq \label{fmoments}
 f_\alpha^a =  \sum_{n =1}^\infty \lp s_n^a\rp^2 ,\quad a = \mu,\sigma
\enq
are the total amount of information contained in the full series of moments, in the respective cases described above. The ratios $\epsilon_\mu$ and $\epsilon_\sigma$, defined as
\beq
\epsilon_a := \frac{f_\alpha^a} {F^a_\alpha} ,\quad a = \mu,\sigma.
\enq
are the fraction of the information that can be accessed by extraction of the full set of moments of $X$. The two asymptotic regimes of very small and very large fluctuation variance $\sigma_\delta$ can be seen without difficulty. In both cases, it is seen that the first non vanishing term of the corresponding series dominates completely its value. For very small variance, or equivalently $q$ very close to unity, $\epsilon_a$ tends to unity, illustrating the fact the distribution becomes arbitrary close to Gaussian : all the information is contained in the first two moments. The large variance regime is more interesting, and, even tough the information coefficients decays very sharply as well, the series (\ref{fmoments}) are far from converging to the corresponding expressions (\ref{Fmuex}) and (\ref{Fsigex}) showing the total amount of information. Considering only the dominant first term in the relevant series and setting $q \rightarrow 0$, one obtains 
\begin{equation} \label{asymptotics}
\epsilon_\mu \rightarrow \frac{1}{\sigma_\delta^2} \ln  \lp 1 + \sigma_\delta^2\rp .
\end{equation}
and a much more dramatic decay of $\epsilon_\sigma$ :
\begin{equation} \label{asymptotics2}
\epsilon_\sigma \rightarrow \frac{4}{\sigma_\delta^8} \ln \lp 1 + \sigma_\delta^2\rp.
\end{equation}
%-------------------------------------------------------------
%-------------------------------------------------------------
 Both series given in (\ref{fmoments}) are quickly convergent and well suited for numerical evaluation. Figure \ref{fig1} shows the accessible fractions $\epsilon_a$ of information through extraction of the full series moments. Figure \ref{fig2} shows the repartition of this accessible fraction among the first 10 moments. Most relevant from a cosmological point of view in figure \ref{fig1} is the solid line, dealing with the case of the  parameters of interest entering the variance only. These figures shows clearly that the moments, as probes of the lognormal matter field, are penalized by two different processes. First, as soon as the field shows non-linear features, following equations (\ref{asymptotics}) and (\ref{asymptotics2}), almost the entirety of the information content cannot be accessed anymore by extracting its successive moments. Within a range of one magnitude in the variance, the moments goes from very efficient probes to highly inefficient. Second, as shown in figure \ref{fig2}, as  the variance of the field approaches unity, this accessible fraction gets quickly transferred from the variance alone to higher order moments. This repartition of the information within the moments is built out of two different regimes. First, for large variance, or  large $n$, we see easily from the above expressions (\ref{anbn}) and (\ref{Ansigma}) that in both cases the information coefficients decays exponentially,
\begin{equation} \label{as1}
s_n^2 \propto \lp 1 + \sigma_\delta^2 \rp^{-n},\quad n\ln \lp 1 + \sigma^2_\delta \rp  \gg   1.
\end{equation}
On the other hand, if the variance or $n$ is small enough, we can set $1 - q^n \approx -n\ln q $, and we obtain, very roughly,
\beq\label{as2}
s_n^2 \propto \lb n \ln \lp 1 + \sigma_\delta^2 \rp\rb^{n},\quad n\ln \lp 1 + \sigma^2_\delta \rp   \ll 1,
\enq
explaining the trend with variance seen in figure \ref{fig2}, that puts more importance to higher order moments as the variance grows.
Note that the latter regime can occur only for small enough values of the variance. Deeper in the non linear regime, the trend is therefore reversed, obeying (\ref{as1}) for all values of $n$, with a steeper decay for higher variance.

 \begin{figure}
  \includegraphics[width = \textwidth]{figs/fig1}
 \caption{\label{fig1} The fraction of the total information content that is accessible through extraction of the full series of moments of the lognormal field, as function of the square root of the variance of the fluctuations.}
 \end{figure}

 \begin{figure}
  \includegraphics[width = \textwidth]{figs/fig2}
 \caption{\label{fig2} The distribution of the information within the first 10 moments of the lognormal field, given by the coefficients $\lp s^\sigma_n \rp^2$, equation (\ref{Ansigma}), normalized to the information content of the second moment, for three different values of $\sigma_\delta$. Note that deeper in the non linear regime, the trend is reversed.}
 \end{figure}
 
 \subsection{A $q$-analog of the logarithm}
 \begin{figure}
  \includegraphics[width = \textwidth]{figs/fig3}
 \caption{\label{fig3}The information density of the lognormal distribution, dashed, and, solid, its approximation through the associated orthonormal polynomials, in the $a = \sigma$ case, for fluctuations of unit variance. While most of the information of the lognormal field in this regime is actually contained in the underdense regions, the moments are essentially unable to catch it.}
 \end{figure}
 % \begin{figure}
  %\includegraphics[width = \textwidth]{Infdensitymu}
 %\caption{\label{fig3}The information density  $p(x,\alpha)\:s^2(x,\alpha)$ for the lognormal distribution, dotted, and, solid, its approximation through the associated orthonormal polynomials, in the $a = \sigma$ case. Each logarithmic interval on this plot contributes equally to the total amount of information. While most of the information is actually contained in the underdense regions, the moments are essentially unable to catch it.}
% \end{figure}
These results show clearly that large parts of the information become invisible to the moments. However, it does not tell us what is responsible for this phenomenon. It is therefore of interest to look in a little bit more into the details of this missing pieces of information. As we have seen, these are due to the inability of the polynomials to reconstruct precisely the score function. 
In the case $a = \mu$, the score function of the lognormal distribution is easily shown to take the form of a logarithm in base $q$,
\beq
\begin{split}
s(x)% &=  \frac{\partial  \ln p(x,\alpha)}{\partial \alpha} = \\
%&= \frac{\partial \ln \mu}{\partial \alpha} \lp \frac {\ln \lp x/\mu\rp }{\ln q} + \frac 12 \rp \\
& = -\frac 12 -  \ln_q \lp \frac  {x} {\mu}\rp .
\end{split}
\enq
Therefore the series
\beq
s^\mu(x) := \sum_{n = 0}^\infty s_n^\mu P_n(x)
\enq
will represent some function, very close to a logarithm for $q \rightarrow 1$ over the range of $p(x,\alpha)$. It will however fail to reproduce some of its features at lower $q$-values. This is hardly surprising, since it is well known that the logarithm function does not have a Taylor expansion over the full positive axis. For this reason, the approximation $s^\mu(x)$ of $s(x)$ through polynomials can indeed only fail when the fluctuation variance becomes large enough. In the appendix, we show that $s^\mu(x)$ takes the form
\beq \label{smu}
s^\mu(x) = - \sum_{k = 1}^\infty \frac{q^k}{1-q^k}\lb 1 +(-1)^k\frac{q^{k(k-1)}}{\pochh  q q k} \lp \frac{x}{\mu}\rp^k\rb.
\enq
 It is interesting to note that this series expansion is almost identical to the one of the $q$-analog of the logarithm $S_q(x)$  defined by E. Koelink and W. Van Assche, with the only difference being the replacement of $q^{k(k-1)/2} $ by $q^{k(k-1)}$ (See \citep{Koelink09}, and also \citep{Gautschi06}). Due to this replacement, $s^\mu$ does not possess several properties $S_q$ has and makes it a real $q$-analog of the logarithm, such as $S_q(q^{-n}) =  n$, for positive integers. The qualitative behavior of $s^\mu$ stays however close to $S_q$. Notably, its behavior in underdense regions, $x/ \mu \ll 1$,  where as seen from (\ref{smu}) $s^\mu$ tends to a finite value, is very different from a logarithm.
 \newline\newline
This calculation can be performed as well in the case $a = \sigma$, with similar conclusions. Since it is rather tedious and not very enlightening, we do not reproduce it in these pages. We show in figure \ref{fig3} the information density, equation (\ref{infdensity}), of the lognormal distribution (dashed line), 
 and its approximation by the orthogonal polynomials (solid line),
 \beq
 p(x,\alpha)\lp \sum_{n = 0}^\infty s_n^\sigma P_n(x)\rp^2,
 \enq
 when the fluctuation variance $\sigma^2_\delta$ is equal to unity. It is clear from this figure that in this regime, while most of information is located within the underdense regions of the lognormal field, the moments are however unable to catch it. \newline
 To check the correctness of our numerical and analytical calculations, we compared the total information content as evaluated from integrating the information densities on figure \ref{fig3} to the one given by the equation (\ref{Fsigex}), respectively (\ref{fmoments}), with essentially perfect agreement.
 %------------------------------------------------------------------
\subsection{Comparison to standard perturbation theory}
For any distribution, the knowledge of its first $2n$ moments allow directly, for instance from equation (\ref{infn}), the evaluation of the independent information content of the first $n$ moments. This even if the exact shape of the distribution is not known, or too complicated. In particular, we can use the explicit expressions for the first six moments of the density fluctuation field within the framework of standard perturbation theory (SPT) provided by F. Bernardeau in \citep{1994A&A...291..697B}, in order to compare $s_2$ and $s_3$ as given from SPT to their lognormal analogs.\newline\newline
We note that a comparison to \citep{1994A&A...291..697B} can only be very incomplete and, to some extent, it can only fail. It is indeed part of the  approach in \citep{1994A&A...291..697B}, when producing functional forms for the distribution of the fluctuation field, to invert the relation between a moment generating function and its probability density function. For such an inversion to be possible it is of course necessary that the probability density is uniquely determined by its moments. As said, this is not the case for the lognormal distribution. Therefore, that approach can never lead to an exact lognormal distribution, or to any distribution for which the moment hierarchy forms an incomplete set of probes. However, such a comparison can still lead to conclusions relevant for many practical purposes, such as those dealing with the first few moments.
\newline\newline
The variance of the field is explicitly given as an integral over the matter power spectrum,
\beq \label{varbdeau}
\sigma^2_\delta  = \frac{1}{2\pi^2}\int_0^\infty dk \:k^2P(k,\alpha) \left|W(kR)\right|^2,
\enq
where $W(kR)$ is the Fourier transform of the real space top hat filter of size $R$, and any cosmological parameter $\alpha$ entering the power spectrum $P(k)$.
In the notation of \citep{1994A&A...291..697B}, the moments of the fluctuation field $m_n = \av{\delta^n}$ are given by the deconnected, or Gaussian, components, while the connected components $\av{\delta^n}_c ,\quad n \ge 3$ are given in terms of parameters $S_n$,
\beq \label{mbdeau} \begin{split}
\av{\delta^n}_c = \sigma^{2(n-1)}S_n.
\end{split}
\enq
The parameters $S_n$ contain a leading, scale independent coefficient, and deviation from this scale independence are given in terms of the logarithmic derivative of the variance,
\beq
\gamma_i = \frac{d^i \ln \sigma^2_\delta}{d\:\ln R^i},\quad i = 1,\cdots
\enq
Neglecting the very weak dependence of $S_n$ on cosmology, from (\ref{mbdeau}) we can write
\beq
\begin{split}
 \frac{\partial m_n}{\partial \alpha} = \frac{\partial \sigma_\delta^2}{\partial \alpha}\cdot \begin{cases} 0,&\quad n = 1 \\  1,&\quad n = 2
 \\ 2 m_3 \:/ \: \sigma_\delta^2,&\quad n = 3  \end{cases}
\end{split}
\enq
With the coefficients $S_n$ up to $n = 6$ given in  \citep[page 703]{1994A&A...291..697B}, and the above relations, we performed a straightforward evaluation of the information coefficients $s_2^2$ and $s_3^2$, using equation (\ref{infn}). The variance was obtained from (\ref{varbdeau}) within a flat $\Lambda$CDM universe ($\Omega_\Lambda = 0.7,\Omega_m = 0.3,\Omega_b = 0.045, h = 0.7$),  with power spectrum parameters ($\sigma_8 = 0.8, n = 1$) and we used the transfer function from Eisenstein and Hu \citep{1998ApJ...496..605E}. The needed derivatives $\gamma_i, \: i = 1,\cdots, 4$ were obtained numerically through finite differences.
\newline\newline
In figure \ref{fig4}, we show the ratio
\beq
\lp \frac{s^\sigma_3}{s^\sigma_2} \rp^2
\enq
i.e. the relative importance of the third moment with respect to the second, as function of the variance, both for the lognormal distribution and the SPT predictions. This ratio is identically zero for a Gaussian distribution.
The models stands in good agreement over many orders of magnitude. It is striking that both models consistently predict that a the entrance of the non-linear regime,  this ratio takes a maximal value close to unity. Surely, the SPT curve for larger values of the variance is hard to interpret, since out of its domain of validity. 
  \begin{figure}
  \includegraphics[width = \textwidth]{figs/fig4}
 \caption{\label{fig4}The ratio of the independent information content of the third moment to that of the second moment, for the lognormal field (dashed) and standard perturbation theory (solid), as function of the square root of the variance of the fluctuations. }
 \end{figure}
 %---------------------------
\section{Several variables}
\newcommand{\vecn}{\mathbf n}
\newcommand{\vecm}{\mathbf m}
\newcommand{\veci}{\mathbf i}
\newcommand{\vecj}{\mathbf j}
So far, we have considered only one variable, and wish now to extend our analysis to the more interesting multidimensional case. It is possible to derive formally a general expression for the independent information content of the $n$-point correlations of any distribution. This proceeds in strict analogy with the one-dimensional case, where an expansion of the score function in polynomials of several variables is made. It is presented in some more details in the appendix. For the lognormal field, a given model parameter can only enter via the means of the logarithm of the field at each point or through the elements of its two-point correlation matrix.  We could however not transform the corresponding expressions in a useful, easily evaluated form in a general situation, like in the one dimensional case.  We focus therefore on two more restricted but tractable situations. First, in analogy with the $a = \mu$ case, we consider a parameter that enters the mean of the field $\rho $ and no elements of the correlation matrix. In this case, the complete amount of information can be extracted via the mean of $\ln \rho$, and compare that amount to the one obtained by extracting the mean of $\rho$ only. In a second step, we consider the extraction of the correlation amplitude $\xi(r)$ between independent pairs of cells separated by that distance $r$. In this case, the full amount of information on any parameter impacting $\xi(r)$ is in the correlation of $\ln \rho$, and compare that to the more standard approach of the extraction of the correlation of $\rho$.
%-----------------------------------------------
\subsection{Basic properties of the multivariate lognormal distribution}
%-----------------------------------------------
The random vector $\rho = \lp \rho_1,\cdots,\rho_d \rp$ has a multivariate lognormal distribution if $\ln\rho := \lp \ln \rho_1,\cdots, \ln \rho_d \rp$ is normally distributed, for some
 mean vector $\bar \ln\rho$ and covariance matrix $\xi_{\ln \rho}$. 
 Since we have in mind the vector $\rho$ to be a sample of an homogeneous lognormal field, we will use the notation
 \beq
 \rho_i = \rho(x_i),\quad i = 1,\cdots,d,
 \enq
 the points $x_i$ lying in some $n-$dimensional space. The means $\mlnrho_i$ are the same at each point, and the covariance matrix is  a discrete version of the corresponding correlation function,
 \beq
 \lb \xi_{\ln \rho} \rb_{ij} = \xi_{\ln\rho}(x_i - x_j),\quad i,j = 1,\cdots,d
 \enq
 which depends only on the separation vector.
 For some vector of natural numbers  (multiindex) $\vecj = (j_1,\cdots,j_d)$, the correlations
 \beq
 m_\vecj = \av{\rho^\vecj }=  \av{\rho(x_1)^{j_1}\cdots\rho(x_d)^{j_d}}
 \enq
 are again given by simple Gaussian integrals and read explicitly
 \beq \label{moments2}
 m_\vecj = \exp\lp \mlnrho \cdot \vecj + \frac 12 \:\vecj^T \xi_{\ln \rho} \cdot \vecj \rp.
 \enq
 By the independent information content $s_n^2$ of the n-point correlations we mean the independent bits of information within all the correlations of the same order $n$, that is within all $m_\vecj$ such that
 \beq
 |\vecj| := \sum_{i = 1}^d j_i = n.
 \enq
The convenient property (\ref{separability}) between the moments becomes
 \beq \label{separability2}
 m_{\veci + \vecj} = m_\veci \:m_\vecj \exp \lp \veci ^T \xi_{\ln \rho} \cdot \vecj \rp :=  m_\veci \:m_\vecj \:Q_{\veci\vecj}.
 \enq
 From these relations, one infers that the correlations of the fluctuations $\xi$ of $\rho$, defined as
 \beq \label{xidef}
  \xi(x_i-x_j) = \frac{1}{\mrho^2}\av{ \lp \rho(x_i) - \mrho \rp\lp \rho(x_j) - \mrho \rp}, 
 \enq
  are related to those of $\ln\rho$ through
 \beq \label{corrrel}
 \begin{split}
 \xi_{\ln \rho}\lp r \rp & = \ln\lb 1 + \xi \lp r \rp \rb.
 \end{split}
 \enq
 On the other hand. the means obey
 \beq
 \begin{split}
  \mlnrho &= \ln \mrho-\frac 12  \xi_{\ln \rho}(0) \\ 
  &=  \ln \mrho-\frac 12  \ln \lp 1 + \sigma^2_\delta \rp.
  \end{split}
 \enq
 The Fisher information content of $\rho$ is again given by the standard expression for the Gaussian field $\ln\rho$. It splits into the part coming from the observation of $\mlnrho$ and the one coming from the correlations $\xi_{\ln\rho}$,
 \beq\label{infmulti}
 F_\alpha = \frac 12 \Tr \lb \xi_{\ln \rho}^{-1} \frac{\partial \xi_{\ln \rho}}{\partial \alpha}\:\xi_{\ln \rho}^{-1} \frac{\partial \xi_{\ln \rho}}{\partial \alpha} \rb + \frac{\partial \mlnrho}{\partial \alpha}\xi_{\ln\rho}^{-1} \cdot \frac{\partial \mlnrho}{\partial \alpha}.
 \enq
 We denote by $Q_N$ the square matrix defined as
\beq
\lb Q_N  \rb_{\veci\vecj} = Q_{\veci\vecj},\quad |\veci|,|\vecj| \le N,
\enq
which we will make future use of. We note that by virtue of equations (\ref{separability2}) and (\ref{corrrel}), its matrix elements read
\beq \label{qm}
Q_{\veci\vecj} = \prod_{k,l = 1}^d\lp 1 + \xi \lp x_k - x_l\rp \rp^{i_kj_l}.
\enq
%-----------------------------------------------
%\subsection{Independent information in the $n$-point correlations}
%-----------------------------------------------
A general expression for the independent information content $s_n^2$ of the correlations of order n, equation (\ref{smulti}), and its link to the completeness of the orthogonal polynomials is presented for completeness in the appendix. This machinery is however not compulsory for the following considerations, which are restricted to the two lowest order correlations. We will only use the analog of equation (\ref{infn}), which gives the total amount of information contained in the correlations up to order $N$,
\beq\label{infm}
\sum_{n = 1}^N s_n^2 = \sum_{|\veci|,|\vecj| = 1}^N \frac{\partial m_\veci}{\partial \alpha}\lb \Sigma^{-1} \rb_{\veci\vecj}\frac{\partial m_\vecj}{\partial \alpha},
\enq
where $\Sigma$ is the covariance matrix
\beq
\Sigma_{\veci\vecj} = m_{\veci + \vecj} - m_\veci m_\vecj,\quad|\veci|,|\vecj| \le N.
\enq
For the lognormal distribution, the property (\ref{separability2}) allow us to rewrite this last expression in the equivalent form
\beq \label{infsum}
\sum_{n = 1}^N s_n^2 = \sum_{|\veci|,|\vecj| = 0}^N \frac{\partial \ln m_\veci}{\partial \alpha}\lb  Q_N^{-1} \rb_{\veci\vecj}\frac{\partial \ln m_\vecj}{\partial \alpha}.
\enq
%-----------------------------------------------
\subsection{Extraction of the mean}
%-----------------------------------------------
In this case, we set
\beq \label{cond}
\frac{\partial \xi(r)}{\partial \alpha } = 0
\enq
for any argument. Again, the actual value of the derivative of the mean with respect to $\alpha$ will play no role.
This condition (\ref{cond}) implies that $\partial_\alpha \xi_{\ln \rho} $ vanishes as well. We can read out from equation (\ref{infmulti}) that the total amount of information is given by
\beq
\begin{split}
F_\alpha &= \lp \frac{\partial \ln \mrho}{\partial \alpha}\rp^2 \sum_{i,j = 1}^d \lb \xi_{\ln\rho}^{-1}\rb_{ij} \\
\end{split}
\enq
We stress that since $\ln\rho$ is Gaussian, the information is accessible in its entirety by extraction of the mean of $\ln \rho$. On the other hand, the amount extracted by looking at the mean of $\rho$ itself is equation (\ref{infm}) with $N = 1$.  Using the definition of $\xi$ in equation (\ref{xidef}), it becomes
\beq
s_1^2 =  \lp \frac{\partial \ln \mrho}{\partial \alpha}\rp^2 \sum_{i,j = 1}^d \lb \xi^{-1} \rb_{ij}.
\enq
In the limit of a continuous sample  $d \rightarrow \infty$, the sum
\beq
\sum_{i,j = 1}^d \lb \xi^{-1} \rb_{ij}
\enq
becomes a double integral over space, which can be performed by Fourier transformation, and is the inverse of the power spectrum of the field at zero argument,
\beq \begin{split}
\sum_{i,j = 1}^d \lb \xi^{-1} \rb_{ij} & \stackrel{N\rightarrow \infty}{\rightarrow} \frac{ V}{ P_\rho( k = 0)} \\
P_\rho(0) &= \int_V d^nr \:\xi(r) 
\end{split}
\enq
and similarly for $\xi_{\ln\rho}$. We conclude that the loss of information by looking at the mean of the field only is given straightforwardly by the ratio of the power of the fields $\ln \rho$ and $\rho$ at zero argument.
\beq
\epsilon := \frac{s_1^2}{F_\alpha} =\frac{P_{\ln \rho}(0)}{P_\rho(0)}.
\enq
From the explicit representation of $P_{\ln\rho}(0)$, 
\beq
P_{\ln \rho}(0) = \int_V d^nr \ln \lp 1 + \xi(r)\rp
\enq
and the fact that $\ln \lp 1 + x \rp$ is strictly smaller than $x$ whenever $x \ne 0$, it follows that the loss of information always occurs, but is substantial only if the correlation function takes substantial values. However the information loss $\epsilon$ is roughly insensitive to the presence of some correlation scale. We see that the presence of correlations does not alter the main conclusions drawn in the first part of his work. \newline
%Since the power spectrum of a field is always positive, this also puts a non-trivial constraint on the correlation function $\xi$ to possibly originate from a lognormal field. The following inequalities must indeed hold,
%\beq
%0 \le \int_V d^nr \ln \lp 1 + \xi(r)\rp \le \int_V d^nr\: \xi(r).
%\enq
%As we discussed, the second is always true, but the first may not. For this reason, fields with very low power at zero, for which the rightmost term vanishes, hardly qualify as lognormal fields.
\subsection{Extraction of correlations}
We suppose now the parameter $\alpha$ enters the correlation function $\xi$ for some argument $r$.
Since the field is lognormal, measurement of $\xi_{\ln\rho}(r)$ captures all the information on $\alpha$. We want to compare this amount to the one extracted by measuring $\xi(r)$ itself. We suppose further that $\xi(r)$ is extracted from a number of independent pairs of points separated by that distance $r$. The independency of the pairs allow us to simplify drastically the problem, since by additivity of the information the information loss will be  independent of the number of pairs. Our problem becomes thus two-dimensional. Our assumptions on the impact of the parameter $\alpha$ are, more explicitly, 
\beq \label{ass2}
\frac{\partial \mrho}{\partial \alpha }= 0,\quad \frac{\partial \sigma^2_\delta}{\partial \alpha} = 0,\quad \frac{\partial \xi(r)}{\partial \alpha} \ne 0.
\enq
We point out that this is very different from the $a = \sigma$ case that we treated earlier, since here the variance $\sigma^2_\delta$ only acts as a noise source and not as a source of information.
The correlation matrix of a pair of points of the homogeneous Gaussian field $\ln \rho$ separated by $r$ reads, according to (\ref{corrrel}),
\beq
\xi_{\ln \rho} = \begin{pmatrix} \ln \lp 1 + \sigma^2_\delta \rp & \ln  \lp 1 +\xi(r) \rp  \\ \ln \lp 1 +\xi(r) \rp & \ln  \lp 1 + \sigma^2_\delta \rp & \end{pmatrix}.
\enq
The positivity of the matrix constrains, at a fixed variance $\sigma^2_\delta$, the values of $\xi(r)$ to the following range
\beq
1 + \xi(r) = \lp 1 + \sigma^2_\delta\rp^\eta,\quad \eta \in (-1,1).
\enq
Clearly, vanishing correlations corresponds to $\eta = 0$, positive correlations to $\eta > 0$, and negative correlations to $\eta < 0$. 
By assumption, the parameter $\alpha$ does enter $\xi(r)$ only. Therefore,
\beq \label{above}
\frac{\partial \xi_{\ln \rho}}{\partial \alpha} = \frac{\partial_\alpha \xi (r)}{1 + \xi(r)} \begin{pmatrix} 0 & 1 \\ 1 & 0 \end{pmatrix}.
\enq
Putting (\ref{above}) in equation (\ref{infmulti}), we obtain that the total amount of information on $\alpha$ is
\beq\label{f2ptln}
F_\alpha = \lp \frac{\partial_\alpha \xi (r)}{1 + \xi(r)}\rp^2\frac{1 + \eta^2}{\lp 1 - \eta^2 \rp^2}\frac{1}{\ln^2\lp 1 + \sigma^2_\delta \rp}.
\enq
To obtain the information obtained by extracting $\xi$, we first note that under our assumption (\ref{ass2}) the mean carries no information,
\beq
s_1 = 0.
\enq
For this reason, $s_2^2$ is given by equation (\ref{infsum}), with $N = 2$. The only non-zero element of the vector of derivatives $\partial_\alpha \ln m_\veci,\:|\veci| \le 2$, is in our configuration (\ref{ass2}) for the multiindex  $\veci = (1,1)$. From  equations (\ref{moments2}) and (\ref{corrrel}), we obtain
\beq
\frac{\partial \ln m_{(1,1)}}{\partial \alpha } = \frac{\partial \xi(r)}{\partial \alpha}\frac 1 {1 + \xi(r)}.
\enq
It follows immediately that $s_2^2$ is given by
\beq\label{f2pt}
s_2^2 = \lp \frac{\partial_\alpha \xi (r)}{1 + \xi(r)}\rp^2\lb Q_2^{-1} \rb_{(1,1)(1,1)}.
\enq
 Of special interest is the limit of low correlations, where the exact result 
\beq \label{xi0}
\frac{s_2^2}{F_\alpha} = \frac1  {\sigma^4_\delta} \ln^2\lp 1 + \sigma^2_\delta\rp, \quad \textrm{for}\quad \xi(r) = 0.
\enq
can be obtained making profit of the simple structure of the $Q_2$ matrix.
We note that $Q_2$ is in our two-point configuration a 6 dimensional matrix, where, as seen from its representation (\ref{qm}), all of its elements are products and powers of $1 + \sigma_\delta^2$ and $1 + \xi(r)$.
The needed inverse matrix element can be written as ratio of determinants
\beq \label{poly}
\lb Q_2^{-1} \rb_{(1,1)(1,1)} = \frac{\det \hat Q_2}{\det Q_2}, 
\enq
where $\hat Q_2$ is the 5-dimensional matrix originating from $Q_2$ where the row and column corresponding to the multiindex $(1,1)$ have been taken out. Both of these determinants are therefore clearly polynomials in $1 + \sigma_\delta^2$ and $1 + \xi(r)$. The asymptotic behavior of the accessible information for large variance can be thus obtained by noticing that $\eta \rightarrow 0$ for any value of $\xi$. Looking then at the  leading coefficients of the two polynomials entering (\ref{poly}), we obtain
\beq 
\begin{split}
\det Q_2 & \rightarrow \lp \sigma^2_\delta \rp^{12}\lp 1 + \xi(r) \rp^2\\
\det \hat Q_2 & \rightarrow \lp \sigma^2_\delta \rp^{10}.
\end{split}
\enq
Therefore, the information loss
\beq \label{infoxiloss}
\epsilon := \frac{s_2^2}{F_\alpha}
\enq
tends to, for asymptotic values of the variance,
\beq\begin{split}
\epsilon &\rightarrow \frac 1 {\sigma^4_\delta}  \frac{\ln^2\lp 1 + \sigma^2_\delta  \rp} {\lp1 + \xi(r) \rp^2} \\
&= \frac{\epsilon (\xi = 0)} {\lp1 + \xi(r) \rp^2}.
\end{split}
\enq
The second line follows from the first using the exact result for vanishing correlations given in equation (\ref{xi0}).
The efficiency of $\xi$ in extracting the information on any parameter therefore always goes to zero, following approximately the inverse squared variance. The presence of substantial positive correlations, generic for a field generated by gravitational instability on a wide range of scales, only makes the information loss worse.
This is illustrated in figure \ref{figxi}, where the dotted line shows the loss of information at the non linearity scale $\xi(r) = 1$, evaluated numerically from equations (\ref{f2ptln}) and (\ref{f2pt}), together with the exact result (\ref{xi0})  for vanishing correlations (solid line).
%------------------------
\begin{figure}
  \includegraphics[width = \textwidth]{figs/fig5}
 \caption{\label{figxi} The loss of information $\epsilon$ in extracting correlations of $\rho$ instead of $\ln \rho$ for a lognormal field, equation (\ref{infoxiloss}), in the limit of vanishing correlations (solid line), and at the non linearity scale $\xi(r) = 1$ (dashed) as function of the square root of the variance of the fluctuations.}
 \end{figure}
 %------------------------

\section{Summary and conclusion}
We have investigated in details the structure of the information within the moments of the univariate lognormal distribution, as a model for the matter density field. We have provided exact expressions, equations (\ref{anbn}) and (\ref{Ansigma}) for the independent information content of each moment. Using these expressions, we have shown that the moments become dramatically incomplete probes in the non linear regime.  In the cosmologically relevant case of the parameter entering the power spectrum of the fluctuations, the fraction of the information that is accessible from the moments is close to one fourth at $\sigma_\delta = 1$, and decays following the inverse $4$th power of the variance. We showed it is mainly due to the inability of the moments to probe the information located in the underdense regions of the distribution. Besides, a comparison to standard perturbation theory showed for the lower order moments showed that both approaches are consistent and predict that the third order moment becomes as important as the variance itself when entering the non linear regime.\newline\newline In a second step, we extended our results to the multivariate case, showing that the mean of the field and two-point correlations become in a very similar manner very inefficient probes, for any parameter of interest. With the help of two simplified situations we have shown that the presence of correlations only makes the information loss even worse. More specifically, we have shown that  the extraction of the two-point correlation function at any argument provides access to a fraction of the information which is generically well below unity at the entrance of the non linear regime, and decays like the inverse squared variance. 
\newline\newline
These results, making clear that the information content of the lognormal field not only gets transferred to higher order point functions, but also becomes largely inaccessible to the correlation function hierarchy in the non linear regime, confirm to full extent qualitative suspicions raised in \citep[section 4]{1991MNRAS.248....1C}, to which we refer for a more complete discussion on physical arguments that may source such a behavior. \newline\newline
We can understand for any random field if the hierarchy members are promising probes or not from the following considerations. Let $p[\phi,\alpha]$ be the probability density function for a realization $\phi$ of the field. As we have seen, the information content of the first $N$-correlation functions is based on the approximation of the score function $\partial_\alpha \ln p[\phi] $ through polynomials up to order $N$, over the range of $p[\phi]$. Let us assume for instance that for any value of the model parameter  $\ln p[\phi]$ can be expanded in a low order Taylor series in the field,
\beq \label{expfield}\begin{split}
\ln p[\phi,\alpha] &= \sum_{n = 0}^N \int dx_1\cdots dx_n \\
&\lambda_n \lp x_1,\cdots,x_n,\alpha \rp \phi(x_1)\cdots\phi(x_n). 
\end{split}
\enq
This class of distributions, including Gaussian fields for which $N = 2$, can arise notably as maximal entropy distributions for fixed values of the first $N$-correlation functions. The coefficient $\lambda_n$ is called in this framework the potential associated to the $n$-th correlation function (See \citep[e.g.]{jaynes83,caticha08}). Since $\partial_\alpha \ln p$ is itself of polynomial of order $N$, all the information is contained is the first $N$-correlation functions. Of course, the relative importance of each one of these will be modulated by the sensitivity of the potentials to the parameter $\alpha$ and their covariances. This situation is certainly the one where the correlation function hierarchy are the probes of choice, since only a finite number of these grasp the entire information content. \newline\newline
Two different processes may at this point render the hierarchy inefficient, or incomplete. First of all, if a large number of terms are needed in the expansion (\ref{expfield}) to reproduce accurately the score function $\partial_\alpha \ln p$. In this case, one would need to go deep down the hierarchy in order to catch the information. This is certainly not desirable. The last case occurs when $\partial_\alpha \ln p$ has no Taylor expansion at all over the relevant range. It is then simply not possible to represent accurately the score function. Parts of the information (given in the field analog of equation (\ref{MSE})) becomes invisible to the correlation function hierarchy. The lack of a Taylor expansion for the logarithm function is the reason for the failure of the moments and correlation functions to catch the information of a lognormal field in the non linear regime, when the range of the probability density function becomes very large. \newline\newline
We emphasize, as in \citep{1991MNRAS.248....1C}, that these peculiar dynamics of the information are not due to a pathological character of the lognormal distribution. It should be expected for any distribution decaying slowly at infinity. We can add to their discussion that this is so because  $\ln p$ cannot be well reproduced by polynomials under this condition.
\newline\newline
Given the very high amplitude of these effects within the lognormal assumption, we believe that in order to get the best out of future galaxy survey data, it is crucial to understand better these issues. The present work presents first steps to this aim. It is also very consistent and brings strong support to the recent studies started in \citep{2009ApJ...698L..90N,2011ApJ...731..116N,2011arXiv1103.2166W} making in the non linear regime the logarithm of the field rather than the field itself the central quantity of interest. It remains however to be seen to what extent the approach presented in this work is able to provide quantitative predicitions for the statistical power of higher point functions, or for power spectrum extraction. We leave these aspects for future work.

\section{Derivation of relation (\ref{lemma}) \label{proof}}
To prove (\ref{lemma}),  we note that both sides of the equation are polynomials of degree $n$ in $t$, and that the zeroes of the right hand side are given by
\beq
t = q^{-i}, \quad i = 0,\cdots, n-1.
\enq 
We first show that the left hand side evaluated at these points does vanish as well, so that the two polynomials must be proportional. We then find the constant of proportionality by requiring $P_n$ to have the correct normalization. \newline
The first step is performed by noting that
\beq
\av{P_n(q^{-i}x)} = \frac 1 {m_i}\av{P_n(x)x^i }, \quad i = 0,1,\cdots
\enq
an identity which is proven by expanding $P_n $ in both sides of the equation  in terms of the transition matrix $C$, and using the relation (\ref{separability}) between the moments.
Since $P_n$ is by construction orthogonal to any polynomial of strictly lower degree, we have indeed
\beq
\av{P_n(q^{-i}x)} = 0,\quad i = 0,\cdots,n-1. 
\enq
This implies
\beq \label{sumrule}
\sum_{k = 0}^n C_{nk} m_k\:t^k  =\alpha_n \pochh t q n
\enq
for some constant of proportionality $\alpha_n$. To find it, 
%we use the expansion of the $q$-Pochammer symbol in powers of $t$
% which is given by the Cauchy binomial theorem,
%\beq \label{Cauchyb}
%\pochh t q n = \sum_{k = 0}^n  q^{k(k-1)/2}\binq nk q(-t)^k,
%\enq
%where
%\beq
%\binq n k q = \frac{\pochh q q n}{\pochh q q k \pochh q q {n-k}}
%\enq is the Gaussian binomial coefficient. Matching powers of $t$,
%we obtain
%\beq \label{}
%C_{nk}m_k = \alpha_nq^{k(k-1)/2} \binq n k q (-1)^k,
%\enq
%where $\alpha_n$ is the constant of proportionality. We need to show
%\beq
%\alpha_n = -\frac{q^{n/2} }{\sqrt {\pochh q q n}}.
%\enq
we note that by expanding the normalization condition of $P_n$,
\beq \begin{split}
1 &= \av{P_n^2(x)}, 
\end{split}
\enq
using again property (\ref{separability}), it must hold that
\beq
1 = \sum_{i,j = 0}^nC_{ni}m_j\: C_{nj}m_j\: q^{-ij}.
\enq
The sums can be performed using equation (\ref{sumrule}), leading to the following equation for $\alpha_n$,
\beq
1 = (-1)^n\:\alpha_n^2\: q^{n(n-1)/2}\pochh {q^{-n}}qn.
\enq
This expression simplifies to
\beq
\alpha_n^2 = \frac{q^n}{\pochh q q n}
\enq
and the sign of $\alpha_n$ must be $-1^n$ in order to have a positive matrix element $C_{nn}$. This concludes the proof of (\ref{lemma}).
%--------------------------------------------------------------------------
\section{Derivation of  the representation (\ref{smu})}
In order to get the explicit series representation of (\ref{smu}), we first obtain from relation (\ref{lemma}) the exact expression of the transition matrix $C$. The expansion of the $q$-Pochammer symbol on the right hand side of (\ref{lemma}) in powers of $t$ is the Cauchy binomial theorem,
\beq
\pochh t q n = \sum_{k = 0}^n \binq n k q q^{k(k-1)/2}(-t)^k,
\enq   
where
\beq
\binq n k q = \frac{\pochh q q n}{\pochh q q k \pochh q q {n-k}}
\enq is the Gaussian binomial coefficient. Matching powers of $t$ in (\ref{lemma}) we obtain the explicit form
\beq \label{}
C_{nk}=(-1)^{n-k} \frac{q^{n/2}}{\sqrt{\pochh q q n}} \binq n k q q^{k^2}\mu^{-k}.
\enq
Therefore, interchanging the $n$ and $k$ sums in (\ref{smu}) , it holds
\beq
s^\mu(x) =-\sum_{n = 1}^\infty \frac{q^n}{1- q^n} + \sum_{k = 1}^\infty q^{k^2} \lp -\frac x  {\mu}\rp^k \sum_{n = k}^\infty\frac{q^n}{1-q^n}\binq n k q.
\enq
With the help of some algebra the following identity is not difficult to show
\beq
\sum_{n = k}^\infty\frac{q^n}{1-q^n}\binq n k q = \frac 1 {\pochh q q k}\frac{q^k}{1 - q^k},\quad k \ge 1.
\enq
Consequently, the series expansion of $s_\mu(x)$ is given by
\beq
s^\mu(x) = - \sum_{k = 1}^\infty \frac{q^k}{1-q^k}\lb 1 +(-1)^k\frac{q^{k(k-1)}}{\pochh  q q k} \lp \frac{x}{\mu}\rp^k\rb
\enq
%----------------------------------------------------
\section{Several variables}
We first need a little bit of notation. For a variable $X$ taking values $x = \lp x_1,\cdots x_d\rp$, we use the multindex notation
\beq
\begin{split}
x^\vecn &= x_1^{n_1}\cdots x_d^{n_d} \\
\vecn &= \lp n_1,\cdots n_d\rp,\quad n_i = 0,1,\cdots. \\
|\vecn| &:= \sum_{i = 1}^dn_i,
\end{split}
\enq
where $|\vecn|$ is the order of the multiindex $\vecn$.
A moment of order $N$ is given by
\beq
m_\vecn = \av{x^\vecn}, \quad |\vecn| = N,
\enq
and the covariance between the moments is
\beq
m_{\vecn + \vecm} - m_\vecn m_\vecm =: \Sigma_{\vecn\vecm}.
\enq
In this notation, the decomposition of the information in independent bits of order $N$ proceeds by strict analogy with the one dimensional case. We refer to \citep{Dunkl01} for the general theory of orthogonal polynomials in several variables. A main difference being that at a fixed order $N$ there are not one but $\begin{pmatrix} N+ d -1\\  d \end{pmatrix}$ independent orthogonal polynomials, which are not uniquely defined. The orthogonality of the polynomials of same order is not essential for our purposes, but requiring the following condition is enough,
\beq \label{conditions}
\begin{split}
\av{P_\vecn(x) P_\vecm(x)} &= 0 ,\quad |\vecn| \ne |\vecm| \\
\av{P_\vecn(x) P_\vecm(x)} &= \lb H_n\rb_{\vecn\vecm} ,\quad |\vecn| = |\vecm| = n\\
\end{split}
\enq
for some matrices $H_n$.
The component of some function $f$ parallel to the polynomial $P_\vecn$ is
\beq
s_\vecn := \av{f(x)P_\vecn(x)}, 
\enq
and the expansion of $f$ in terms of these polynomials reads, in the notation of \cite[section 3.5]{Dunkl01}
\beq
S_N(f)(x) = \sum_{n = 0}^N\sum_{|\vecn|,|\vecm| = n}s_\vecn \lb H_n^{-1}\rb_{\vecn\vecm}P_\vecm(x).
\enq
It will converge to the actual function $f$ for $N \rightarrow \infty$ if the set of polynomials is complete, whereas it may not if not. The expansion is also independent of the freedom there is in the choice of the orthogonal polynomials in equations (\ref{conditions}).  Writing the orthogonal polynomials in terms of a triangular transition matrix
\beq
P_\vecn(x) = \sum_{|\vecm|\le |\vecn|}C_{\vecn \vecm}x^\vecm
\enq
and taking $f$ as the score function $s(x,\alpha)$, it is simple to see that the independent bits of information of order $n$ are given by
\beq
\begin{split} \label{smulti}
s_n^2 &= \sum_{|\vecn|,|\vecm| = n} s_\vecn \lb H^{-1}_n \rb_{\vecn\vecm}s_\vecm \\
&=    \sum_{|\veci|,|\vecj| \le n} \lb C^TH_n^{-1}C\rb_{\veci \vecj} \frac{\partial m_\veci}{\partial \alpha}\frac{\partial m_\vecj}{\partial \alpha},
\end{split}
\enq
and the strict analog of equation (\ref{infn}) holds for each $N$,
\beq
\sum_{n= 1}^N s_n^2 = \sum_{|\veci|,|\vecj| = 1 }^N \frac{\partial m_\veci}{\partial \alpha}\lb \Sigma^{-1} \rb_{\veci\vecj} \frac{\partial m_\vecj}{\partial \alpha}.
\enq

\section{Weak lensing convergence field}

N-point correlation functions, first introduced in cosmology by Peebles and collaborators to describe the large scale distribution of galaxies \cite{1980lssu.book.....P}, are now ubiquitous in this field. They are at the heart of many cosmological probes like the CMB, galaxy clustering, or notably weak lensing, which was recognized as one of the most promising probe of the dark components of the universe \cite{2001PhR...340..291B,2004PhRvD..70d3009H,2006astro.ph..9591A,2009ApJ...695..652B}, and which traces the cosmological convergence field.\newline
 On large scales, or in the linear regime, correlations are a particularly convenient approach to tackle the difficult problem of statistical inference on cosmological parameters. Indeed, primordial cosmological fluctuation fields are believed to obey Gaussian statistics, and the first two members of the hierarchy, the mean and the two-point correlation function, provide a complete description of such fields. However, much less is known about the pertinence of the correlation hierarchy in the non-linear regime, or on small scales, where in principle a lot of information is contained, if only due to the large number of modes available for the analysis. More elaborated statistical models  must be made in this regime. For instance, the statistics of the matter field and its weighted projection the convergence field were shown to be closer to lognormal, at least in low dimensional settings \cite{1991MNRAS.248....1C,2000MNRAS.314...92T,2002ApJ...571..638T,2006ApJ...645....1D}, though with sizeeable deviations still.\newline
 Two effects relevant for statistical inference can in principle play a role entering the non linear regime, departing from Gaussian initial conditions. First, information may propagate to higher order correlators. Second, the correlation function hierarchy may not provide a complete description of the field anymore %\cite{footnote2}
 , so that information escapes the hierarchy. Even though this second possibility was pointed out qualitatively in an astrophysical context already in \cite{1991MNRAS.248....1C}, it seems it was not given further attention in the literature.
\newline
In this \textit{Letter} we show, using accurate fits of the convergence one-point probability density function to numerical simulations \cite{2006ApJ...645....1D} that the second effect very quickly completely dominates the convergence field, and thus that the hierarchy is not well suited for inference on cosmological parameters anymore. 
\paragraph{Fisher information and orthogonal polynomials.}
The approach is based on decomposing the Fisher's matrix valued information measure in components unambiguously associated to the independent information content of the correlations of a given order. It was recently proposed in \cite{2011ApJ...738...86C}, building upon \cite{Jarrett84}. Exact results at all orders were obtained only for the moment hierarchy of a idealized, perfectly lognormal one dimensional variable, where analytical methods could be applied. In cosmology, the Fisher information matrix is widely used for many years now to estimate the accuracy with which cosmological parameters will be extracted from future experiments aimed at some observables \cite[e.g.]{Tegmark97a,2004PhRvD..70d3009H,2009ApJ...695..652B}, assuming Gaussian statistics.

For a general probability density function $p(x,\alpha,\beta)$, $\alpha$, $\beta, \cdots$ any model parameters, its definition is
\beq \label{FI}
F_{\alpha\beta} = \av{\frac{\partial \ln p}{\partial \alpha}\frac{\partial \ln p}{\partial \beta}}.
\enq
Its inverse can be seen through the Cram\'er-Rao bound \cite{Tegmark97a} to be the best covariance matrix of the relevant parameters achievable with the help of unbiased estimators.
The general procedure to decompose the Fisher information content into uncorrelated pieces, corresponding to an orthogonal system, was presented in a statistical journal in  \cite{Jarrett84}.  When the observables of interest are products of the variables, i.e. moments or more generally correlation functions, the orthogonal system are orthogonal polynomials. It is discussed in detail in an cosmological context in \cite{2011ApJ...738...86C}.
In particular, the variables for which the Fisher information content on $\alpha$ is entirely within the first $N$ pieces, such as the Gaussian variables for $N = 2$, are those for which the function $\partial_\alpha  \ln p$ entering
(\ref{FI}), called the score function, is a polynomial of order $N$ in $x$.
In the case of a single variable, %\cite{footnote4}
the uncorrelated contribution of order $N$ to the Fisher information matrix $\Fab$ is given by
 \beq
s_N(\alpha)s_N(\beta),
 \enq
 where the Fisher information coefficients $s_N$ are the components of the score function with respect to the orthonormal polynomial of order $N$,
 \beq \label{sndef}
 s_N(\alpha) = \av{\frac{\partial \ln p}{\partial \alpha}P_N(x)},
 \enq
 \beq
 \av{P_n(x)P_m(x)} = \delta_{mn},\quad n,m \ge 0
 \enq
 For any $N$, the following relation holds
 \beq \label{sumsn}
 \sum_{n = 1}^Ns_n(\alpha)s_n(\beta) = \sum_{i,j = 1}^{N}\frac{\partial m_i}{\partial \alpha } \lb \Sigma^{-1}\rb_{ij}\frac{\partial m_j}{\partial \beta },
 \enq
 where $m_i = \av{x^i}$ and $\Sigma_{ij} = m_{i+j} - m_im_j$ is the covariance matrix.
 The right hand side being the expression describing the Fisher information content of the moments $m_1$ to $m_N$. Whether one recovers the full matrix $\Fab$ with $N\rightarrow \infty$ or only parts of it depends on the distribution under consideration. A sufficient condition is that the polynomials $P_n$ form a complete basis set, which is then essentially equivalent to the condition that the distribution can uniquely be recovered from its moments hierarchy \cite[and references therein]{1991MNRAS.248....1C,2011ApJ...738...86C}. This and other sufficient criteria for completeness are tightly linked to the decay rate of the probability density function at infinity. 
 
 We define the cumulative efficiency $\epsilon_N$ of the moments up to order $N$ to capture Fisher information on $\alpha$ as
 \beq
 \label{eff}
 \epsilon_N(\alpha):= \frac{\sum_{n = 1}^Ns_n^2(\alpha)}{F_ {\alpha\alpha}}.
 \enq
 From the Cram\'er-Rao bound, $\sqrt{\epsilon_N}$ is the ratio of the the best constraints achievable on $\alpha$ with any unbiased estimator to the expected constraints on $\alpha$ from the extraction of the first $N$ moments .
 \paragraph{Fisher information coefficients}
 We use the fits to simulations from \cite{2006ApJ...645....1D}, valid down to the arcsecond scales.  Initially built to correct for the failure of the lognormal distribution to reproduce the high and low density tails of the convergence $\kappa$ on a single lens plane, it reproduces accurately the cosmological convergence as well, taking into account the broader lensing kernel \cite{2011ApJ...742...15T}. In terms of the reduced variable $x$,
  \beq
 x = 1 + \frac \kappa{ \left |\kappa_{\textrm{empty}} \right |} =: 1 + \delta_m^\eff,
 \enq
 where $\kappa_\textrm{empty}$ is the minimal value of the convergence, corresponding to a light ray traveling an empty region, it takes the form of a generalized lognormal model for the associated effective matter fluctuations $\delta_m^\eff$,
 \beq \label{model}
 p(x,\sigma) = \frac{Z}{x} \exp \lb -\frac{1}{2\omega^2} \lp \ln x + \frac{\omega^2}{2}   \rp^2\lp 1 +\frac{A}{x} \rp \rb.
 \enq
 In this equation, the three parameters $Z$, $A$ and $\omega$ are such that the mean of $x$ is unity, and its variance $\sigma^2 = \sigma^2_\kappa / \kappa^2_{\textrm{empty}}$ (we are neglecting here a small but non-zero mean of the convergence argued in \cite{2011ApJ...742...15T}). Therefore, the only relevant parameter is the variance of the associated matter fluctuations $\sigma^2$, fixed by the cosmology from $\kappa_{\textrm{empty}}$ and the convergence power spectrum, together with some filter function corresponding to the smoothing scale, determining the level of non linearity of the field \cite[figure 1 ]{2006ApJ...645....1D}. Linear and non-linear regime being separated at $\sigma^2 \approx 1$. We obtained %\cite{footnote1}
 $Z,A$ and $\omega^2$, shown in figure \ref{fig1}, 
 with the help of a standard implementation of the Newton-Raphson method for non-linear systems of equations.
 \begin{figure}
  \includegraphics[width = \textwidth]{figs/fig1PRL}
 \caption{\label{fig1}The three parameters $Z$,$A$ and $\omega^2$ entering the generalized lognormal model, as function of the variance of $\delta_m^\eff $.} 
 \end{figure}
 %With the probability density function at hand, there are several ways to obtain the Fisher information coefficients $s_N(\sigma^2)$. One is through the evaluation of the moments and their derivatives and the use of equation (\ref{sumsn}). This is however hardly to be recommended due to the very severe ill-conditioning of moment and covariance matrices, even for moderate value of $N$.
 \newline
Orthogonal polynomials can very conveniently be generated by recursion, as exposed in details in \cite{Gautschi04}, since they satisfy a three terms recurrence formula. We define for convenience
 \beq
 \hat \pi_N(x) := \sqrt{p(x,\sigma)}\pi_N(x), 
 \enq
 where $\pi_N(x)$ is $P_N(x)$ rescaled such that the coefficient of $x^N$ is unity. The recursion relations in \cite {Gautschi04} %[theorem 1.27 ]
 become
  \beq
 \begin{split}
\hat \pi_{k + 1} &= (x - \alpha_k)\hat\pi_k -\beta_k \hat\pi_{k-1}, \\
 \alpha_k &:= \frac{\int_0^\infty dx\: x \:\hat \pi^2_k(x) }{\int_0^\infty dx\: \hat \pi^2_k(x) } \\
 \beta_k &:= \frac{\int_0^\infty dx\:\hat \pi^2_k(x) }{\int_0^\infty dx\:\hat \pi^2_{k-1}(x) },
 \end{split}
 \enq
 and $\pi_{-1}(x) = 0, \pi_1(x) = 1, \beta_0 = 1$, that we implemented using an appropriate discretization of the $x$-axis.  Proper normalization of the polynomials can be performed afterwards. The Fisher information coefficients were then obtained with the help of equation (\ref{sndef}), using a precise five point finite difference method for the derivatives of $Z,A$ and $\omega^2$ with respect to $\sigma^2$ that are needed to obtain the score function.\newline
In figure \ref{fig2}, we show the cumulative efficiency $\epsilon_N(\sigma^2)$, for $N = 2$ to $N = 5$, from bottom to top. (Note that $s_1(\sigma^2)$ vanishes since the mean of $x$ is unity for any value of the variance). The uppermost line contains therefore the variance, the skewness, the kurtosis as well as the 5th moment of the field.
The contribution of each successive moment can be read out from the difference between the corresponding successive curves. For higher $N$ quick convergence of $\epsilon_N$ occurs, presented in figure \ref{fig3} as the solid line, showing $\epsilon_{10}$. For small values of the variance, the field is still close to Gaussian, so that the Fisher information is close to be entirely within the the 2nd moment, and accordingly the ratio $\epsilon$ is close to unity in this regime. It is obvious from these figures that the main effect for larger values of the variance is not that Fisher information is transferred to higher order moments, but rather the dramatic cutoff as soon as the variance crosses $0.1$.  At redshift 1, this corresponds to the scale of $\approx 1'$ \cite[figure 1 ]{2006ApJ...645....1D}, so still within scales probed by weak lensing. For $\sigma \sim 1$, the ratio is close to $0.05$, meaning that all moments completely fails to capture the information. Optimal constraints on any cosmological parameter entering $\sigma$ are thus for this value of the variance a factor $1/\sqrt{0.05} \sim 4.5$ tighter than those achievable with the help of the entire hierarchy. 
 \begin{figure}
  \includegraphics[width = \textwidth]{figs/fig2PRL}
 \caption{\label{fig2} The cumulative efficiency $\epsilon_N$ of the moments of the convergence in capturing Fisher information, for $N =2$ to $N = 5$, defined in eq. (\ref{eff}), from bottom to top, as function of the variance  of $\delta_m^\eff $.} 
 \end{figure}
 \newline\noindent
In figure \ref{fig3} we compare these results to the exact analytical expressions given in \cite{2011ApJ...738...86C} for the lognormal distribution, shown as the dashed line. These are given by, accounting for the different normalization,
\beq
s^2_N(\sigma^2) = q^2 \frac{q^N}{1-q^N} \lp \prod_{n = 1}^{N-1} \lp1 - q^n \rp \rp\lp \sum_{n = 1}^{N-1} \frac{q^n}{1-q^n}\rp^2,
\enq
with $q := 1/ (1 + \sigma^2)$. The total Fisher information content being in this case $(q/\ln q)^2 / 2 -q^2/ (4\ln q)$.
There also the information content of the moments saturates quickly as $N$ grows. It is striking that the incompleteness of the moment hierarchy occurs much earlier in the convergence field than in the lognormal. This can be understood from the following considerations. The main effect of the improved model (\ref{model}) for the convergence is to reproduce accurately the very sharp cutoff of the probability density function at low convergence values \cite[figure 3-6]{2006ApJ...645....1D}. This cutoff is very sensitive to the variance of the field, more sensitive than the cutoff of the lognormal. However, there the contribution to the moment $m_n$, $x^n$, is beaten down by orders of magnitude. To make this point clearer, we show in figure \ref{fig4} the Fisher information density $p \lp \partial_{\sigma^2}\ln p\rp^2$ for the lognormal distribution (dashed) and the model we used (solid), at the scale of $\sigma = 1$ It is obvious in both cases that a large fraction of the information is contained in the underdense regions, describing the cutoff of the distribution, but unaccessible to the moments of $x$. Since this is even more the case for the convergence field, the efficiency is accordingly even worse.
\paragraph{Restoration of the information} Finally we investigate to what extent the moment hierarchy of $\ln x$ contains more Fisher information than the hierarchy of $x$. Though our method is completely independent, this can be seen as complementary to recent works looking at the statistics of the field after local transforms, and at the statistical power of its power spectrum initiated in \cite{2009ApJ...698L..90N,2011ApJ...731..116N,2011ApJ...729L..11S}, even though in these works the fact that information actually completely escapes the hierarchy is not appreciated. This is done with the very same method used above, by obtaining the polynomials orthogonal to the distribution of $\ln x$, or equivalently decomposing the score function of $x$ in polynomials in $\ln x$ rather than in $x$. This is seen to perform very well, as shown by the dotted lines in figure \ref{fig3}. From bottom to top are plotted $\epsilon_1$,$\epsilon_2$ and $\epsilon_3$. Also shown in the figure is $\epsilon_{10}$ but it is not to be distinguished from unity, meaning that completeness of the hierarchy is restored. We see that over the full range at least $80\%$ of the information is back in the two first moments, and $95\%$ in the first three.
  \begin{figure}  \includegraphics[width = \textwidth]{figs/fig3PRL}
 \caption{\label{fig3}Solid and dashed line : the efficiency $\epsilon_{N = 10}$ of the first $10$ moments to capture Fisher information, for the convergence field (solid) and lognormal field (dashed). The curves do not change anymore with increasing $N$. Dotted : $\epsilon_1$,$\epsilon_2$, $\epsilon_3$ and $\epsilon_{10}$ for the logarithmic transform of the field, from bottom to top.} 
 \end{figure}
  \begin{figure}
  \includegraphics[width = \textwidth]{figs/fig4PRL}
 \caption{\label{fig4} The Fisher information density of the lognormal (dashed) and the convergence field (solid), renormalized such that it integrates to unity. Clearly, the Fisher information is mostly contained within the underdense regions. The moments are however sensitive to the tail.}
  \end{figure}
%-------------------------------- CONCLUSIONS :
\paragraph{Conclusions}
We have studied the statistical power of the moment hierarchy of the convergence field, when leaving the linear regime. Notably, the hierarchy ceases to provide a complete description of the statistics of the convergence, letting an increasingly large fraction of the Fisher information actually escape the hierarchy, and thus making constraints on cosmological parameters achievable with measurements of the hierarchy suboptimal by increasingly large factors. While our results are exact only for the one point distribution (or equivalently the full correlation function hierarchy of the convergence field in the limit of vanishing correlations), the correlation function hierarchy will also show a similar behavior, though the amplitude of the loss in information and constraining power may vary from parameter to parameter in the details. This is because this defect, for any number of variables, is due to the very slow decay rate at infinity of the field distribution, which cannot be reproduced by the exponential of a polynomial in the relevant variables. Our findings are consistent with previous analytical results on the lognormal distribution \cite{2011ApJ...738...86C}, and numerical work from $N$-body simulations at the power spectrum level \cite{2009ApJ...698L..90N,2011ApJ...731..116N}. Making a tighter connection to such simulation results with the methods presented here is the subject of future work. Of course, the quest for the information in the non linear regime already has problems of its own, such as shot noise issues, or accurate modeling, that we did not consider here. Nonetheless, these results clearly shows that if the correlation function hierarchy is to play a substantial role in getting constraints out of the mildly or non-linear regime, then an approach similar to a Gaussianizing transform \cite{2011ApJ...731..116N,2011ApJ...729L..11S}, in this work a simple logarithmic mapping, can hardly be avoided though the details still needs to be figured out. It is reassuring that this approach seems to work well to first order, and that first steps have recently already been taken in that direction in perturbation theory \cite{2011ApJ...735...32W}, for the matter field. Our work also points toward low convergence regions as carrying large amounts of information, though the importance of noise issues needs to be clarified in this regime. Thus, many promising ways have still to be explored to make profit of mildly and non-linear scales.



%%
%% End of file `sample.tex'.


==> chapter4.tex <==
%\setprelude{\uppercase{A\scriptsize{n inconceivably numerous host of stars must be here arranged\\ together }\normalsize{[...],}\scriptsize{ because their free positions towards each other\\ would otherwise have presented irregular forms and not exact\\ figures}}\normalsize{.}
%\vspace{5truemm}\\
%\normalsize{Immanuel Kant, {\it Universal History and Theory of the Heavens} \cite{kant1755}}}

\chapter{The correlated lognormal field as a model for the matter density field}
\label{ch4}


\begin{center}
Motivated by recent results on lognormal statistics showing that the moment hierarchy of a lognormal variable completely fails at capturing its information content in the large variance regime,  we discuss in this work the inadequacy of the hierarchy of correlation functions to describe a correlated lognormal field, which provides a roughly accurate description of the non-linear cosmological matter density field. We present families of fields having the same hierarchy of correlation functions than the lognormal field at all orders. This explicitly demonstrates the little studied though known fact that the correlation function hierarchy never provides a complete description of a lognormal field, and that it fails to capture information in the non-linear regime, where other simple observables are left totally unconstrained. We discuss why  perturbative, Edgeworth-like approaches to statistics in the non-linear regime, common in cosmology, can never reproduce or predict that effect, and why it is however generic for tailed fields, hinting at a breakdown of the perturbation theory based on the field fluctuations. We make a rough but successful quantitative connection to N-body simulations results, that showed that the spectrum of the log-density field carries more information than the spectrum of the field  entering the non-linear regime.
 \end{center}

%Commands :
\newcommand{\muln}{\bar A}
\newcommand{\covln}{\xi_{A}}
\newcommand{\sigln}{\sigma_{\ln\rho}}
\newcommand{\murho}{\bar \rho}
\newcommand{\sigd}{\sigma_\delta}
\newcommand{\sigrho}{\sigma_{\rho}}
\newcommand{\snlnmu}[2]{s_{#1}^{\muln}(#2)}
\newcommand{\snsig}[2]{s_{#1}^{\sigln^2}(#2)}

\newcommand{\idk}{\frac{d^3k}{(2\pi)^3}}
\newcommand{\Vcell}{V_{\textrm{cell}}}.

%-------------------------------- INTRODUCTION :
\section{Introduction}
The non-linear regime of structure formation in the Universe is the heart of highly challenging problems for statistical inference. This regime is also potentially very rewarding, due to the large number of modes present. As seen from the point of view of statistics, the overall picture of the linear regime is very simple in principle. Since fluctuations are believed to obey Gaussian statistics at early times, an optimal description is furnished by the two point correlation, equivalently by the (power) spectrum, the second member of the hierarchy of the $n$-point correlation functions \citep{1979MNRAS.186..145W,1980lssu.book.....P,1985ApJ...289...10F,2002PhR...367....1B}. The question of optimality is however very far from clear leaving the linear regime, and clearly out of reach yet, due to our inability to model and handle accurately very high dimensional (field) statistics beyond the Gaussian. Beside the difficulties inherent in an accurate modeling of the observables on these scales, that can be approached with perturbation theory or $N$-body simulations, statistical inference also faces other types of problems. For instance, it was shown that surprisingly little information is to be extracted from the spectrum on these scales \citep{2005MNRAS.360L..82R,2006MNRAS.370L..66N,2008ApJ...686L...1L}, due to the appearance of heavy correlations between the modes. A recent approach using local transforms of the field prior the extraction of the spectrum, also applied to its weighted projection the weak lensing convergence field, was shown be successful at recapturing much information
\citep{2009ApJ...698L..90N,2011ApJ...729L..11S,2011ApJ...731..116N,2011arXiv1109.5639S,2011PhRvD..84b3523Y,2011MNRAS.tmp.1390J,2011ApJ...742...91N}. This holds at least in the absence of discreteness or shape noise issues. While it is yet not totally clear to what extent such improvements can propagate to improvements from  galaxy survey or other sort of data, it opens a new perspective on the statistics and the description of non-linear fields. The success of these transforms, and the diagonal shape of the covariance of the spectrum up to much smaller scales that it creates, suggests that a lognormal picture is not inaccurate. That is, $\ln(1 + \delta)$ may be not too far away from a Gaussian field on these scales. Some other tentative arguments for, and confirmations to some extent of this picture in lower dimensionality have been known for a long time, and in a variety of contexts \citep[e.g.]{1991MNRAS.248....1C,1995ApJ...443..479B,1996ApJ...463..409M,2000MNRAS.314...92T,2011arXiv1105.3980H}.
\newline\newline
Beside the fact that higher order correlations may carry information, another, in cosmology largely ignored process of statistical relevance is at work for tailed fields.  The correlation function hierarchy need not provide a complete description of a field anymore in this regime, so that higher order statistics may fail to capture additional pieces of information, as first pointed out in \citep{1991MNRAS.248....1C}. This possibly means that these results on the log transform of the matter field not only bring back information from higher order statistics, but also information that was lost to the hierarchy.
The one dimensional lognormal distribution is a known instance where the moment hierarchy does not specify fully its statistics. Explicit examples of other one dimensional distributions with the same moments are known \citep{Heyde63}.  For this reason, the correlation function hierarchy cannot specify fully the statistics of a lognormal field. The first quantitative evaluation of this effect, exact in one dimension, has shown that this has a huge impact on the efficiency with which cosmological parameters can be extracted from the moment hierarchy in the non-linear regime \citep{2011ApJ...738...86C}. As pointed out by \citep{1991MNRAS.248....1C}, this is a generic effect for tailed fields. Both the matter field a well as, and even more so the convergence field \citep{2006ApJ...645....1D,2011ApJ...742...15T} show large tails in the non-linear regime. Using fits to simulations, this effect was indeed shown to affect parameter inference in the one dimensional distribution of the convergence field \citep{PhysRevLett.108.071301}. Very little is however known in higher dimensional settings. It is therefore important to gain more insights on these issues, since they strongly suggest a fundamental limitation of the correlation function hierarchy in the non-linear regime.
\newline
\newline
The main purpose of this work is to make the existence of this effect within any correlated lognormal field and its correlation function hierarchy obvious. To this aim, nothing can be better than an explicit example. In section \ref{otherfields}, we will therefore present families of fields all having the same hierarchy of correlation functions at all orders as the lognormal field, for any mean and two point correlation function. We show in this light why this effect is irrelevant in the linear regime, but not in the non-linear regime. Before turning to these aspects, we discuss in section \ref{problem} why more standard approaches in cosmology, of perturbative nature, while of course perfectly sound in the weakly non-linear regime, can never predict or reproduce this effect. These are presumably reasons for which this effect has been so little studied in cosmology so far, and are worth a few comments. In section \ref{connection}, we then make a successful connection to these recent simulation results, and we conclude in section \ref{conclusion}.
%We end with a discussion in section \ref{discussion}. 
The appendix collects proofs of key statements in section \ref{otherfields}.
\newline
\subsection{Notation and definitions}
We will be dealing with random vectors $\rho = (\rho_1,\cdots,\rho_d)$, being the sample a field
\beq
\rho_i = \rho(x_i) > 0.
\enq
For a vector $\vecn = \lp n_1,\cdots,n_d \rp$ of non negative integers (multiindex), we write as $\rho^\vecn$ the monomial in $d$ variables,
\beq
\rho^\vecn  = \rho(x_1)^{n_1}\cdots \rho(x_d)^{n_d}.% = \rho(x_1)^{n_1}\cdots \rho(x_d)^{n_d}.
\enq
Throughout this work, we reserve bold letters for vectors of integers exclusively.
Let  $p_\rho(\rho)$ be a $d$-dimensional probability density function such that all correlations of the form $\av{\rho^\vecn}$ exist.  We write the moment $\av{\rho^\vecn}$ with $m_\vecn$. Explicitly
\beq
m_\vecn = \av{\rho^{n_1}(x_1)\cdots \rho^{n_d}(x_d)}.
\enq
Correlations of order $n$ are given by moments such that the order $|\vecn|$ of the multiindex, defined as
\beq
|\vecn| :=  \sum_{i = 1}^{d}n_i
\enq
is equal to $n$.
We call these quantities moments or correlations of order $n$.  These moments coincide with the values of a continuous $n$-point correlation function on the grid sampled by $(x_1,\cdots,x_d)$. We write $\delta$ for the dimensionless fluctuation field, and $A$ for the field defined by $\ln \rho$. 
\beq 
A := \ln \rho,\quad \delta := \frac{\rho -\bar\rho}{\bar \rho}.
\enq
Such assignments involving ratios or logarithms of $d$-dimensional quantities should be understood component per component. %--------------------
\section{The problem with tailed fields}\label{problem}
In one dimension, the fact that the hierarchy does not always specify fully the distribution is a well known and still active topic of research in the theory of moments in mathematics \citep[for classical references]{Shohat63,Akhiezer65,Simon97theclassical}. The moment problem is to find a distribution corresponding to a given moment series. When a unique solution exists, it is called a  determinate moment problem.
When several exist (in this case always infinitely many), it is called an indeterminate moment problem. We can refer to \citet{1991MNRAS.248....1C,2011ApJ...738...86C} for a discussion in a cosmological context and more references. The theory of the moment problem in several dimensions is less developed, but typical criteria that guarantee determinacy, or indeterminacy, linked to the decay rate of the distribution, stay basically unchanged. Guiding us throughout the discussion in this section will be the following instance: for any dimension $d$, if
\beq \label{criterium}
\av{e^{ c |\rho | }} < \infty, \quad |\rho| = \lp \rho_1^2+ \cdots + \rho_d^2\rp^{1/2}
\enq
for some $c > 0$, then the moment problem corresponding to the moments of that distribution is determinate \citep[theorem 3.1.17]{Dunkl01}.
By a  'tailed' distribution, we have in mind in this work a decay at infinity which is less than exponential, and thus for which this criterion fails. In this regime, there may thus be several distributions with the same hierarchy of correlations.
\subsection{On its relevance for parameter inference}
It should be clear why this can have in general a dramatic impact for parameter inference from correlations. Imagine a series of distributions with identical correlations at all orders, one of these distributions being the one that actually describes the observations. Since the distributions are different, they will make in general different predictions for observables other than the correlations. Pick for definiteness an observable $\av{f(\rho)}(\alpha)$ with different predictions among this family of distribution, $\alpha$ any model parameter. The knowledge of the entire hierarchy is unable to distinguish from these different predictions for $\av{f}$, since they result from equally valid distributions.
If $\alpha$ enters the true distribution in such a way that it makes a sharp prediction on the value of $\av{f}$, this is highly valuable information definitely lost to an analyst extracting correlations exclusively.
On the other hand this argument allows us also to see that this effect can become relevant only when perturbation theory breaks down. If the fluctuation field $\delta$ is small, $f$ can be expanded in powers of $\delta$, and thus $\av{f}$ can be obtained in an unique way from the correlation hierarchy of $\delta$.
\newline\newline
 There is a remarkable way to understand what is happening there in terms of Fisher information, familiar to cosmologists.  Recall that the Fisher information matrix $F_{\alpha\beta}$ associated to a probability density function $p(\rho|\alpha,\beta,\cdots)$ is defined as
\beq\label{Fab}\Fab = \av {\frac{\partial \ln p}{\partial\alpha}\frac{\partial \ln p}{\partial\beta} }.\enq
Among the many properties that makes it a meaningful measure of information are its positivity, additivity for independent variables, its invariance under invertible transformations, the Cram\'er Rao bound and the information inequality, stating that any set of observables carries at most the same amount of Fisher information as $\rho$ itself. See \citep{fisher25,Rao,vandenbos07} for references to statistical works, and \citep{1996PhRvD..54.1332J,1996PhRvL..76.1007J,Tegmark97b,1997ApJ...480...22T} for the first implementations in cosmology, for Gaussian variables. We refer to \citep{2011MNRAS.417.1938C} for an extensive discussion of the information inequality in a cosmological context, and its deep connection with the concept of entropy. It is a fact that the Fisher information content on $\alpha$ of the distribution is entirely within the first $n$ correlations if the function $\partial_\alpha \ln p$ is a polynomial of order $n$.  In particular, the distributions for which the Fisher information matrix is within the entire hierarchy are precisely those for which the functions $\partial_\alpha \ln p$ can be written as a power series over the range of $p$. If not, the mean squared residual to the best series expansion is the amount of Fisher information absent from the hierarchy \citep[for a proof]{2011ApJ...738...86C}.  It is simple to show that criterion \eqref{criterium}, that guarantees that the distribution is uniquely set by its correlations, implies as well that the entire amount of Fisher information is within the hierarchy : this follows from the very next theorem of the same reference \citep[theorem 3.1.18]{Dunkl01}, that states that the polynomials in the $d$ variables form a dense set of functions with respect to the least mean squared residual criterion, if \eqref{criterium} is met. In particular the functions $\partial_\alpha \ln p$ can be arbitrarily well approximated by polynomials with respect to that criterion,  and therefore the correlations contain all of the Fisher information. 
\newline
\newline
It is important to note that if criterion \eqref{criterium} happens to be met due to a cutoff at a large value $\rho_\textrm{cut}$, on a otherwise tailed distribution, the correlations still are poor probes for any practical purposes.
For instance, if a variable is lognormal over a very long range, but decay quickly at infinity starting from $\rho_\textrm{cut}$. Indeed, if $\rho_\textrm{cut}$ is large enough, the correlations of order up to, say, $2N$, will be identical to that of the lognormal. Since the information content of the first $N$ correlations depends on the first $2N$ only, they will be equally poor probes as for the lognormal. They will contain the exact same amount of Fisher information as the ones of the lognormal. It is the correlations of order $>N$, that are able to feel the cutoff,  that will make up for the difference between the total information content of the lognormal distribution and its correlation hierarchy (if the cutoff is at a large enough value,  from \eqref{Fab} the two distributions have the same total amount of information). The hierarchy is thus still not well suited for the analysis of data in this regime.
\newline
\newline
For the same reason, even though any lognormal field is indeterminate, this effect plays no role for parameter inference in the linear regime, when the actual range of the variables is still small, and the tail at infinity is not yet felt. This is because in this regime on one hand the lognormal is still very close to a Gaussian over the range where it takes substantial values, and thus the lowest order correlations will still contain most of the Fisher information, and on the other hand a few higher order terms are able to reproduce deviations of the functions $\partial_\alpha \ln p$ from the Gaussian very accurately over this small range. This is consistent with the findings in section \ref{otherfields} showing that the families presented there are indistinguishable form the lognormal for any practical purposes in the linear regime.
\subsection{On other approaches to non Gaussian statistics}
Let us comment in light of the criterion \eqref{criterium} on typical perturbative approaches in cosmology to parametrize (weakly) non Gaussian distributions. These involves moments, such as Gram-Charlier, Edgeworth expansions, or the relation between the moment generating function and the distribution \citep[e.g.]{1985ApJ...289...10F,1994A&A...291..697B,1994ApJ...435..536C,1995ApJ...442...39J,1995ApJ...443..479B,1998A&AS..130..193B}, in one or several dimensions. It is therefore interesting to see to what extent they fit into this picture.  Typically, when applied to the $\delta$ field, to first order these parametrize the non-Gaussianity through a polynomial with coefficients involving the cumulants, or equivalently the moments of the variable. Schematically,
 \beq \label{Edge}
 p_\nu(\nu) \propto e^{-\nu^2/2}\lp1 + \alpha_3H_3(\nu) + \alpha_4H_4(\nu) +\cdots\rp,
 \enq
 with $\nu = \delta/\sigma_\delta$. The coefficient $\alpha_i$ depends on the first $i$ moments. The correction is given in terms of Hermite polynomials $H_{n}$, which are the orthogonal polynomials associated to the Gaussian distribution. Such expansions never produce a tailed distribution, in the sense that \eqref{criterium} is always met. The decay of the distribution namely still is Gaussian. Now, to first order and over the range of $p$, equation  \eqref{Edge} is equivalent to
 \beq
 \ln p_\nu(\nu) \approx \cst - \nu^2/2 + \alpha_3H_3(\nu) + \alpha_4H_4(\nu) + \cdots 
 \enq
 Therefore, the functions $\partial_\alpha \ln p$ will have close to polynomial form.
 This is perfectly consistent with that decomposition of the Fisher information. Indeed, this expansion creates  a probability density for which its Fisher information content is within the moments that were used to build it. This is another way to see that moment-indeterminate distributions cannot be produced by perturbative expansions.

 \section{Fields with the same hierarchy of correlation functions.}\label{otherfields}
%%%%%%%%
After reviewing the basic properties of correlated lognormal variables, we present both continuous as well as discrete families that have the same correlations as the lognormal at all orders, for any dimensionality $d$. In fact, it turns out that a stronger statement is true :  for these families, all observables of the form
\beq
\av{\rho(x_1)^{n_1}\cdots\rho(x_d)^{n_d}},\quad n_i = \cdots -1,0,1 \cdots
\enq
are identical to those of the lognormal field, i.e. any $n_i$ can also be negative as well. Including the hierarchy of inverse powers and 'mixed' powers to the usual hierarchy thus still does not provide a complete description.
\newline
\newline
These families are generalizations to any number of dimension, means and two-point correlations of known one dimensional examples that can be found in the statistical literature \citep{Heyde63,Stojanov87}.
\newline
\newline
Requirements such as homogeneity and isotropy are actually not needed for this section. In particular, unless otherwise specified, $\bar A$ is a $d$-dimensional mean vector $(\bar A(x_1),\cdots,\bar A(x_d))$, whose components can differ in principle. Nevertheless, the picture we have in mind is that of statistically homogeneous isotropic fields in a box of volume $V$, where some set of Fourier modes $k_\min$ to $k_\max$ can be probed. The corresponding Fourier representation of the two point correlations, in a continuous notation, is
\beq
\lb \xi_{A,\delta}\rb_{ij} = \int \idk P_{A,\delta}(k)e^{ik\cdot (x_i - x_j)} = \xi_{A,\delta}(x_i-x_j),
\enq
where the integral runs over these modes, and $\xi_{A,\delta}(r)$ is the ordinary two-point correlation function of $\delta$ or $A$. The matrix inverse is given by
\beq
\lb \xi^{-1}_{A,\delta}\rb_{ij} = \int \idk \frac{1}{P_{A,\delta}(k)}e^{ik\cdot (x_i-x_j)}.
\enq
This representation allow us to define a bit more rigorously what we mean by linear and non-linear lognormal field, or linear and non-linear regime, in the following discussion : if needed, it can be formally set as $P_{A}(k) \rightarrow 0 $ or $P_{A}(k) \rightarrow \infty $ respectively, for all $k$.
%-------------------
\subsection{Basic properties of lognormal fields}\label{defln}
%------------------
We say the field $\rho := (\rho(x_1),\cdots,\rho(x_d))$ is lognormal if the $d$-dimensional probability density function for $A$ is Gaussian,
\beq \label{A}
p_A(A) = \frac1{\lp 2\pi |\xi_A| \rp^{d/2}}\exp\lp  -\frac 12 (A - \bar A) \cdot \xi_A^{-1} (A -\bar A) \rp,
\enq
where $\bar A$ is the mean vector of $A$, and $\xi_A$ its covariance matrix, 
\beq
\lb \xi_A \rb_{ij} = \av{\lp A(x_i) - \bar A(x_i) \rp \lp A(x_j) - \bar A(x_j) \rp}.
\enq
The probability density for the vector $\rho$ itself is then a $d$-dimensional lognormal distribution, that we define for further reference as $p^{LN}_\rho$ :
\beq \label{pLN}
\begin{split}
p^{LN}_\rho(\rho) := \frac{ p_A(\ln \rho) }{\prod_{i = 1}^d \rho(x_i)}.
\end{split}
\enq
The means and two point correlations of $A$ and $\delta$ are in one to one correspondence. We have
\beq \label{meanA}
\bar A = \ln \bar \rho - \frac 12  \sigma^2_A
\enq
where $\sigma^2_A$ is the diagonal of $\xi_A$, i.e. the variances of the individual $d$ points. Also,
\beq \label{reldA}
\lb \xi_A \rb_{ij} = \ln \lp 1 + \lb  \xi_\delta \rb_{ij} \rp,\quad \lb \xi_\delta \rb_{ij}  := \av{\delta(x_i)\delta(x_j)} .
\enq
Especially, the variances are related through
\beq
\sigma^2_A  = \ln \lp 1 + \sigma^2_\delta\rp.
\enq
%The correlations of $\rho$ takes the simple following form
%\beq\label{Correlationrho} 
%m_\vecn = \exp \lp  \bar A \cdot \vecn + \frac 12 \vecn \cdot \xi_A \vecn\rp.
%\enq
%Note that for a lognormal field, the expectation values of negative powers of the variables also exist, and that in equation \eqref{Correlationrho}, the multiindex $\vecn$ can also have negative entries.
%----------
%------------
\subsection{Continuous family} Define the statistics of $\rho = \rho(x_1),\cdots,\rho(x_d))$ through the following. Pick a real number $\epsilon$ with $|\epsilon| \le 1$. Pick further a set of angular frequencies $\veck = (\omega_1,\cdots,\omega_d)$. Each of these must be an integer. Fix $p^{LN}_\rho(\rho)$ the $d$-dimensional lognormal distribution with mean $\bar A$ and covariance matrix $\xi_A$ defined above. Then set
\beq \label{Heydeextended}
p_\rho(\rho) := p^{LN}_\rho(\rho)\lb 1 + \epsilon \sin \lp  \pi \veck \cdot \xi_A^{-1} \lp A - \bar A \rp \rp \rb
\enq
Since $|\epsilon| \le 1$ this is positive and seen to be a well defined probability density function\footnote{For $d = 1$, there are very slight differences with Heyde original family. Heyde unnecessarily writes $2\pi$ instead of $\pi$, and restricts $\epsilon$ and $\omega$ to be positive.}. The claim that $p_\rho(\rho)$ defined in this way has the same moments $m_\vecn$ as the lognormal for any multiindex $\vecn$ is proved in the appendix. Note that in the above definition, $\bar A$ is the quantity that enters the definition of lognormal variables in equation \eqref{A}. It is however not the mean of $A = \ln \rho$ anymore, when $\rho$ is defined through \eqref{Heydeextended}.
\newline
\newline
The functional form of $p_\rho(\rho)$ consists of the lognormal envelope modulated by sinusoidal oscillations in $A$.  The smaller the two-point function the higher frequency the oscillations. This may sound curious at first, since it seems to imply that the more linear the field, the more different the distributions within this family will thus appear. However, this is precisely when the oscillations are the strongest that this effect is less relevant. This can be seen as the following. Taking the average of any function $f$ with respect to $p_\rho$ leads trivially to
\beq
\av{f} = \av{f}_{LN} + \epsilon \av{f  \sin \lp  \pi \veck \cdot \xi_A^{-1} \lp A - \bar A \rp \rp }_{LN},
\enq
where the subscript $_{LN}$ denotes the average with respect to the lognormal distribution.
In the limit of the very linear regime, other terms fixed, the second term will average out to zero for any reasonable $f$, since it is the integral of an highly oscillating function weighted by a smooth integrand. In the non-linear regime this in general ceases to be the case. 
This is illustrated as the solid lines in figures \ref{fig:pdfs} ($\sigma_\delta  = 1$) and \ref{fig:pdf2s} ($\sigma_\delta  = 0.1$), showing the member of that family in one dimension with minimal frequency $\omega = 1$, and $\epsilon = 0.1$. The dotted lines on these figures are the usual Gaussian for $A- \bar A = z$.  
%For clarity, for $d = 1$ we have the Heyde family\footnote{There is a slight difference with Heyde original family, which contains an unneeded factor of $2\pi$ rather than $\pi$.}, 
%\beq
%p_\rho(\rho) =  p^{LN}_\rho(\rho)\lb 1 + \sin \lp k \pi  \frac{\ A - \bar A} {\sigma^2_A}   \rp \rb
%\enq
  \begin{figure}
 \includegraphics[width = \textwidth]{figs/fig1APJ}
  \caption{\label{fig:pdfs} Three different one dimensional distributions for $z = A-\bar A$, with identical moments $\av{\rho^n}, \: \rho = e^A$, for all integer $n$, positive or negative. The dashed line is the zero mean Gaussian distribution, so that $\rho$ is lognormal. The solid the member of the family in \eqref{Heydeextended} with the lowest possible frequency, and amplitude $\epsilon = 0.1$. The discrete one is \eqref{discreteP} with shift parameter $\alpha = 0.25$. They are shown at the scale of non linearity $\sigma_\delta = 1$, where this indeterminacy starts to become very relevant for inference. The families in any dimension are qualitatively identical to these. } 
 \end{figure}
  \begin{figure}
 \includegraphics[width = \textwidth]{figs/fig2APJ}
 \caption{\label{fig:pdf2s} Same as figure \ref{fig:pdfs}, for $\sigma_\delta = 0.1$, when the indeterminacy if far less relevant for inference, for the reasons given in the text. The discrete distribution has been scaled by a constant factor for convenience.} 
 \end{figure}
The probability density function for $\ln \rho$ is not purely Gaussian anymore. It is therefore of interest to see how the correlations of $A$ deviate from those of Gaussian variables. For instance the means $\av{A-\bar A}$ do not vanish anymore as for the lognormal. A straightforward calculation leads to
\beq
\av{(A - \bar A)(x_i)} = -\epsilon \:\pi \omega_i \exp\lp-\frac{\pi^2}2 \veck\cdot \xi_A^{-1} \veck\rp.
\enq
Picking $\veck$ as having a single non zero entry, $\omega$, at $x_i$ we get that they can be as large as
\beq \label{meanz}
\begin{split}
\av{(A - \bar A)(x_i)} &= -\epsilon \:\pi \omega \exp\lp-\frac{\pi^2}2 w^2 \lb \xi_A^{-1}\rb_{ii}\rp \\
&:=  -\epsilon \:\pi \omega\exp\lp-\frac{\pi^2}2 \frac {\omega^2}{\sigma^2_{A,\textrm{eff}}(x_i)} \rp
\end{split}
\enq
Observables as simple as the means of $A$ are therefore not constrained by the knowledge of the entire correlation hierarchy of the lognormal field. While the effect is irrelevant in the linear regime (for say $\sigma_{A,\textrm{eff}} = 0.1$, the maximal value of the mean in equation \eqref{meanz} is only $\approx 10^{-215})$, deep in the non-linear regime this is not the case anymore. It is easy to show from the above expression that the range available to $ \av{\lp A - \bar A\rp(x_i)}$, choosing $w$ appropriately, scales to infinity with $\propto \sigma_{A,\textrm{eff}}$. The means are thus left totally unconstrained in that regime. This and the very sharp behavior is of course a generic effect, not limited to that particular observable. It is obvious that the relevance of this effect for parameter inference is very  sensitive to the degree of linearity of the field, and that large amounts of information are lost to the hierarchy in the high variance regime\footnote{Among this family, it turns out that some observables such as the variances $\av{(A-\bar A)^2(x_i)}$ are always identical to $\sigma^2_A(x_i)$ for any choice of $\epsilon$ and $\veck$. We do not attach any significance to this, since this is not the case for the discrete family, though closed analytical expressions cannot be obtained in this case.}.
\subsection{Discrete family}
Fix again the dimensionality $d$, the vector $\bar A$ and the matrix $\covln$. For all integer valued $d$-dimensional multiindex $\vecn$ define a realization $A_\vecn$ of $A$ as the following. Pick $\alpha = (\alpha_1,\cdots,\alpha_d)$ any point, and set
\beq \label{An}
A_\vecn := \bar A + \xi_A \cdot \lp \vecn - \alpha \rp.
\enq
While $\alpha$ can in principle be anything,  only components $\alpha_i \in [0,1)$ will actually define different grids. As usual, $\rho$ is given by exponentiation,
\beq \label{rhon}
\rho_\vecn := \exp\lp A_\vecn \rp
\enq
Assign then to these realizations parametrized by $\vecn$ a probability
\beq \label{discreteP}
P_\vecn = \frac 1 Z \exp \lp-\frac 12 \lp A_\vecn - \bar A\rp \cdot \xi_A^{-1}\lp A_\vecn - \bar A\rp\rp.
\enq
These are usual Gaussian probabilities for $A_\vecn$, except that we have only a discrete set of field realizations.
Note that it can be written, maybe more conveniently, as
\beq
P_\vecn = \frac 1 Z \exp \lp -\frac 12  \lp \vecn -  \alpha\rp \cdot \xi_A \lp \vecn - \alpha\rp\rp.
\enq
Since $\xi_A$ is positive definite, the normalization factor $Z$ is seen to be well defined, as for more usual Gaussian integrals, and so are the probabilities. This discrete probability distribution has the same moments of $\rho_\vecn$ than the $d$-dimensional lognormal distribution with associated $\bar A$ and $\xi_A$, as proven in the appendix. Again, negative entries in $\vecn$ are allowed.
\newline
\newline
This family is clearly different from the previous, continuous one. Rather than modulating the lognormal distribution with an oscillating factor, it is a series of Dirac delta functions sampling the lognormal on the grid given by \eqref{An}. The role of $\alpha$ is to shift the sample by a small amount. If $\alpha$ is set to zero, then $A = \bar A$ is part of the sample, while it is not if not. The fact that  this indeterminacy is irrelevant in the linear regime comes this time from realizing that for any nice enough function $f$, the average of $f$ will converge to $\av{f}_{LN}$ due to the trapezoidal rule of quadrature. The grid spacing at which $A$ is sampled in this way in \eqref{rhon} becomes namely thinner and thinner. In the non-linear regime, the spacing is however very large, leading again to large deviations. This is also illustrated in figure \ref{fig:pdfs} and \ref{fig:pdf2s} for the one dimensional version of it, with shift parameter $\alpha = 0.25$.
%----
\section{Connection to simulations and discussion}\label{connection}
One of us \citep{2011ApJ...742...91N} analysed the Coyote Universe N-body simulations suite \citep{2010ApJ...715..104H,2010ApJ...713.1322L} in a box of volume $V = 2.2 $Gpc$^3$, with $256^3$ cells, extracting the spectrum  $P(k)$ of $A$ and $\delta$ over then range $0.02/$Mpc $ \lesssim k \lesssim 0.6 /$Mpc, comparing their statistical power as function of the smallest scale $k_\max$ included in the analysis for several cosmological parameters. It was found that the spectrum of $A$ has more constraining power on cosmological parameters than that of $\delta$, when the non linear scales are included in the analysis. We refer to that paper for more details on the procedures and results. In this framework, $\rho$ is $1 + \delta$, and thus $A   =\ln (1 + \delta)$. The fields are statistically homogeneous and isotropic.
\newline\newline
Given the considerations of the previous sections, and the fact that the density field is known to be somewhat  close to lognormal, these results can hardly be considered surprising. The field $A$ must be indeed closer to a Gaussian field for all values of the cosmological parameters, so that low order $N$ point functions of $A$ must contain a larger fraction of the information than those of $\delta$ (it is useful to remember that the full fields $A$ and $\delta$ carry in all cases the very same total amount of information, since the mapping between them is parameter independent and invertible). In this section we want to go a step further from these qualitative considerations and make a quantitative comparison of these results to simple analytical methods using lognormal statistics.
\subsection{Treating information in $A$ as Gaussian.}
First, we need to make sure that a Gaussian description of the field $A$ is reasonable, at least for what concerns the information  content. In particular, this is not the case for the smallest scales of $A$, since the covariance matrix of $P_A$ in the $256^3$ box clearly shows substantial off diagonal elements starting from $k \simeq 0.3$/Mpc. We therefore repeated the same analysis, performing the logarithmic transform on the $\delta$ field only after smoothing $\delta$ on twice the original length scale, by merging the $256^3$ into $128^3$ cells. This allowed us to extract the spectra of $A$ and $\delta$ over the range  $0.02/$Mpc $ \lesssim k \lesssim 0.3 /$Mpc,  with a diagonal covariance matrix over the full range to a very good approximation. It is important to realize that sadly it is not identical to the much simpler approach of considering the original $A$ field only up to the new $k_\max$: since all the scales of $\delta$ have an impact on the large scales of $A$, the operations of smoothing $\delta$ and then log transforming $\delta$ are not identical to log transforming $\delta$ and then smoothing $A$.
\newline\newline
For a purely Gaussian field with spectrum $P$, the information content on $\alpha$ in the spectrum is given by
\beq \label{FG}
F_{\alpha\alpha}  = \frac V 2 \int \idk \lp \frac{\partial \ln P(k)}{\partial \alpha} \rp^2,
\enq
where the sum runs over the modes extracted,
and
\beq \label{cstrFG}
\frac 1 {\sqrt{F_{\alpha\alpha}}} =: \Delta(\alpha)
\enq
can be thought of as approximating the constraints on $\alpha$ achievable with these modes.  We focus for reasons that become clear below primarily on the parameter $\ln \sigma^2_8$, which has a roughly constant impact both on $\ln P_{\delta}$ and $\ln P_{A}$. In figure \ref{fig:cstr}, we compare this for the $\delta$ field and the $A$ field as function of $k_\max$. The solid lines are the simulation results, evaluating the covariance matrix $C_{kk'}$ between the modes $k$ and $k'$ and setting
\beq \label{FGnum}
\Delta(\ln \sigma^2_8) = \sum_{k,k'\le k_\max}\frac{\partial \ln P(k)}{\partial{\ln \sigma^2_8}}  C^{-1}_{kk'}\frac{\partial \ln P(k')}{\partial{\ln \sigma^2_8}},
\enq
while the dashed lines are in both cases equation \eqref{cstrFG} given by \eqref{FG}, with the derivatives being those extracted from the simulations. Since the derivatives are roughly constant, the dashed lines scale like $k^{-3/2}$, i.e. the inverse root of the number of modes. It is clear that the log transform extends the (rough) validity of the Gaussian approximation in terms of Fisher information to the full range of scales we are dealing with. Note however that this is a statement only up to the four point level, since those are the only ones that enter \eqref{FG} and \eqref{FGnum}.
\begin{figure}
\includegraphics[width = \textwidth]{figs/fig3APJ}
\caption{Comparison of various estimates of the error bar on the linear power spectrum amplitude, $\ln\sigma_8^2$, constrained using power spectra of the overdensity $\delta$ (black) and the log-density $A$ (red) in an $N$-body simulation.  Solid curves show how the error bars tighten as the maximum $k$ analyzed increases up to the Nyquist frequency, as in e.g. \cite{2011ApJ...742...91N}, equation \eqref{FGnum}. Dotted curves neglect the non-Gaussian component of the covariance matrices, as well as the discrete nature of the Fourier-space mode lattice, equation \eqref{FG}.  The arrows (one for each choice of $\sigma_A$, 0.7 and 0.9) show the expected degradation of the error bars from analyzing $\delta$ instead of $A$ in our model given by equation \eqref{ratioss}; these factors appear numerically in the first column of Table \ref{table}.    \label{fig:cstr}}
\end{figure}
\subsection{Comparison to simulations}
To compare these results to analytical predictions from lognormal statistics, we first note the following. For a parameter, such as $\ln \sigma^2_8$, that obeys roughly
\beq
\frac{\partial \ln P_A(k)}{\partial \alpha} \approx \cst = : c,
\enq
the correlated Gaussian field $A$ is equivalent, from the point of the view of the information on that parameter, to a field with the same variance but with $\xi(r) = 0$ for $r > 0$. This may not sound like an obvious statement so let us show this explicitly : start from equation \eqref{FG} which leads to
\beq
F_{\alpha\alpha} = c^2\: \frac V 2 \int \idk
\enq
The integration on the right, in a discrete description, is the number of available modes, equal to the number $d$ of grid points, times the spacing of the modes $\Delta k = (2\pi)^3/V$. It follows
\beq \label{Ftot}
F_{\alpha\alpha} = c^2 \: \frac d 2.\
\enq
On the other hand, the observation of $d$ uncorrelated Gaussian variables with variance $\sigma^2_A$ always carries the information
\beq \label{Fvar}
 d\: \lp \frac{\partial \sigma^2_A}{\partial \alpha}\rp^2 \frac 1{2\sigma^4_A}
\enq
in their variances.
If the derivative of $\ln P$ is the constant $c$, we have
\beq
\begin{split}
\frac{\partial  \sigma^2_A}{\partial \alpha} &=\int \idk  \frac{\partial P_A(k) }{\partial\alpha } \\ &= \int \idk P_A(k) \frac{\partial\ln P_A(k)}{\partial \alpha} \\& =  c
\: \sigma^2_A.
\end{split}
\enq
and thus expressions \eqref{Ftot} and \eqref{Fvar} are identical. In terms of information on such parameters, the correlated, Gaussian $A$ field is thus exactly equivalent to $d$ uncorrelated Gaussian variables with the same variances. These parameters  can be seen as entering therefore predominantly the variance, the two point correlation function at zero lag, that contains most information, and the correlations at non zero lag carrying little independent information. This is also expected to hold for the $\delta$ field, since it is very non-linear and the variance dominates  over the clustering in the two point correlation matrix, i.e. the two point correlation matrix is close to diagonal, so that the variance will dominate in any covariance matrix, as well as in the sensitivity to the parameter.
\newline\newline
Since information just adds up for any number independent variables, this means that we can try and use directly the exact results one of us derived \citep{2011ApJ...738...86C} for the one dimensional lognormal distribution to get a rough but still reasonable estimate of the improvement in the constraints from analyzing the $A$ field. In that work were derived the cumulative efficiencies
\beq
\epsilon_N^\sigma = \frac{1}{F_{\alpha\alpha}} \sum_{n = 2}^N\lp s_n^\sigma\rp^2  \in (0,1)
\enq
of the first $N$ moments of the $\delta$ field to catch the information in $A$ (equations 31-35 as well as figure 2 and figure 1, solid line, in that paper). These coefficients are extremely sensitive functions of $\sigma^2_A$, decaying like $\exp(-4\sigma^2_A) \sim \sigma_\delta^{-8} $ as soon as $\sigma_A$ becomes close to unity.
\newline\newline
There is a slight modification to make to these coefficients so that we can confront them to the simulations. From the simulations only the spectrum of $A$ were extracted, but not the mean of $A$, which also carries information in principle, even if $\delta$ itself has zero mean. For a one dimensional lognormal variable with unit mean, we have from equation \eqref{meanA} that $\bar A = -\frac 12 \sigma^2_A $. For that lognormal variable the total information is given by the usual formula for the Gaussian $A$,
\beq
F_{\alpha\alpha} = \frac{1}{\sigma^2_A}\lp \frac{\partial \bar A}{\partial \alpha} \rp^2+ \frac{1}{2\sigma^4_A}\lp\frac{\partial \sigma^2_A}{\partial \alpha}\rp^2.
\enq
It reduces thus to
 \beq
 F_{\alpha\alpha} = \frac{1}{2\sigma^4_A}\lp\frac{\partial \sigma^2_A}{\partial \alpha}\rp^2 \lp 1 + \frac{\sigma^2_A}{2}\rp,
\enq
where the rightmost term contains the part of the information in the mean of $A$.
The efficiencies ratios of the moments of $\delta$ to that of the variance of $A$ only, excluding the mean, becomes thus
\beq
\tilde \epsilon_N^\sigma:= \epsilon^\sigma_N \lp 1 + \frac {\sigma^2_A} 2\rp.
\enq
Note that in principle theses efficiencies can now be larger than unity, if the moments of $\delta$ would capture not only the information in $\sigma^2_A$, but also that in $\bar A$.
\newline
\newline
The improvement factors, i.e. the ratio of the constraints on $\alpha$ from analyzing the first $N$ correlation functions of $\delta$, to the the constraint from the two-point function of A, are thus in this model
\beq \label{ratioss}
\lb \tilde \epsilon^\sigma_N \rb^{-1/2} =: \Delta^\delta_N(\alpha)/ \Delta^A_2(\alpha).
\enq
They are independent of the parameter $\alpha$ in this one dimensional picture, since the only relevant parameter is $\sigma^2_A$, or equivalently $\sigma^2_\delta$. Remember that the denominator on the right hand side can actually be calculated for any lognormal field from \eqref{FG}, our additional assumptions can be seen thus as entering only the numerator. We argued that this ratio is expected to be correct for parameters such as $\ln \sigma^2_8$, but they become in all cases exact for a lognormal field whose variance dominates enough the clustering, $\xi_\delta(r) / \sigma_\delta^2 \ll 1$, for all $r$. The effective nearest neighbor distance given the modes we used can be evaluated as $r_\min \approx \int \idk ^{-1/3}$,  and we find $\xi_\delta(r_\min) / \sigma^2_\delta = 0.3$.
\newline\newline
Finally, there is slight ambiguity in evaluating $\tilde \epsilon_n^\sigma$. A purely lognormal field has $\sigma_A = [\ln (1+\sigma^2_\delta)]^{1/2}$, but this relation is not fulfilled precisely in our simulations. We obtain $\sigma_A = 0.7, \sigma_\delta = 1.1$ and so $, [\ln (1 + \sigma_\delta^2)]^{1/2} = 0.9$ rather than $0.7$. This discrepancy may be due of course to an intrinsic failure of the lognormal assumption, or to the presence of the smallest scales, slightly correlated, as seen from the start of saturation in figure \ref{fig:cstr}. 
\newline\newline
We show in the first two rows of Table \ref{table} the factors of improvement for these two values of $\sigma_A, 0.7 $ and $0.9$, for $N= 2,3$ and $\infty$.  In the third row is shown the improvement found extracting $P_A$ rather than $P_\delta$ in the simulations. Given our assumptions, and the very high sensitivity of $\epsilon_N^\sigma$ to the variance of the field, they agree remarkably : for the sake of comparison, a variance twice as large of $\sigma_A = 2 \rightarrow \sigma_\delta = 7.3$ would have predicted a factor of $\Delta_2 (\delta)/ \Delta_2(A) = 522$, and for $\sigma_A = 3 \rightarrow \sigma_\delta = 90$ a factor of $\approx 5\cdot10^6$. 
\newline
 \newline
We also performed this analysis for the tilt parameter $n_s$, which from its very definition has a very differentiated impact over different modes, and finding, just as in the original analysis \citep{2011ApJ...742...91N}, that the improvement factor is roughly parameter independent as shown in the fourth row of the table. This is another argument supporting the view that the dynamics of the information are indeed captured by such a simple picture. It may be due to the fact that the smallest scales, containing the largest number of modes, contributes the majority of the information in $A$ for any parameter, and thus that the sensitivity can be effectively treated as constant, equal to its value on small scales, making our argument above valid for basically any parameter. Note that for both values of $\sigma_A$ the spectrum of $A$ still outperforms the entire hierarchy of $\delta$ by a sizeable factor for the lognormal model. Of course, this is much more speculative.

\begin{center} 
\begin{table} 
\begin{tabular*}{\textwidth}{|cccc}
%% All data must appear between the \startdata and \enddata commands
%\startdata
&$\Delta^\delta_2 / \Delta^A_2$ & $\Delta^\delta_3 / \Delta^A_2$ &$\Delta^\delta_\infty / \Delta^A_2$ \\ 
LN, $\sigma_A = 0.7$ & 2.0 & 1.6 & 1.3 \\
LN, $\sigma_A = 0.9$ & 2.9 & 2.4 & 2.1 \\
Sim. $\alpha = \ln \sigma^2_8$ & 2.5 & & \\
Sim. $\alpha =  n_s$ & 2.4 & & \\
\end{tabular*}
\end{table}
\end{center}

% \section{Discussion} \label{discussion}

\section{Conclusion and discussion} \label{conclusion}
We have made clear that the correlation functions are generically very poor descriptors and probes of fields with large tails. This is especially true for the lognormal field, a standard prescription for the statistics of cosmological non-linear fields, and we provided other explicit fields with exactly the same hierarchy at all orders. We showed that the knowledge of the entire hierarchy of $N$ point functions of a non-linear lognormal field is insufficient to constrain other, simple, observables. We discussed the links between these aspects and the failure of power series expansions to reproduce relevant functions. We argued that this inadequacy is responsible for the recent successes of the log transforms in cosmology at recapturing information, and that they may not only bring back information from higher order statistics, but likely also information that cannot be probed at all with the hierarchy. We then showed that the factors of improvements on constraints from analyzing the spectrum of $A$ to that of $\delta$ as seen in $N$-body simulations are in quantitative agreement with simple analytical predictions using lognormal statistics.
\newline
\newline
Observational noise issues were not considered in this work. It remains therefore unclear to what extent these improvements can be achieved with actual galaxy survey data. Generically, it is reasonable to expect that noise will reduce these improvement factors. This work nonetheless makes clear that in this case, improving the specifications of a survey in order to decrease the observational  (e.g. shot) noise will be at the same time actually reducing the efficiency with which cosmological parameters can be extracted with the hierarchy of $\delta$ (i.e. the fraction of information that is contained in the hierarchy with respect to the total).
\newline
\newline
Surely, the question of the incompleteness of the hierarchy of the matter or any other field is in itself to a certain extent academical, since high order correlations will probably anyway stay out of reach for a long time. Nevertheless, it provides directions and insights into the recent successes of these transforms, strongly suggesting that in the non-linear regime, an approach using transforms is much more promising than targeting higher order statistics for inference on any parameter. We are also convinced that the statistical methods and formalism introduced will be more widely applicable in the future. Progress on these issues will be reported in due time.

\clearpage
\newpage

%%%%%%%%
\section{Proofs}\label{proofs}
%%%%%%%%
We prove the claim made in this work that the distributions we defined have the same correlations than the lognormal at all orders.  As we will see this is also true including 'negative orders' and 'mixed orders', i.e. when negative powers of the variables are allowed in the correlations. 
\newline
Recall that for lognormal variables $\rho = (\rho_1,\cdots,\rho_d)$ with means and covariance matrix of their logarithms $\bar A = (\bar A _1,\cdots \bar A_d)$ and $\covln$ we have
\beq \label{mln}
m_\vecn := \av{\rho^\vecm}=  \av{\rho_1^{n_1}\cdots \rho_d^{n_d}} =  \exp \lp \vecn \cdot \bar A + \frac 12 \vecn\cdot \covln \vecn \rp,\quad \vecn = (n_1,\cdots,n_d).
\enq
A simple proof of this fact is to make use of the standard formulae for Gaussian integrals, valid for any positive matrix $\xi_A$, mean vector $A$ and vector $z$, that can be complex valued.
\beq \label{Gintegral}
\frac{1}{\lp 2\pi  \rp^{d/2}}\frac{1}{\sqrt {\det \xi_A}} \int d^d A \exp\lp-\frac 12\lp A - \bar A\rp \cdot \xi_A^{-1}\lp A - \bar A\rp + \lp A - \bar A \rp \cdot z \rp = \exp\lp \frac 12 z \cdot \xi_A z\rp.
\enq
Essentially all calculations in this work follow from this formula. Even the proof for the discrete family can be considered a discrete version of that relation.
%----------
\subsection{Continuous}\label{continuous}
%---------
\noindent
To prove our claim it is enough to show that
\beq \label{toprove1}
\av{\rho^\vecn \sin \lp \pi  \:\veck \cdot \covln^{-1}\lp A -  \bar A\rp\rp }_{LN} = 0.
\enq
This must hold for any  $d$-dimensional multiindices $\veck $ and $\vecn$ (we allow entries to be negative), where the average is taken with respect to the lognormal density function, equation \eqref{pLN}. We proceed as the following : we evaluate the following integral
\beq \label{A4}
I(\vecn,\veck) := \av{\rho^\vecn \exp \lp i\pi  \:\veck \cdot \covln^{-1}\lp A -  \bar A\rp\rp }_{LN},
\enq
and show that its imaginary part vanishes for $ \veck$ and $\vecn$ as specified.
\newline
Writing equation \eqref{A4} using
\beq
\rho^\vecn = \exp(\vecn \cdot A) = \exp\lb \vecn \cdot \lp A - \bar A \rp + \vecn \cdot \bar A \rb
\enq
leads immediately to the Gaussian integral given in \eqref{Gintegral}, with $z = \vecn +  i \pi \xi_A^{-1}\veck$. It follows from that equation
\beq
I(\vecn,\veck) = \exp \lb \vecn\cdot \bar A + \frac 12 \lp \vecn + i\pi \covln^{-1}\veck \rp \cdot \covln  \lp \vecn +i \pi \covln^{-1}\veck \rp  \rb.
\enq
Separating real from imaginary argument, this expression reduces to
\beq
\begin{split}
I(\vecn,\veck) =& \exp \lp  \vecn\cdot \bar A + \frac 12 \vecn \cdot \covln \vecn - \frac{ \pi^2}{2}\veck\cdot \covln^{-1}\veck   \rp \cdot \exp \lp i\pi  \: \veck \cdot \vecn \rp.
\end{split}
\enq
The imaginary part of that expression is thus proportional to $\sin \pi\: \veck \cdot \vecn$. Whenever $\veck$ and $\vecn$ are integer valued, so is their scalar product $\veck \cdot \vecn = \sum_i \omega_in_i$. Therefore, the sine vanishes and \eqref{toprove1} is proved.
\subsection{Discrete}
\noindent
From equation \eqref{An} and \eqref{rhon}, we have
\beq
\rho_\vecn^\vecm = \exp \lp \vecm \cdot \bar A + \vecm \cdot \xi_A\lp \vecn - \alpha \rp \rp.
\enq
It follows that the moments of $\rho$ are given by
\beq
\av{\rho^\vecm} = \frac {e^{\vecm\cdot \bar A}} Z \sum_{\vecn \in \mathbb Z^d} \exp \lb -\frac 12 \lp \vecn -\alpha \rp\xi_A \lp \vecn-\alpha\rp + \vecm\cdot \xi_A\lp \vecn - \alpha \rp\rb.
\enq
The proof is based on completing the square in the exponent, in perfect analogy of standard proofs of the Gaussian integral in \eqref{Gintegral}. Write
\beq
 -\frac 12  \lp \vecn -\alpha \rp \cdot \covln  \lp \vecn -\alpha \rp + \vecm \cdot \covln  \lp \vecn -\alpha \rp = -\frac 12 \lp \vecn - \vecm -\alpha \rp \covln \lp \vecn - \vecm - \alpha\rp + \frac 12 \vecm\cdot \covln \vecm,
\enq
and then perform the shift of summing index $\vecn \rightarrow \vecn + \vecm$, obtaining
\beq
\av{\rho^\vecm} = \exp \lp\vecm \cdot \bar A + \frac 12 \vecm \cdot \covln \vecm\rp \frac 1 Z \sum_{\vecn \in \mathbb Z^d}\exp\lp-\frac 12 \lp \vecn -\alpha \rp \cdot \covln \lp \vecn -\alpha \rp \rp.
\enq
Since the sum ranges over all the multiindices, the shift does not create boundary terms.
This last sum is nothing else than $Z$, so that we recover
\beq
\av{\rho^\vecm} = \exp \lp\vecm \cdot \bar A + \frac 12 \vecm \cdot \covln \vecm\rp,
\enq
which are indeed the same as the lognormal in \eqref{mln}. Again, this is also true if negative entries in $\vecm$ are permitted.
%
% ****** End of file apstemplate.tex ******


